Comparison Between IPv4 to IPv6 Transition Techniques

The IPv4 addresses exhaustion demands a protocol transition from IPv4 to IPv6. The original transition technique, the dual stack, is not widely deployed yet and it demanded the creation of new transition techniques to extend the transition period. This work makes an experimental comparison of techniques that use dual stack with a limited IPv4 address. This limited address might be a RFC 1918 address with a NAT at the Internet Service Provider (ISP) gateway, also known as Carrier Grade NAT (CGN), or an Address Plus Port (A+P) shared IPv4 address. The chosen techniques also consider an IPv6 only ISP network. The transport of the IPv4 packets through the IPv6 only networks may use IPv4 packets encapsulated on IPv6 packets or a double translation, by making one IPv4 to IPv6 translation to enter the IPv6 only network and one IPv6 to IPv4 translation to return to the IPv4 network. The chosen techniques were DS-Lite, 464XLAT, MAP-E and MAP-T. The first part of the test is to check some of the most common usages of the Internet by a home user and the impacts of the transition techniques on the user experience. The second part is a measured comparison considering bandwidth, jitter and latency introduced by the techniques and processor usage on the network equipment.

==> README <==
LaTeX package 'doclicense'
~~~~~~~~~~~~~~~~~~~~~~~~~~
Copyright (C) 2015 by Robin Schneider <ypid@riseup.net>

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in
  http://www.latex-project.org/lppl.txt
and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.

CTAN: https://www.ctan.org/pkg/doclicense
Code repository: https://github.com/ypid/latex-packages/tree/master/doclicense

Question on Stackexchange: https://tex.stackexchange.com/a/226788/32320


  DESCRIPTION
Support for putting documents under a license.

The doclicense package allows you to put your document under a license and include a link
to read about the license or include an icon or image of the license.
Currently, only Creative Commons is supported but this package is designed to
handle all kinds of licenses.

  GENERATING THE FILES
You can generate the doclicense.sty file with: tex doclicense.ins

The documentation can be generated with:

    pdflatex doclicense.dtx
    makeindex -s gglo.ist -o doclicense.gls doclicense.glo
    makeindex -s gind doclicense
    pdflatex doclicense.dtx
    thumbpdf doclicense
    pdflatex doclicense.dtx

Note that this will only work when this directory is below your
$TEXMFHOME tree (unless the doclicense package is already installed
for example by your TeX distribution). Example for doing this manually:

    mkdir --parents ~/texmf/tex/latex/ && cd ~/texmf/tex/latex/
    git clone https://github.com/ypid/latex-packages.git ypid-latex-packages
    cd ypid-latex-packages/doclicense && make build
    ## Or
    make all

If you have not worked with $TEXMFHOME you might want to refer to the
documentation of your TeX distribution for details. See also the next section.

  IMPORTANT NOTES REGARDING TDS

Please note that the images/ and the license-texts/ subdirectories must end up in the runtime tex/
subtree (that is tex/latex/doclicense/) for the \doclicenseImage macro and the \doclicense*FullText macros to work
correctly.


==> images/Makefile <==
WGET_OPTIONS ?= --no-verbose

.PHONY: default all
default: all

all: doclicense-CC-by.pdf doclicense-CC-by-sa.pdf doclicense-CC-by-nd.pdf doclicense-CC-by-nc.pdf doclicense-CC-by-nc.eu.pdf doclicense-CC-by-nc-sa.pdf doclicense-CC-by-nc-sa.eu.pdf doclicense-CC-by-nc-nd.pdf doclicense-CC-by-nc-nd.eu.pdf doclicense-CC-pd.pdf doclicense-CC-zero.pdf
	rename 's#\.eu\.#-eu.#' -v *
	for file in *-eu.pdf; do oldfile="$${file%-eu.pdf}.eu.pdf"; ln -s "$$file" "$$oldfile"; done

doclicense-CC-pd.pdf: doclicense-CC-publicdomain.pdf
	mv "$<" "$@"
	ln -sf "$@" "$<"

doclicense-CC-zero.pdf: doclicense-CC-cc-zero.pdf
	mv "$<" "$@"
	ln -sf "$@" "$<"

doclicense-CC-%.pdf: %.svg
	rsvg-convert -f pdf -o "$@" "$<"

doclicense-CC-%.pdf: %.eps
	epstopdf "$<" --outfile="$@"

%.svg:
	wget $(WGET_OPTIONS) "http://mirrors.creativecommons.org/presskit/buttons/88x31/svg/$@"

%.eps:
	wget $(WGET_OPTIONS) "http://mirrors.creativecommons.org/presskit/buttons/88x31/eps/$@"

.PHONY: clean distclean
clean: distclean
	rm -rf *.svg
	rm -rf *.eps


==> license-texts/doclicense-CC-by-3.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution 3.0 Unported}





\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES
NOT PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE
DOES NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE
COMMONS PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS.
CREATIVE COMMONS MAKES NO WARRANTIES REGARDING THE
INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR DAMAGES
RESULTING FROM ITS USE.
\end{quotation}
\subsubsection{\emph{License}}
\par THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS
OF THIS CREATIVE COMMONS PUBLIC LICENSE (``CCPL'' OR
``LICENSE''). THE WORK IS PROTECTED BY COPYRIGHT AND/OR OTHER
APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS
PROHIBITED.
\par BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU
ACCEPT AND AGREE TO BE BOUND BY THE TERMS OF THIS LICENSE.
TO THE EXTENT THIS LICENSE MAY BE CONSIDERED TO BE A
CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS CONTAINED HERE
IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.
\par \textbf{1. Definitions}
\begin{enumerate}
\item \textbf{``Adaptation''} means a work based upon
the Work, or upon the Work and other pre-existing works,
such as a translation, adaptation, derivative work,
arrangement of music or other alterations of a literary
or artistic work, or phonogram or performance and
includes cinematographic adaptations or any other form in
which the Work may be recast, transformed, or adapted
including in any form recognizably derived from the
original, except that a work that constitutes a
Collection will not be considered an Adaptation for the
purpose of this License. For the avoidance of doubt,
where the Work is a musical work, performance or
phonogram, the synchronization of the Work in
timed-relation with a moving image (``synching'') will be
considered an Adaptation for the purpose of this
License.
\item \textbf{``Collection''} means a collection of
literary or artistic works, such as encyclopedias and
anthologies, or performances, phonograms or broadcasts,
or other works or subject matter other than works listed
in Section 1(f) below, which, by reason of the selection
and arrangement of their contents, constitute
intellectual creations, in which the Work is included in
its entirety in unmodified form along with one or more
other contributions, each constituting separate and
independent works in themselves, which together are
assembled into a collective whole. A work that
constitutes a Collection will not be considered an
Adaptation (as defined above) for the purposes of this
License.
\item \textbf{``Distribute''} means to make available
to the public the original and copies of the Work or
Adaptation, as appropriate, through sale or other
transfer of ownership.
\item \textbf{``Licensor''} means the individual,
individuals, entity or entities that offer(s) the Work
under the terms of this License.
\item \textbf{``Original Author''} means, in the case
of a literary or artistic work, the individual,
individuals, entity or entities who created the Work or
if no individual or entity can be identified, the
publisher; and in addition (i) in the case of a
performance the actors, singers, musicians, dancers, and
other persons who act, sing, deliver, declaim, play in,
interpret or otherwise perform literary or artistic works
or expressions of folklore; (ii) in the case of a
phonogram the producer being the person or legal entity
who first fixes the sounds of a performance or other
sounds; and, (iii) in the case of broadcasts, the
organization that transmits the broadcast.
\item \textbf{``Work''} means the literary and/or
artistic work offered under the terms of this License
including without limitation any production in the
literary, scientific and artistic domain, whatever may be
the mode or form of its expression including digital
form, such as a book, pamphlet and other writing; a
lecture, address, sermon or other work of the same
nature; a dramatic or dramatico-musical work; a
choreographic work or entertainment in dumb show; a
musical composition with or without words; a
cinematographic work to which are assimilated works
expressed by a process analogous to cinematography; a
work of drawing, painting, architecture, sculpture,
engraving or lithography; a photographic work to which
are assimilated works expressed by a process analogous to
photography; a work of applied art; an illustration, map,
plan, sketch or three-dimensional work relative to
geography, topography, architecture or science; a
performance; a broadcast; a phonogram; a compilation of
data to the extent it is protected as a copyrightable
work; or a work performed by a variety or circus
performer to the extent it is not otherwise considered a
literary or artistic work.
\item \textbf{``You''} means an individual or entity
exercising rights under this License who has not
previously violated the terms of this License with
respect to the Work, or who has received express
permission from the Licensor to exercise rights under
this License despite a previous violation.
\item \textbf{``Publicly Perform''} means to perform
public recitations of the Work and to communicate to the
public those public recitations, by any means or process,
including by wire or wireless means or public digital
performances; to make available to the public Works in
such a way that members of the public may access these
Works from a place and at a place individually chosen by
them; to perform the Work to the public by any means or
process and the communication to the public of the
performances of the Work, including by public digital
performance; to broadcast and rebroadcast the Work by any
means including signs, sounds or images.
\item \textbf{``Reproduce''} means to make copies of
the Work by any means including without limitation by
sound or visual recordings and the right of fixation and
reproducing fixations of the Work, including storage of a
protected performance or phonogram in digital form or
other electronic medium.
\end{enumerate}
\par \textbf{2. Fair Dealing Rights.} Nothing in this
License is intended to reduce, limit, or restrict any uses
free from copyright or rights arising from limitations or
exceptions that are provided for in connection with the
copyright protection under copyright law or other
applicable laws.
\par \textbf{3. License Grant.} Subject to the terms
and conditions of this License, Licensor hereby grants You
a worldwide, royalty-free, non-exclusive, perpetual (for
the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:
\begin{enumerate}
\item to Reproduce the Work, to incorporate the Work into
one or more Collections, and to Reproduce the Work as
incorporated in the Collections;
\item to create and Reproduce Adaptations provided that any
such Adaptation, including any translation in any medium,
takes reasonable steps to clearly label, demarcate or
otherwise identify that changes were made to the original
Work. For example, a translation could be marked ``The
original work was translated from English to Spanish,'' or
a modification could indicate ``The original work has been
modified.'';
\item to Distribute and Publicly Perform the Work including
as incorporated in Collections; and,
\item to Distribute and Publicly Perform Adaptations.
\item 
\par For the avoidance of doubt:
\begin{enumerate}
\item \textbf{Non-waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme cannot be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License;
\item \textbf{Waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme can be waived, the
Licensor waives the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License; and,
\item \textbf{Voluntary License Schemes}. The
Licensor waives the right to collect royalties,
whether individually or, in the event that the
Licensor is a member of a collecting society that
administers voluntary licensing schemes, via that
society, from any exercise by You of the rights
granted under this License.
\end{enumerate}

\end{enumerate}
\par The above rights may be exercised in all media and
formats whether now known or hereafter devised. The above
rights include the right to make such modifications as are
technically necessary to exercise the rights in other media
and formats. Subject to Section 8(f), all rights not
expressly granted by Licensor are hereby reserved.
\par \textbf{4. Restrictions.} The license granted in
Section 3 above is expressly made subject to and limited by
the following restrictions:
\begin{enumerate}
\item You may Distribute or Publicly Perform the Work only
under the terms of this License. You must include a copy
of, or the Uniform Resource Identifier (URI) for, this
License with every copy of the Work You Distribute or
Publicly Perform. You may not offer or impose any terms
on the Work that restrict the terms of this License or
the ability of the recipient of the Work to exercise the
rights granted to that recipient under the terms of the
License. You may not sublicense the Work. You must keep
intact all notices that refer to this License and to the
disclaimer of warranties with every copy of the Work You
Distribute or Publicly Perform. When You Distribute or
Publicly Perform the Work, You may not impose any
effective technological measures on the Work that
restrict the ability of a recipient of the Work from You
to exercise the rights granted to that recipient under
the terms of the License. This Section 4(a) applies to
the Work as incorporated in a Collection, but this does
not require the Collection apart from the Work itself to
be made subject to the terms of this License. If You
create a Collection, upon notice from any Licensor You
must, to the extent practicable, remove from the
Collection any credit as required by Section 4(b), as
requested. If You create an Adaptation, upon notice from
any Licensor You must, to the extent practicable, remove
from the Adaptation any credit as required by Section
4(b), as requested.
\item If You Distribute, or Publicly Perform the Work or
any Adaptations or Collections, You must, unless a
request has been made pursuant to Section 4(a), keep
intact all copyright notices for the Work and provide,
reasonable to the medium or means You are utilizing: (i)
the name of the Original Author (or pseudonym, if
applicable) if supplied, and/or if the Original Author
and/or Licensor designate another party or parties (e.g.,
a sponsor institute, publishing entity, journal) for
attribution (``Attribution Parties'') in Licensor's
copyright notice, terms of service or by other reasonable
means, the name of such party or parties; (ii) the title
of the Work if supplied; (iii) to the extent reasonably
practicable, the URI, if any, that Licensor specifies to
be associated with the Work, unless such URI does not
refer to the copyright notice or licensing information
for the Work; and (iv) , consistent with Section 3(b), in
the case of an Adaptation, a credit identifying the use
of the Work in the Adaptation (e.g., ``French translation
of the Work by Original Author,'' or ``Screenplay based on
original Work by Original Author''). The credit required
by this Section 4 (b) may be implemented in any
reasonable manner; provided, however, that in the case of
a Adaptation or Collection, at a minimum such credit will
appear, if a credit for all contributing authors of the
Adaptation or Collection appears, then as part of these
credits and in a manner at least as prominent as the
credits for the other contributing authors. For the
avoidance of doubt, You may only use the credit required
by this Section for the purpose of attribution in the
manner set out above and, by exercising Your rights under
this License, You may not implicitly or explicitly assert
or imply any connection with, sponsorship or endorsement
by the Original Author, Licensor and/or Attribution
Parties, as appropriate, of You or Your use of the Work,
without the separate, express prior written permission of
the Original Author, Licensor and/or Attribution
Parties.
\item Except as otherwise agreed in writing by the Licensor
or as may be otherwise permitted by applicable law, if
You Reproduce, Distribute or Publicly Perform the Work
either by itself or as part of any Adaptations or
Collections, You must not distort, mutilate, modify or
take other derogatory action in relation to the Work
which would be prejudicial to the Original Author's honor
or reputation. Licensor agrees that in those
jurisdictions (e.g. Japan), in which any exercise of the
right granted in Section 3(b) of this License (the right
to make Adaptations) would be deemed to be a distortion,
mutilation, modification or other derogatory action
prejudicial to the Original Author's honor and
reputation, the Licensor will waive or not assert, as
appropriate, this Section, to the fullest extent
permitted by the applicable national law, to enable You
to reasonably exercise Your right under Section 3(b) of
this License (right to make Adaptations) but not
otherwise.
\end{enumerate}
\par \textbf{5. Representations, Warranties and
Disclaimer}
\par UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN
WRITING, LICENSOR OFFERS THE WORK AS-IS AND MAKES NO
REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING,
WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE
ABSENCE OF LATENT OR OTHER DEFECTS, ACCURACY, OR THE
PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT DISCOVERABLE.
SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.
\par \textbf{6. Limitation on Liability.} EXCEPT TO
THE EXTENT REQUIRED BY APPLICABLE LAW, IN NO EVENT WILL
LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR ANY
SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY
DAMAGES ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK,
EVEN IF LICENSOR HAS BEEN ADVISED OF THE POSSIBILITY OF
SUCH DAMAGES.
\par \textbf{7. Termination}
\begin{enumerate}
\item This License and the rights granted hereunder will
terminate automatically upon any breach by You of the
terms of this License. Individuals or entities who have
received Adaptations or Collections from You under this
License, however, will not have their licenses terminated
provided such individuals or entities remain in full
compliance with those licenses. Sections 1, 2, 5, 6, 7,
and 8 will survive any termination of this License.
\item Subject to the above terms and conditions, the
license granted here is perpetual (for the duration of
the applicable copyright in the Work). Notwithstanding
the above, Licensor reserves the right to release the
Work under different license terms or to stop
distributing the Work at any time; provided, however that
any such election will not serve to withdraw this License
(or any other license that has been, or is required to
be, granted under the terms of this License), and this
License will continue in full force and effect unless
terminated as stated above.
\end{enumerate}
\par \textbf{8. Miscellaneous}
\begin{enumerate}
\item Each time You Distribute or Publicly Perform the Work
or a Collection, the Licensor offers to the recipient a
license to the Work on the same terms and conditions as
the license granted to You under this License.
\item Each time You Distribute or Publicly Perform an
Adaptation, Licensor offers to the recipient a license to
the original Work on the same terms and conditions as the
license granted to You under this License.
\item If any provision of this License is invalid or
unenforceable under applicable law, it shall not affect
the validity or enforceability of the remainder of the
terms of this License, and without further action by the
parties to this agreement, such provision shall be
reformed to the minimum extent necessary to make such
provision valid and enforceable.
\item No term or provision of this License shall be deemed
waived and no breach consented to unless such waiver or
consent shall be in writing and signed by the party to be
charged with such waiver or consent.
\item This License constitutes the entire agreement between
the parties with respect to the Work licensed here. There
are no understandings, agreements or representations with
respect to the Work not specified here. Licensor shall
not be bound by any additional provisions that may appear
in any communication from You. This License may not be
modified without the mutual written agreement of the
Licensor and You.
\item The rights granted under, and the subject matter
referenced, in this License were drafted utilizing the
terminology of the Berne Convention for the Protection of
Literary and Artistic Works (as amended on September 28,
1979), the Rome Convention of 1961, the WIPO Copyright
Treaty of 1996, the WIPO Performances and Phonograms
Treaty of 1996 and the Universal Copyright Convention (as
revised on July 24, 1971). These rights and subject
matter take effect in the relevant jurisdiction in which
the License terms are sought to be enforced according to
the corresponding provisions of the implementation of
those treaty provisions in the applicable national law.
If the standard suite of rights granted under applicable
copyright law includes additional rights not granted
under this License, such additional rights are deemed to
be included in the License; this License is not intended
to restrict the license of any rights under applicable
law.
\end{enumerate}
 
\begin{quotation}
\subsubsection{Creative Commons Notice}
\par Creative Commons is not a party to this License, and
makes no warranty whatsoever in connection with the Work.
Creative Commons will not be liable to You or any party
on any legal theory for any damages whatsoever, including
without limitation any general, special, incidental or
consequential damages arising in connection to this
license. Notwithstanding the foregoing two (2) sentences,
if Creative Commons has expressly identified itself as
the Licensor hereunder, it shall have all rights and
obligations of Licensor.
\par Except for the limited purpose of indicating to the
public that the Work is licensed under the CCPL, Creative
Commons does not authorize the use by either party of the
trademark ``Creative Commons'' or any related trademark or
logo of Creative Commons without the prior written
consent of Creative Commons. Any permitted use will be in
compliance with Creative Commons' then-current trademark
usage guidelines, as may be published on its website or
otherwise made available upon request from time to time.
For the avoidance of doubt, this trademark restriction
does not form part of this License.
\par Creative Commons may be contacted at \url{https://creativecommons.org/}.
\end{quotation} 



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-3.0-plaintext.tex <==
Creative Commons Legal Code

Attribution 3.0 Unported

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR
    DAMAGES RESULTING FROM ITS USE.

License

THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS OF THIS CREATIVE
COMMONS PUBLIC LICENSE ("CCPL" OR "LICENSE"). THE WORK IS PROTECTED BY
COPYRIGHT AND/OR OTHER APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS PROHIBITED.

BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU ACCEPT AND AGREE
TO BE BOUND BY THE TERMS OF THIS LICENSE. TO THE EXTENT THIS LICENSE MAY
BE CONSIDERED TO BE A CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS
CONTAINED HERE IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.

1. Definitions

 a. "Adaptation" means a work based upon the Work, or upon the Work and
    other pre-existing works, such as a translation, adaptation,
    derivative work, arrangement of music or other alterations of a
    literary or artistic work, or phonogram or performance and includes
    cinematographic adaptations or any other form in which the Work may be
    recast, transformed, or adapted including in any form recognizably
    derived from the original, except that a work that constitutes a
    Collection will not be considered an Adaptation for the purpose of
    this License. For the avoidance of doubt, where the Work is a musical
    work, performance or phonogram, the synchronization of the Work in
    timed-relation with a moving image ("synching") will be considered an
    Adaptation for the purpose of this License.
 b. "Collection" means a collection of literary or artistic works, such as
    encyclopedias and anthologies, or performances, phonograms or
    broadcasts, or other works or subject matter other than works listed
    in Section 1(f) below, which, by reason of the selection and
    arrangement of their contents, constitute intellectual creations, in
    which the Work is included in its entirety in unmodified form along
    with one or more other contributions, each constituting separate and
    independent works in themselves, which together are assembled into a
    collective whole. A work that constitutes a Collection will not be
    considered an Adaptation (as defined above) for the purposes of this
    License.
 c. "Distribute" means to make available to the public the original and
    copies of the Work or Adaptation, as appropriate, through sale or
    other transfer of ownership.
 d. "Licensor" means the individual, individuals, entity or entities that
    offer(s) the Work under the terms of this License.
 e. "Original Author" means, in the case of a literary or artistic work,
    the individual, individuals, entity or entities who created the Work
    or if no individual or entity can be identified, the publisher; and in
    addition (i) in the case of a performance the actors, singers,
    musicians, dancers, and other persons who act, sing, deliver, declaim,
    play in, interpret or otherwise perform literary or artistic works or
    expressions of folklore; (ii) in the case of a phonogram the producer
    being the person or legal entity who first fixes the sounds of a
    performance or other sounds; and, (iii) in the case of broadcasts, the
    organization that transmits the broadcast.
 f. "Work" means the literary and/or artistic work offered under the terms
    of this License including without limitation any production in the
    literary, scientific and artistic domain, whatever may be the mode or
    form of its expression including digital form, such as a book,
    pamphlet and other writing; a lecture, address, sermon or other work
    of the same nature; a dramatic or dramatico-musical work; a
    choreographic work or entertainment in dumb show; a musical
    composition with or without words; a cinematographic work to which are
    assimilated works expressed by a process analogous to cinematography;
    a work of drawing, painting, architecture, sculpture, engraving or
    lithography; a photographic work to which are assimilated works
    expressed by a process analogous to photography; a work of applied
    art; an illustration, map, plan, sketch or three-dimensional work
    relative to geography, topography, architecture or science; a
    performance; a broadcast; a phonogram; a compilation of data to the
    extent it is protected as a copyrightable work; or a work performed by
    a variety or circus performer to the extent it is not otherwise
    considered a literary or artistic work.
 g. "You" means an individual or entity exercising rights under this
    License who has not previously violated the terms of this License with
    respect to the Work, or who has received express permission from the
    Licensor to exercise rights under this License despite a previous
    violation.
 h. "Publicly Perform" means to perform public recitations of the Work and
    to communicate to the public those public recitations, by any means or
    process, including by wire or wireless means or public digital
    performances; to make available to the public Works in such a way that
    members of the public may access these Works from a place and at a
    place individually chosen by them; to perform the Work to the public
    by any means or process and the communication to the public of the
    performances of the Work, including by public digital performance; to
    broadcast and rebroadcast the Work by any means including signs,
    sounds or images.
 i. "Reproduce" means to make copies of the Work by any means including
    without limitation by sound or visual recordings and the right of
    fixation and reproducing fixations of the Work, including storage of a
    protected performance or phonogram in digital form or other electronic
    medium.

2. Fair Dealing Rights. Nothing in this License is intended to reduce,
limit, or restrict any uses free from copyright or rights arising from
limitations or exceptions that are provided for in connection with the
copyright protection under copyright law or other applicable laws.

3. License Grant. Subject to the terms and conditions of this License,
Licensor hereby grants You a worldwide, royalty-free, non-exclusive,
perpetual (for the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:

 a. to Reproduce the Work, to incorporate the Work into one or more
    Collections, and to Reproduce the Work as incorporated in the
    Collections;
 b. to create and Reproduce Adaptations provided that any such Adaptation,
    including any translation in any medium, takes reasonable steps to
    clearly label, demarcate or otherwise identify that changes were made
    to the original Work. For example, a translation could be marked "The
    original work was translated from English to Spanish," or a
    modification could indicate "The original work has been modified.";
 c. to Distribute and Publicly Perform the Work including as incorporated
    in Collections; and,
 d. to Distribute and Publicly Perform Adaptations.
 e. For the avoidance of doubt:

     i. Non-waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme cannot be waived, the Licensor
        reserves the exclusive right to collect such royalties for any
        exercise by You of the rights granted under this License;
    ii. Waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme can be waived, the Licensor waives the
        exclusive right to collect such royalties for any exercise by You
        of the rights granted under this License; and,
   iii. Voluntary License Schemes. The Licensor waives the right to
        collect royalties, whether individually or, in the event that the
        Licensor is a member of a collecting society that administers
        voluntary licensing schemes, via that society, from any exercise
        by You of the rights granted under this License.

The above rights may be exercised in all media and formats whether now
known or hereafter devised. The above rights include the right to make
such modifications as are technically necessary to exercise the rights in
other media and formats. Subject to Section 8(f), all rights not expressly
granted by Licensor are hereby reserved.

4. Restrictions. The license granted in Section 3 above is expressly made
subject to and limited by the following restrictions:

 a. You may Distribute or Publicly Perform the Work only under the terms
    of this License. You must include a copy of, or the Uniform Resource
    Identifier (URI) for, this License with every copy of the Work You
    Distribute or Publicly Perform. You may not offer or impose any terms
    on the Work that restrict the terms of this License or the ability of
    the recipient of the Work to exercise the rights granted to that
    recipient under the terms of the License. You may not sublicense the
    Work. You must keep intact all notices that refer to this License and
    to the disclaimer of warranties with every copy of the Work You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Work, You may not impose any effective technological
    measures on the Work that restrict the ability of a recipient of the
    Work from You to exercise the rights granted to that recipient under
    the terms of the License. This Section 4(a) applies to the Work as
    incorporated in a Collection, but this does not require the Collection
    apart from the Work itself to be made subject to the terms of this
    License. If You create a Collection, upon notice from any Licensor You
    must, to the extent practicable, remove from the Collection any credit
    as required by Section 4(b), as requested. If You create an
    Adaptation, upon notice from any Licensor You must, to the extent
    practicable, remove from the Adaptation any credit as required by
    Section 4(b), as requested.
 b. If You Distribute, or Publicly Perform the Work or any Adaptations or
    Collections, You must, unless a request has been made pursuant to
    Section 4(a), keep intact all copyright notices for the Work and
    provide, reasonable to the medium or means You are utilizing: (i) the
    name of the Original Author (or pseudonym, if applicable) if supplied,
    and/or if the Original Author and/or Licensor designate another party
    or parties (e.g., a sponsor institute, publishing entity, journal) for
    attribution ("Attribution Parties") in Licensor's copyright notice,
    terms of service or by other reasonable means, the name of such party
    or parties; (ii) the title of the Work if supplied; (iii) to the
    extent reasonably practicable, the URI, if any, that Licensor
    specifies to be associated with the Work, unless such URI does not
    refer to the copyright notice or licensing information for the Work;
    and (iv) , consistent with Section 3(b), in the case of an Adaptation,
    a credit identifying the use of the Work in the Adaptation (e.g.,
    "French translation of the Work by Original Author," or "Screenplay
    based on original Work by Original Author"). The credit required by
    this Section 4 (b) may be implemented in any reasonable manner;
    provided, however, that in the case of a Adaptation or Collection, at
    a minimum such credit will appear, if a credit for all contributing
    authors of the Adaptation or Collection appears, then as part of these
    credits and in a manner at least as prominent as the credits for the
    other contributing authors. For the avoidance of doubt, You may only
    use the credit required by this Section for the purpose of attribution
    in the manner set out above and, by exercising Your rights under this
    License, You may not implicitly or explicitly assert or imply any
    connection with, sponsorship or endorsement by the Original Author,
    Licensor and/or Attribution Parties, as appropriate, of You or Your
    use of the Work, without the separate, express prior written
    permission of the Original Author, Licensor and/or Attribution
    Parties.
 c. Except as otherwise agreed in writing by the Licensor or as may be
    otherwise permitted by applicable law, if You Reproduce, Distribute or
    Publicly Perform the Work either by itself or as part of any
    Adaptations or Collections, You must not distort, mutilate, modify or
    take other derogatory action in relation to the Work which would be
    prejudicial to the Original Author's honor or reputation. Licensor
    agrees that in those jurisdictions (e.g. Japan), in which any exercise
    of the right granted in Section 3(b) of this License (the right to
    make Adaptations) would be deemed to be a distortion, mutilation,
    modification or other derogatory action prejudicial to the Original
    Author's honor and reputation, the Licensor will waive or not assert,
    as appropriate, this Section, to the fullest extent permitted by the
    applicable national law, to enable You to reasonably exercise Your
    right under Section 3(b) of this License (right to make Adaptations)
    but not otherwise.

5. Representations, Warranties and Disclaimer

UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN WRITING, LICENSOR
OFFERS THE WORK AS-IS AND MAKES NO REPRESENTATIONS OR WARRANTIES OF ANY
KIND CONCERNING THE WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE,
INCLUDING, WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE ABSENCE OF
LATENT OR OTHER DEFECTS, ACCURACY, OR THE PRESENCE OF ABSENCE OF ERRORS,
WHETHER OR NOT DISCOVERABLE. SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION
OF IMPLIED WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.

6. Limitation on Liability. EXCEPT TO THE EXTENT REQUIRED BY APPLICABLE
LAW, IN NO EVENT WILL LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR
ANY SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY DAMAGES
ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK, EVEN IF LICENSOR HAS
BEEN ADVISED OF THE POSSIBILITY OF SUCH DAMAGES.

7. Termination

 a. This License and the rights granted hereunder will terminate
    automatically upon any breach by You of the terms of this License.
    Individuals or entities who have received Adaptations or Collections
    from You under this License, however, will not have their licenses
    terminated provided such individuals or entities remain in full
    compliance with those licenses. Sections 1, 2, 5, 6, 7, and 8 will
    survive any termination of this License.
 b. Subject to the above terms and conditions, the license granted here is
    perpetual (for the duration of the applicable copyright in the Work).
    Notwithstanding the above, Licensor reserves the right to release the
    Work under different license terms or to stop distributing the Work at
    any time; provided, however that any such election will not serve to
    withdraw this License (or any other license that has been, or is
    required to be, granted under the terms of this License), and this
    License will continue in full force and effect unless terminated as
    stated above.

8. Miscellaneous

 a. Each time You Distribute or Publicly Perform the Work or a Collection,
    the Licensor offers to the recipient a license to the Work on the same
    terms and conditions as the license granted to You under this License.
 b. Each time You Distribute or Publicly Perform an Adaptation, Licensor
    offers to the recipient a license to the original Work on the same
    terms and conditions as the license granted to You under this License.
 c. If any provision of this License is invalid or unenforceable under
    applicable law, it shall not affect the validity or enforceability of
    the remainder of the terms of this License, and without further action
    by the parties to this agreement, such provision shall be reformed to
    the minimum extent necessary to make such provision valid and
    enforceable.
 d. No term or provision of this License shall be deemed waived and no
    breach consented to unless such waiver or consent shall be in writing
    and signed by the party to be charged with such waiver or consent.
 e. This License constitutes the entire agreement between the parties with
    respect to the Work licensed here. There are no understandings,
    agreements or representations with respect to the Work not specified
    here. Licensor shall not be bound by any additional provisions that
    may appear in any communication from You. This License may not be
    modified without the mutual written agreement of the Licensor and You.
 f. The rights granted under, and the subject matter referenced, in this
    License were drafted utilizing the terminology of the Berne Convention
    for the Protection of Literary and Artistic Works (as amended on
    September 28, 1979), the Rome Convention of 1961, the WIPO Copyright
    Treaty of 1996, the WIPO Performances and Phonograms Treaty of 1996
    and the Universal Copyright Convention (as revised on July 24, 1971).
    These rights and subject matter take effect in the relevant
    jurisdiction in which the License terms are sought to be enforced
    according to the corresponding provisions of the implementation of
    those treaty provisions in the applicable national law. If the
    standard suite of rights granted under applicable copyright law
    includes additional rights not granted under this License, such
    additional rights are deemed to be included in the License; this
    License is not intended to restrict the license of any rights under
    applicable law.


Creative Commons Notice

    Creative Commons is not a party to this License, and makes no warranty
    whatsoever in connection with the Work. Creative Commons will not be
    liable to You or any party on any legal theory for any damages
    whatsoever, including without limitation any general, special,
    incidental or consequential damages arising in connection to this
    license. Notwithstanding the foregoing two (2) sentences, if Creative
    Commons has expressly identified itself as the Licensor hereunder, it
    shall have all rights and obligations of Licensor.

    Except for the limited purpose of indicating to the public that the
    Work is licensed under the CCPL, Creative Commons does not authorize
    the use by either party of the trademark "Creative Commons" or any
    related trademark or logo of Creative Commons without the prior
    written consent of Creative Commons. Any permitted use will be in
    compliance with Creative Commons' then-current trademark usage
    guidelines, as may be published on its website or otherwise made
    available upon request from time to time. For the avoidance of doubt,
    this trademark restriction does not form part of this License.

    Creative Commons may be contacted at https://creativecommons.org/.


==> license-texts/doclicense-CC-by-4.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution 4.0 International}







Official translations of this license are available in other languages.



\par Creative Commons Corporation (“Creative Commons”) is not a law firm and does not provide legal services or legal advice. Distribution of Creative Commons public licenses does not create a lawyer-client or other relationship. Creative Commons makes its licenses and related information available on an “as-is” basis. Creative Commons gives no warranties regarding its licenses, any material licensed under their terms and conditions, or any related information. Creative Commons disclaims all liability for damages resulting from their use to the fullest extent possible.


\par \textbf{Using Creative Commons Public Licenses}
\par Creative Commons public licenses provide a standard set of terms and conditions that creators and other rights holders may use to share original works of authorship and other material subject to copyright and certain other rights specified in the public license below. The following considerations are for informational purposes only, are not exhaustive, and do not form part of our licenses.
\begin{quotation}\textbf{Considerations for licensors:} Our public licenses are intended for use by those authorized to give the public permission to use material in ways otherwise restricted by copyright and certain other rights. Our licenses are irrevocable. Licensors should read and understand the terms and conditions of the license they choose before applying it. Licensors should also secure all rights necessary before applying our licenses so that the public can reuse the material as expected. Licensors should clearly mark any material not subject to the license. This includes other CC-licensed material, or material used under an exception or limitation to copyright. More considerations for licensors.\end{quotation}
\begin{quotation}\textbf{Considerations for the public:} By using one of our public licenses, a licensor grants the public permission to use the licensed material under specified terms and conditions. If the licensor’s permission is not necessary for any reason–for example, because of any applicable exception or limitation to copyright–then that use is not regulated by the license. Our licenses grant only permissions under copyright and certain other rights that a licensor has authority to grant. Use of the licensed material may still be restricted for other reasons, including because others have copyright or other rights in the material. A licensor may make special requests, such as asking that all changes be marked or described. Although not required by our licenses, you are encouraged to respect those requests where reasonable.
More considerations for the public.\end{quotation}

\subsubsection{Creative Commons Attribution 4.0 International Public License}
\par By exercising the Licensed Rights (defined below), You accept and agree to be bound by the terms and conditions of this Creative Commons Attribution 4.0 International Public License (``Public License''). To the extent this Public License may be interpreted as a contract, You are granted the Licensed Rights in consideration of Your acceptance of these terms and conditions, and the Licensor grants You such rights in consideration of benefits the Licensor receives from making the Licensed Material available under these terms and conditions.
\par \textbf{Section 1 – Definitions.}
\begin{enumerate}
\item \textbf{Adapted Material} means material subject to Copyright and Similar Rights that is derived from or based upon the Licensed Material and in which the Licensed Material is translated, altered, arranged, transformed, or otherwise modified in a manner requiring permission under the Copyright and Similar Rights held by the Licensor. For purposes of this Public License, where the Licensed Material is a musical work, performance, or sound recording, Adapted Material is always produced where the Licensed Material is synched in timed relation with a moving image.
\item \textbf{Adapter's License} means the license You apply to Your Copyright and Similar Rights in Your contributions to Adapted Material in accordance with the terms and conditions of this Public License.
\item \textbf{Copyright and Similar Rights} means copyright and/or similar rights closely related to copyright including, without limitation, performance, broadcast, sound recording, and Sui Generis Database Rights, without regard to how the rights are labeled or categorized. For purposes of this Public License, the rights specified in Section 2(b)(1)-(2) are not Copyright and Similar Rights.
\item \textbf{Effective Technological Measures} means those measures that, in the absence of proper authority, may not
be circumvented under laws fulfilling obligations under Article 11 of the WIPO Copyright Treaty adopted on December 20, 1996, and/or similar
international agreements.
\item \textbf{Exceptions and Limitations} means fair use, fair dealing, and/or any other exception or limitation to Copyright and Similar Rights that applies to Your use of the Licensed Material.
\item \textbf{Licensed Material} means the artistic or literary work, database, or other material to which the Licensor applied this Public License.
\item \textbf{Licensed Rights} means the rights granted to You subject to the terms and conditions of this Public License, which are limited to all Copyright and Similar Rights that apply to Your use of the Licensed Material and that the Licensor has authority to license.
\item \textbf{Licensor} means the individual(s) or entity(ies) granting rights under this Public License.
\item \textbf{Share} means to provide material to the public by any means or process that requires permission under the Licensed Rights, such as reproduction, public display, public performance, distribution, dissemination, communication, or importation, and to make material available to the public including in ways that members of the public may access the material from a place and at a time individually chosen by them.
\item \textbf{Sui Generis Database Rights} means rights other than copyright resulting from Directive 96/9/EC of the European Parliament and of the Council of 11 March 1996 on the legal protection of databases, as amended and/or succeeded, as well as other essentially equivalent rights anywhere in the world.
\item \textbf{You} means the individual or entity exercising the Licensed Rights under this Public License. \textbf{Your} has a corresponding meaning.
\end{enumerate}
\par \textbf{Section 2 – Scope.}
\begin{enumerate}
\item \textbf{License grant}.
\begin{enumerate}
\item Subject to the terms and conditions of this Public License, the Licensor hereby grants You a worldwide, royalty-free, non-sublicensable, non-exclusive, irrevocable license to exercise the Licensed Rights in the Licensed Material to:
\begin{enumerate}
\item reproduce and Share the Licensed Material, in whole or in part; and
\item produce, reproduce, and Share Adapted Material.
\end{enumerate}
\item Exceptions and Limitations. For the avoidance of doubt, where Exceptions and Limitations apply to Your use, this Public License does not apply, and You do not need to comply with its terms and conditions.
\item Term. The term of this Public License is specified in Section 6(a).
\item Media and formats; technical modifications allowed. The Licensor authorizes You to exercise the Licensed Rights in all media and formats whether now known or hereafter created, and to make technical modifications necessary to do so. The Licensor waives and/or agrees not to assert any right or authority to forbid You from making technical modifications necessary to exercise the Licensed Rights, including technical modifications necessary to circumvent Effective Technological Measures. For purposes of this Public License, simply making modifications authorized by this Section 2(a)(4) never produces Adapted Material.
\item Downstream recipients.

\begin{enumerate}
\item Offer from the Licensor – Licensed Material. Every recipient of the Licensed Material automatically receives an offer from the Licensor to exercise the Licensed Rights under the terms and conditions of this Public License.
\item No downstream restrictions. You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, the Licensed Material if doing so restricts exercise of the Licensed Rights by any recipient of the Licensed Material.
\end{enumerate}

\item No endorsement. Nothing in this Public License constitutes or may be construed as permission to assert or imply that You are, or that Your use of the Licensed Material is, connected with, or sponsored, endorsed, or granted official status by, the Licensor or others designated to receive attribution as provided in Section 3(a)(1)(A)(i).
\end{enumerate}
\item \par \textbf{Other rights}.
\begin{enumerate}
\item Moral rights, such as the right of integrity, are not licensed under this Public License, nor are publicity, privacy, and/or other similar personality rights; however, to the extent possible, the Licensor waives and/or agrees not to assert any such rights held by the Licensor to the limited extent necessary to allow You to exercise the Licensed Rights, but not otherwise.
\item Patent and trademark rights are not licensed under this Public License.
\item To the extent possible, the Licensor waives any right to collect royalties from You for the exercise of the Licensed Rights, whether directly or through a collecting society under any voluntary or waivable statutory or compulsory licensing scheme. In all other cases the Licensor expressly reserves any right to collect such royalties.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 3 – License Conditions.}
\par Your exercise of the Licensed Rights is expressly made subject to the following conditions.
\begin{enumerate}
\item \par \textbf{Attribution}.
\begin{enumerate}
\item \par If You Share the Licensed Material (including in modified form), You must:
\begin{enumerate}
\item retain the following if it is supplied by the Licensor with the Licensed Material:
\begin{enumerate}
\item identification of the creator(s) of the Licensed Material and any others designated to receive attribution, in any reasonable manner requested by the Licensor (including by pseudonym if designated);
\item a copyright notice;
\item a notice that refers to this Public License; 
\item a notice that refers to the disclaimer of warranties;
\item a URI or hyperlink to the Licensed Material to the extent reasonably practicable;
\end{enumerate}
\item indicate if You modified the Licensed Material and retain an indication of any previous modifications; and
\item indicate the Licensed Material is licensed under this Public License,
and include the text of, or the URI or hyperlink to, this Public
License.
\end{enumerate}

\item You may satisfy the conditions in Section 3(a)(1) in any reasonable manner based on the medium, means, and context in which You Share the Licensed Material. For example, it may be reasonable to satisfy the conditions by providing a URI or hyperlink to a resource that includes the required information.
\item If requested by the Licensor, You must remove any of the information required by Section 3(a)(1)(A) to the extent reasonably practicable.
\item If You Share Adapted Material You produce, the Adapter's License You apply must not prevent recipients of the Adapted Material from complying with this Public License.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 4 – Sui Generis Database Rights.}
\par Where the Licensed Rights include Sui Generis Database Rights that apply to Your use of the Licensed Material:
\begin{enumerate}
\item for the avoidance of doubt, Section 2(a)(1) grants You the right to extract, reuse, reproduce, and Share all or a substantial portion of the contents of the database;
\item if You include all or a substantial portion of the database contents in a database in which You have Sui Generis Database Rights, then the database in which You have Sui Generis Database Rights (but not its individual contents) is Adapted Material; and
\item You must comply with the conditions in Section 3(a) if You Share all or a substantial portion of the contents of the database.
\end{enumerate}
For the avoidance of doubt, this Section 4 supplements and does not replace Your obligations under this Public License where the Licensed Rights include other Copyright and Similar Rights.
\par \textbf{Section 5 – Disclaimer of Warranties and Limitation of Liability.}
\begin{enumerate}
\item \textbf{Unless otherwise separately undertaken by the Licensor, to the extent possible, the Licensor offers the Licensed Material as-is and as-available, and makes no representations or warranties of any kind concerning the Licensed Material, whether express, implied, statutory, or other. This includes, without limitation, warranties of title, merchantability, fitness for a particular purpose, non-infringement, absence of latent or other defects, accuracy, or the presence or absence of errors, whether or not known or discoverable. Where disclaimers of warranties are not allowed in full or in part, this disclaimer may not apply to You.}
\item \textbf{To the extent possible, in no event will the Licensor be liable to You on any legal theory (including, without limitation, negligence) or otherwise for any direct, special, indirect, incidental, consequential, punitive, exemplary, or other losses, costs, expenses, or damages arising out of this Public License or use of the Licensed Material, even if the Licensor has been advised of the possibility of such losses, costs, expenses, or damages. Where a limitation of liability is not allowed in full or in part, this limitation may not apply to You.}
\end{enumerate}
\begin{enumerate}
\item The disclaimer of warranties and limitation of liability provided above shall be interpreted in a manner that, to the extent possible, most closely approximates an absolute disclaimer and waiver of all liability.
\end{enumerate}
\par \textbf{Section 6 – Term and Termination.}
\begin{enumerate}
\item This Public License applies for the term of the Copyright and Similar Rights licensed here. However, if You fail to comply with this Public License, then Your rights under this Public License terminate automatically.
\item 
\par Where Your right to use the Licensed Material has terminated under Section 6(a), it reinstates:
\begin{enumerate}
\item automatically as of the date the violation is cured, provided it is cured within 30 days of Your discovery of the violation; or
\item upon express reinstatement by the Licensor.
\end{enumerate}
For the avoidance of doubt, this Section 6(b) does not affect any right the Licensor may have to seek remedies for Your violations of this Public License.
\item For the avoidance of doubt, the Licensor may also offer the Licensed Material under separate terms or conditions or stop distributing the Licensed Material at any time; however, doing so will not terminate this Public License.
\item Sections 1, 5, 6, 7, and 8 survive termination of this Public License.
\end{enumerate}
\par \textbf{Section 7 – Other Terms and Conditions.}
\begin{enumerate}
\item The Licensor shall not be bound by any additional or different terms or conditions communicated by You unless expressly agreed.
\item Any arrangements, understandings, or agreements regarding the Licensed Material not stated herein are separate from and independent of the terms and conditions of this Public License.
\end{enumerate}
\par \textbf{Section 8 – Interpretation.}
\begin{enumerate}
\item For the avoidance of doubt, this Public License does not, and shall not be interpreted to, reduce, limit, restrict, or impose conditions on any use of the Licensed Material that could lawfully be made without permission under this Public License.
\item To the extent possible, if any provision of this Public License is deemed unenforceable, it shall be automatically reformed to the minimum extent necessary to make it enforceable. If the provision cannot be reformed, it shall be severed from this Public License without affecting the enforceability of the remaining terms and conditions.
\item No term or condition of this Public License will be waived and no failure to comply consented to unless expressly agreed to by the Licensor.
\item Nothing in this Public License constitutes or may be interpreted as a limitation upon, or waiver of, any privileges and immunities that apply to the Licensor or You, including from the legal processes of any jurisdiction or authority.
\end{enumerate}
\par Creative Commons is not a party to its public licenses. Notwithstanding, Creative Commons may elect to apply one of its public licenses to material it publishes and in those instances will be considered the “Licensor.” The text of the Creative Commons public licenses is dedicated to the public domain under the CC0 Public Domain Dedication. Except for the limited purpose of indicating that material is shared under a Creative Commons public license or as otherwise permitted by the Creative Commons policies published at creativecommons.org/policies, Creative Commons does not authorize the use of the trademark “Creative Commons” or any other trademark or logo of Creative Commons without its prior written consent including, without limitation, in connection with any unauthorized modifications to any of its public licenses or any other arrangements, understandings, or agreements concerning use of licensed material. For the avoidance of doubt, this paragraph does not form part of the public licenses.\\\\
Creative Commons may be contacted at creativecommons.org.
\par Additional languages available: Bahasa Indonesia, Nederlands, norsk, suomeksi, te reo Māori, українська, 日本語. Please read the FAQ for more information about official translations. 



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-4.0-plaintext.tex <==
Attribution 4.0 International

=======================================================================

Creative Commons Corporation ("Creative Commons") is not a law firm and
does not provide legal services or legal advice. Distribution of
Creative Commons public licenses does not create a lawyer-client or
other relationship. Creative Commons makes its licenses and related
information available on an "as-is" basis. Creative Commons gives no
warranties regarding its licenses, any material licensed under their
terms and conditions, or any related information. Creative Commons
disclaims all liability for damages resulting from their use to the
fullest extent possible.

Using Creative Commons Public Licenses

Creative Commons public licenses provide a standard set of terms and
conditions that creators and other rights holders may use to share
original works of authorship and other material subject to copyright
and certain other rights specified in the public license below. The
following considerations are for informational purposes only, are not
exhaustive, and do not form part of our licenses.

     Considerations for licensors: Our public licenses are
     intended for use by those authorized to give the public
     permission to use material in ways otherwise restricted by
     copyright and certain other rights. Our licenses are
     irrevocable. Licensors should read and understand the terms
     and conditions of the license they choose before applying it.
     Licensors should also secure all rights necessary before
     applying our licenses so that the public can reuse the
     material as expected. Licensors should clearly mark any
     material not subject to the license. This includes other CC-
     licensed material, or material used under an exception or
     limitation to copyright. More considerations for licensors:
	wiki.creativecommons.org/Considerations_for_licensors

     Considerations for the public: By using one of our public
     licenses, a licensor grants the public permission to use the
     licensed material under specified terms and conditions. If
     the licensor's permission is not necessary for any reason--for
     example, because of any applicable exception or limitation to
     copyright--then that use is not regulated by the license. Our
     licenses grant only permissions under copyright and certain
     other rights that a licensor has authority to grant. Use of
     the licensed material may still be restricted for other
     reasons, including because others have copyright or other
     rights in the material. A licensor may make special requests,
     such as asking that all changes be marked or described.
     Although not required by our licenses, you are encouraged to
     respect those requests where reasonable. More_considerations
     for the public: 
	wiki.creativecommons.org/Considerations_for_licensees

=======================================================================

Creative Commons Attribution 4.0 International Public License

By exercising the Licensed Rights (defined below), You accept and agree
to be bound by the terms and conditions of this Creative Commons
Attribution 4.0 International Public License ("Public License"). To the
extent this Public License may be interpreted as a contract, You are
granted the Licensed Rights in consideration of Your acceptance of
these terms and conditions, and the Licensor grants You such rights in
consideration of benefits the Licensor receives from making the
Licensed Material available under these terms and conditions.


Section 1 -- Definitions.

  a. Adapted Material means material subject to Copyright and Similar
     Rights that is derived from or based upon the Licensed Material
     and in which the Licensed Material is translated, altered,
     arranged, transformed, or otherwise modified in a manner requiring
     permission under the Copyright and Similar Rights held by the
     Licensor. For purposes of this Public License, where the Licensed
     Material is a musical work, performance, or sound recording,
     Adapted Material is always produced where the Licensed Material is
     synched in timed relation with a moving image.

  b. Adapter's License means the license You apply to Your Copyright
     and Similar Rights in Your contributions to Adapted Material in
     accordance with the terms and conditions of this Public License.

  c. Copyright and Similar Rights means copyright and/or similar rights
     closely related to copyright including, without limitation,
     performance, broadcast, sound recording, and Sui Generis Database
     Rights, without regard to how the rights are labeled or
     categorized. For purposes of this Public License, the rights
     specified in Section 2(b)(1)-(2) are not Copyright and Similar
     Rights.

  d. Effective Technological Measures means those measures that, in the
     absence of proper authority, may not be circumvented under laws
     fulfilling obligations under Article 11 of the WIPO Copyright
     Treaty adopted on December 20, 1996, and/or similar international
     agreements.

  e. Exceptions and Limitations means fair use, fair dealing, and/or
     any other exception or limitation to Copyright and Similar Rights
     that applies to Your use of the Licensed Material.

  f. Licensed Material means the artistic or literary work, database,
     or other material to which the Licensor applied this Public
     License.

  g. Licensed Rights means the rights granted to You subject to the
     terms and conditions of this Public License, which are limited to
     all Copyright and Similar Rights that apply to Your use of the
     Licensed Material and that the Licensor has authority to license.

  h. Licensor means the individual(s) or entity(ies) granting rights
     under this Public License.

  i. Share means to provide material to the public by any means or
     process that requires permission under the Licensed Rights, such
     as reproduction, public display, public performance, distribution,
     dissemination, communication, or importation, and to make material
     available to the public including in ways that members of the
     public may access the material from a place and at a time
     individually chosen by them.

  j. Sui Generis Database Rights means rights other than copyright
     resulting from Directive 96/9/EC of the European Parliament and of
     the Council of 11 March 1996 on the legal protection of databases,
     as amended and/or succeeded, as well as other essentially
     equivalent rights anywhere in the world.

  k. You means the individual or entity exercising the Licensed Rights
     under this Public License. Your has a corresponding meaning.


Section 2 -- Scope.

  a. License grant.

       1. Subject to the terms and conditions of this Public License,
          the Licensor hereby grants You a worldwide, royalty-free,
          non-sublicensable, non-exclusive, irrevocable license to
          exercise the Licensed Rights in the Licensed Material to:

            a. reproduce and Share the Licensed Material, in whole or
               in part; and

            b. produce, reproduce, and Share Adapted Material.

       2. Exceptions and Limitations. For the avoidance of doubt, where
          Exceptions and Limitations apply to Your use, this Public
          License does not apply, and You do not need to comply with
          its terms and conditions.

       3. Term. The term of this Public License is specified in Section
          6(a).

       4. Media and formats; technical modifications allowed. The
          Licensor authorizes You to exercise the Licensed Rights in
          all media and formats whether now known or hereafter created,
          and to make technical modifications necessary to do so. The
          Licensor waives and/or agrees not to assert any right or
          authority to forbid You from making technical modifications
          necessary to exercise the Licensed Rights, including
          technical modifications necessary to circumvent Effective
          Technological Measures. For purposes of this Public License,
          simply making modifications authorized by this Section 2(a)
          (4) never produces Adapted Material.

       5. Downstream recipients.

            a. Offer from the Licensor -- Licensed Material. Every
               recipient of the Licensed Material automatically
               receives an offer from the Licensor to exercise the
               Licensed Rights under the terms and conditions of this
               Public License.

            b. No downstream restrictions. You may not offer or impose
               any additional or different terms or conditions on, or
               apply any Effective Technological Measures to, the
               Licensed Material if doing so restricts exercise of the
               Licensed Rights by any recipient of the Licensed
               Material.

       6. No endorsement. Nothing in this Public License constitutes or
          may be construed as permission to assert or imply that You
          are, or that Your use of the Licensed Material is, connected
          with, or sponsored, endorsed, or granted official status by,
          the Licensor or others designated to receive attribution as
          provided in Section 3(a)(1)(A)(i).

  b. Other rights.

       1. Moral rights, such as the right of integrity, are not
          licensed under this Public License, nor are publicity,
          privacy, and/or other similar personality rights; however, to
          the extent possible, the Licensor waives and/or agrees not to
          assert any such rights held by the Licensor to the limited
          extent necessary to allow You to exercise the Licensed
          Rights, but not otherwise.

       2. Patent and trademark rights are not licensed under this
          Public License.

       3. To the extent possible, the Licensor waives any right to
          collect royalties from You for the exercise of the Licensed
          Rights, whether directly or through a collecting society
          under any voluntary or waivable statutory or compulsory
          licensing scheme. In all other cases the Licensor expressly
          reserves any right to collect such royalties.


Section 3 -- License Conditions.

Your exercise of the Licensed Rights is expressly made subject to the
following conditions.

  a. Attribution.

       1. If You Share the Licensed Material (including in modified
          form), You must:

            a. retain the following if it is supplied by the Licensor
               with the Licensed Material:

                 i. identification of the creator(s) of the Licensed
                    Material and any others designated to receive
                    attribution, in any reasonable manner requested by
                    the Licensor (including by pseudonym if
                    designated);

                ii. a copyright notice;

               iii. a notice that refers to this Public License;

                iv. a notice that refers to the disclaimer of
                    warranties;

                 v. a URI or hyperlink to the Licensed Material to the
                    extent reasonably practicable;

            b. indicate if You modified the Licensed Material and
               retain an indication of any previous modifications; and

            c. indicate the Licensed Material is licensed under this
               Public License, and include the text of, or the URI or
               hyperlink to, this Public License.

       2. You may satisfy the conditions in Section 3(a)(1) in any
          reasonable manner based on the medium, means, and context in
          which You Share the Licensed Material. For example, it may be
          reasonable to satisfy the conditions by providing a URI or
          hyperlink to a resource that includes the required
          information.

       3. If requested by the Licensor, You must remove any of the
          information required by Section 3(a)(1)(A) to the extent
          reasonably practicable.

       4. If You Share Adapted Material You produce, the Adapter's
          License You apply must not prevent recipients of the Adapted
          Material from complying with this Public License.


Section 4 -- Sui Generis Database Rights.

Where the Licensed Rights include Sui Generis Database Rights that
apply to Your use of the Licensed Material:

  a. for the avoidance of doubt, Section 2(a)(1) grants You the right
     to extract, reuse, reproduce, and Share all or a substantial
     portion of the contents of the database;

  b. if You include all or a substantial portion of the database
     contents in a database in which You have Sui Generis Database
     Rights, then the database in which You have Sui Generis Database
     Rights (but not its individual contents) is Adapted Material; and

  c. You must comply with the conditions in Section 3(a) if You Share
     all or a substantial portion of the contents of the database.

For the avoidance of doubt, this Section 4 supplements and does not
replace Your obligations under this Public License where the Licensed
Rights include other Copyright and Similar Rights.


Section 5 -- Disclaimer of Warranties and Limitation of Liability.

  a. UNLESS OTHERWISE SEPARATELY UNDERTAKEN BY THE LICENSOR, TO THE
     EXTENT POSSIBLE, THE LICENSOR OFFERS THE LICENSED MATERIAL AS-IS
     AND AS-AVAILABLE, AND MAKES NO REPRESENTATIONS OR WARRANTIES OF
     ANY KIND CONCERNING THE LICENSED MATERIAL, WHETHER EXPRESS,
     IMPLIED, STATUTORY, OR OTHER. THIS INCLUDES, WITHOUT LIMITATION,
     WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
     PURPOSE, NON-INFRINGEMENT, ABSENCE OF LATENT OR OTHER DEFECTS,
     ACCURACY, OR THE PRESENCE OR ABSENCE OF ERRORS, WHETHER OR NOT
     KNOWN OR DISCOVERABLE. WHERE DISCLAIMERS OF WARRANTIES ARE NOT
     ALLOWED IN FULL OR IN PART, THIS DISCLAIMER MAY NOT APPLY TO YOU.

  b. TO THE EXTENT POSSIBLE, IN NO EVENT WILL THE LICENSOR BE LIABLE
     TO YOU ON ANY LEGAL THEORY (INCLUDING, WITHOUT LIMITATION,
     NEGLIGENCE) OR OTHERWISE FOR ANY DIRECT, SPECIAL, INDIRECT,
     INCIDENTAL, CONSEQUENTIAL, PUNITIVE, EXEMPLARY, OR OTHER LOSSES,
     COSTS, EXPENSES, OR DAMAGES ARISING OUT OF THIS PUBLIC LICENSE OR
     USE OF THE LICENSED MATERIAL, EVEN IF THE LICENSOR HAS BEEN
     ADVISED OF THE POSSIBILITY OF SUCH LOSSES, COSTS, EXPENSES, OR
     DAMAGES. WHERE A LIMITATION OF LIABILITY IS NOT ALLOWED IN FULL OR
     IN PART, THIS LIMITATION MAY NOT APPLY TO YOU.

  c. The disclaimer of warranties and limitation of liability provided
     above shall be interpreted in a manner that, to the extent
     possible, most closely approximates an absolute disclaimer and
     waiver of all liability.


Section 6 -- Term and Termination.

  a. This Public License applies for the term of the Copyright and
     Similar Rights licensed here. However, if You fail to comply with
     this Public License, then Your rights under this Public License
     terminate automatically.

  b. Where Your right to use the Licensed Material has terminated under
     Section 6(a), it reinstates:

       1. automatically as of the date the violation is cured, provided
          it is cured within 30 days of Your discovery of the
          violation; or

       2. upon express reinstatement by the Licensor.

     For the avoidance of doubt, this Section 6(b) does not affect any
     right the Licensor may have to seek remedies for Your violations
     of this Public License.

  c. For the avoidance of doubt, the Licensor may also offer the
     Licensed Material under separate terms or conditions or stop
     distributing the Licensed Material at any time; however, doing so
     will not terminate this Public License.

  d. Sections 1, 5, 6, 7, and 8 survive termination of this Public
     License.


Section 7 -- Other Terms and Conditions.

  a. The Licensor shall not be bound by any additional or different
     terms or conditions communicated by You unless expressly agreed.

  b. Any arrangements, understandings, or agreements regarding the
     Licensed Material not stated herein are separate from and
     independent of the terms and conditions of this Public License.


Section 8 -- Interpretation.

  a. For the avoidance of doubt, this Public License does not, and
     shall not be interpreted to, reduce, limit, restrict, or impose
     conditions on any use of the Licensed Material that could lawfully
     be made without permission under this Public License.

  b. To the extent possible, if any provision of this Public License is
     deemed unenforceable, it shall be automatically reformed to the
     minimum extent necessary to make it enforceable. If the provision
     cannot be reformed, it shall be severed from this Public License
     without affecting the enforceability of the remaining terms and
     conditions.

  c. No term or condition of this Public License will be waived and no
     failure to comply consented to unless expressly agreed to by the
     Licensor.

  d. Nothing in this Public License constitutes or may be interpreted
     as a limitation upon, or waiver of, any privileges and immunities
     that apply to the Licensor or You, including from the legal
     processes of any jurisdiction or authority.


=======================================================================

Creative Commons is not a party to its public licenses.
Notwithstanding, Creative Commons may elect to apply one of its public
licenses to material it publishes and in those instances will be
considered the "Licensor." Except for the limited purpose of indicating
that material is shared under a Creative Commons public license or as
otherwise permitted by the Creative Commons policies published at
creativecommons.org/policies, Creative Commons does not authorize the
use of the trademark "Creative Commons" or any other trademark or logo
of Creative Commons without its prior written consent including,
without limitation, in connection with any unauthorized modifications
to any of its public licenses or any other arrangements,
understandings, or agreements concerning use of licensed material. For
the avoidance of doubt, this paragraph does not form part of the public
licenses.

Creative Commons may be contacted at creativecommons.org.


==> license-texts/doclicense-CC-by-nc-3.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NonCommercial 3.0 Unported}





\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES
NOT PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE
DOES NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE
COMMONS PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS.
CREATIVE COMMONS MAKES NO WARRANTIES REGARDING THE
INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR DAMAGES
RESULTING FROM ITS USE.
\end{quotation}
\subsubsection{\emph{License}}
\par THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS
OF THIS CREATIVE COMMONS PUBLIC LICENSE (``CCPL'' OR
``LICENSE''). THE WORK IS PROTECTED BY COPYRIGHT AND/OR OTHER
APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS
PROHIBITED.
\par BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU
ACCEPT AND AGREE TO BE BOUND BY THE TERMS OF THIS LICENSE.
TO THE EXTENT THIS LICENSE MAY BE CONSIDERED TO BE A
CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS CONTAINED HERE
IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.
\par \textbf{1. Definitions}
\begin{enumerate}
\item \textbf{``Adaptation''} means a work based upon
the Work, or upon the Work and other pre-existing works,
such as a translation, adaptation, derivative work,
arrangement of music or other alterations of a literary
or artistic work, or phonogram or performance and
includes cinematographic adaptations or any other form in
which the Work may be recast, transformed, or adapted
including in any form recognizably derived from the
original, except that a work that constitutes a
Collection will not be considered an Adaptation for the
purpose of this License. For the avoidance of doubt,
where the Work is a musical work, performance or
phonogram, the synchronization of the Work in
timed-relation with a moving image (``synching'') will be
considered an Adaptation for the purpose of this
License.
\item \textbf{``Collection''} means a collection of
literary or artistic works, such as encyclopedias and
anthologies, or performances, phonograms or broadcasts,
or other works or subject matter other than works listed
in Section 1(f) below, which, by reason of the selection
and arrangement of their contents, constitute
intellectual creations, in which the Work is included in
its entirety in unmodified form along with one or more
other contributions, each constituting separate and
independent works in themselves, which together are
assembled into a collective whole. A work that
constitutes a Collection will not be considered an
Adaptation (as defined above) for the purposes of this
License.
\item \textbf{``Distribute''} means to make available
to the public the original and copies of the Work or
Adaptation, as appropriate, through sale or other
transfer of ownership.
\item \textbf{``Licensor''} means the individual,
individuals, entity or entities that offer(s) the Work
under the terms of this License.
\item \textbf{``Original Author''} means, in the case
of a literary or artistic work, the individual,
individuals, entity or entities who created the Work or
if no individual or entity can be identified, the
publisher; and in addition (i) in the case of a
performance the actors, singers, musicians, dancers, and
other persons who act, sing, deliver, declaim, play in,
interpret or otherwise perform literary or artistic works
or expressions of folklore; (ii) in the case of a
phonogram the producer being the person or legal entity
who first fixes the sounds of a performance or other
sounds; and, (iii) in the case of broadcasts, the
organization that transmits the broadcast.
\item \textbf{``Work''} means the literary and/or
artistic work offered under the terms of this License
including without limitation any production in the
literary, scientific and artistic domain, whatever may be
the mode or form of its expression including digital
form, such as a book, pamphlet and other writing; a
lecture, address, sermon or other work of the same
nature; a dramatic or dramatico-musical work; a
choreographic work or entertainment in dumb show; a
musical composition with or without words; a
cinematographic work to which are assimilated works
expressed by a process analogous to cinematography; a
work of drawing, painting, architecture, sculpture,
engraving or lithography; a photographic work to which
are assimilated works expressed by a process analogous to
photography; a work of applied art; an illustration, map,
plan, sketch or three-dimensional work relative to
geography, topography, architecture or science; a
performance; a broadcast; a phonogram; a compilation of
data to the extent it is protected as a copyrightable
work; or a work performed by a variety or circus
performer to the extent it is not otherwise considered a
literary or artistic work.
\item \textbf{``You''} means an individual or entity
exercising rights under this License who has not
previously violated the terms of this License with
respect to the Work, or who has received express
permission from the Licensor to exercise rights under
this License despite a previous violation.
\item \textbf{``Publicly Perform''} means to perform
public recitations of the Work and to communicate to the
public those public recitations, by any means or process,
including by wire or wireless means or public digital
performances; to make available to the public Works in
such a way that members of the public may access these
Works from a place and at a place individually chosen by
them; to perform the Work to the public by any means or
process and the communication to the public of the
performances of the Work, including by public digital
performance; to broadcast and rebroadcast the Work by any
means including signs, sounds or images.
\item \textbf{``Reproduce''} means to make copies of
the Work by any means including without limitation by
sound or visual recordings and the right of fixation and
reproducing fixations of the Work, including storage of a
protected performance or phonogram in digital form or
other electronic medium.
\end{enumerate}
\par \textbf{2. Fair Dealing Rights.} Nothing in this
License is intended to reduce, limit, or restrict any uses
free from copyright or rights arising from limitations or
exceptions that are provided for in connection with the
copyright protection under copyright law or other
applicable laws.
\par \textbf{3. License Grant.} Subject to the terms
and conditions of this License, Licensor hereby grants You
a worldwide, royalty-free, non-exclusive, perpetual (for
the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:
\begin{enumerate}
\item to Reproduce the Work, to incorporate the Work into
one or more Collections, and to Reproduce the Work as
incorporated in the Collections;
\item to create and Reproduce Adaptations provided that any
such Adaptation, including any translation in any medium,
takes reasonable steps to clearly label, demarcate or
otherwise identify that changes were made to the original
Work. For example, a translation could be marked ``The
original work was translated from English to Spanish,'' or
a modification could indicate ``The original work has been
modified.'';
\item to Distribute and Publicly Perform the Work including
as incorporated in Collections; and,
\item to Distribute and Publicly Perform Adaptations.
\end{enumerate}
\par The above rights may be exercised in all media and
formats whether now known or hereafter devised. The above
rights include the right to make such modifications as are
technically necessary to exercise the rights in other media
and formats. Subject to Section 8(f), all rights not
expressly granted by Licensor are hereby reserved,
including but not limited to the rights set forth in
Section 4(d).
\par \textbf{4. Restrictions.} The license granted in
Section 3 above is expressly made subject to and limited by
the following restrictions:
\begin{enumerate}
\item You may Distribute or Publicly Perform the Work only
under the terms of this License. You must include a copy
of, or the Uniform Resource Identifier (URI) for, this
License with every copy of the Work You Distribute or
Publicly Perform. You may not offer or impose any terms
on the Work that restrict the terms of this License or
the ability of the recipient of the Work to exercise the
rights granted to that recipient under the terms of the
License. You may not sublicense the Work. You must keep
intact all notices that refer to this License and to the
disclaimer of warranties with every copy of the Work You
Distribute or Publicly Perform. When You Distribute or
Publicly Perform the Work, You may not impose any
effective technological measures on the Work that
restrict the ability of a recipient of the Work from You
to exercise the rights granted to that recipient under
the terms of the License. This Section 4(a) applies to
the Work as incorporated in a Collection, but this does
not require the Collection apart from the Work itself to
be made subject to the terms of this License. If You
create a Collection, upon notice from any Licensor You
must, to the extent practicable, remove from the
Collection any credit as required by Section 4(c), as
requested. If You create an Adaptation, upon notice from
any Licensor You must, to the extent practicable, remove
from the Adaptation any credit as required by Section
4(c), as requested.
\item You may not exercise any of the rights granted to You
in Section 3 above in any manner that is primarily
intended for or directed toward commercial advantage or
private monetary compensation. The exchange of the Work
for other copyrighted works by means of digital
file-sharing or otherwise shall not be considered to be
intended for or directed toward commercial advantage or
private monetary compensation, provided there is no
payment of any monetary compensation in connection with
the exchange of copyrighted works.
\item If You Distribute, or Publicly Perform the Work or
any Adaptations or Collections, You must, unless a
request has been made pursuant to Section 4(a), keep
intact all copyright notices for the Work and provide,
reasonable to the medium or means You are utilizing: (i)
the name of the Original Author (or pseudonym, if
applicable) if supplied, and/or if the Original Author
and/or Licensor designate another party or parties (e.g.,
a sponsor institute, publishing entity, journal) for
attribution (``Attribution Parties'') in Licensor's
copyright notice, terms of service or by other reasonable
means, the name of such party or parties; (ii) the title
of the Work if supplied; (iii) to the extent reasonably
practicable, the URI, if any, that Licensor specifies to
be associated with the Work, unless such URI does not
refer to the copyright notice or licensing information
for the Work; and, (iv) consistent with Section 3(b), in
the case of an Adaptation, a credit identifying the use
of the Work in the Adaptation (e.g., ``French translation
of the Work by Original Author,'' or ``Screenplay based on
original Work by Original Author''). The credit required
by this Section 4(c) may be implemented in any reasonable
manner; provided, however, that in the case of a
Adaptation or Collection, at a minimum such credit will
appear, if a credit for all contributing authors of the
Adaptation or Collection appears, then as part of these
credits and in a manner at least as prominent as the
credits for the other contributing authors. For the
avoidance of doubt, You may only use the credit required
by this Section for the purpose of attribution in the
manner set out above and, by exercising Your rights under
this License, You may not implicitly or explicitly assert
or imply any connection with, sponsorship or endorsement
by the Original Author, Licensor and/or Attribution
Parties, as appropriate, of You or Your use of the Work,
without the separate, express prior written permission of
the Original Author, Licensor and/or Attribution
Parties.
\item 
\par For the avoidance of doubt:
\begin{enumerate}
\item \textbf{Non-waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme cannot be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License;
\item \textbf{Waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme can be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License if Your exercise of such
rights is for a purpose or use which is otherwise
than noncommercial as permitted under Section 4(b)
and otherwise waives the right to collect royalties
through any statutory or compulsory licensing scheme;
and,
\item \textbf{Voluntary License Schemes}. The
Licensor reserves the right to collect royalties,
whether individually or, in the event that the
Licensor is a member of a collecting society that
administers voluntary licensing schemes, via that
society, from any exercise by You of the rights
granted under this License that is for a purpose or
use which is otherwise than noncommercial as
permitted under Section 4(c).
\end{enumerate}

\item Except as otherwise agreed in writing by the Licensor
or as may be otherwise permitted by applicable law, if
You Reproduce, Distribute or Publicly Perform the Work
either by itself or as part of any Adaptations or
Collections, You must not distort, mutilate, modify or
take other derogatory action in relation to the Work
which would be prejudicial to the Original Author's honor
or reputation. Licensor agrees that in those
jurisdictions (e.g. Japan), in which any exercise of the
right granted in Section 3(b) of this License (the right
to make Adaptations) would be deemed to be a distortion,
mutilation, modification or other derogatory action
prejudicial to the Original Author's honor and
reputation, the Licensor will waive or not assert, as
appropriate, this Section, to the fullest extent
permitted by the applicable national law, to enable You
to reasonably exercise Your right under Section 3(b) of
this License (right to make Adaptations) but not
otherwise.
\end{enumerate}
\par \textbf{5. Representations, Warranties and
Disclaimer}
\par UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN
WRITING, LICENSOR OFFERS THE WORK AS-IS AND MAKES NO
REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING,
WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE
ABSENCE OF LATENT OR OTHER DEFECTS, ACCURACY, OR THE
PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT DISCOVERABLE.
SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.
\par \textbf{6. Limitation on Liability.} EXCEPT TO
THE EXTENT REQUIRED BY APPLICABLE LAW, IN NO EVENT WILL
LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR ANY
SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY
DAMAGES ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK,
EVEN IF LICENSOR HAS BEEN ADVISED OF THE POSSIBILITY OF
SUCH DAMAGES.
\par \textbf{7. Termination}
\begin{enumerate}
\item This License and the rights granted hereunder will
terminate automatically upon any breach by You of the
terms of this License. Individuals or entities who have
received Adaptations or Collections from You under this
License, however, will not have their licenses terminated
provided such individuals or entities remain in full
compliance with those licenses. Sections 1, 2, 5, 6, 7,
and 8 will survive any termination of this License.
\item Subject to the above terms and conditions, the
license granted here is perpetual (for the duration of
the applicable copyright in the Work). Notwithstanding
the above, Licensor reserves the right to release the
Work under different license terms or to stop
distributing the Work at any time; provided, however that
any such election will not serve to withdraw this License
(or any other license that has been, or is required to
be, granted under the terms of this License), and this
License will continue in full force and effect unless
terminated as stated above.
\end{enumerate}
\par \textbf{8. Miscellaneous}
\begin{enumerate}
\item Each time You Distribute or Publicly Perform the Work
or a Collection, the Licensor offers to the recipient a
license to the Work on the same terms and conditions as
the license granted to You under this License.
\item Each time You Distribute or Publicly Perform an
Adaptation, Licensor offers to the recipient a license to
the original Work on the same terms and conditions as the
license granted to You under this License.
\item If any provision of this License is invalid or
unenforceable under applicable law, it shall not affect
the validity or enforceability of the remainder of the
terms of this License, and without further action by the
parties to this agreement, such provision shall be
reformed to the minimum extent necessary to make such
provision valid and enforceable.
\item No term or provision of this License shall be deemed
waived and no breach consented to unless such waiver or
consent shall be in writing and signed by the party to be
charged with such waiver or consent.
\item This License constitutes the entire agreement between
the parties with respect to the Work licensed here. There
are no understandings, agreements or representations with
respect to the Work not specified here. Licensor shall
not be bound by any additional provisions that may appear
in any communication from You. This License may not be
modified without the mutual written agreement of the
Licensor and You.
\item The rights granted under, and the subject matter
referenced, in this License were drafted utilizing the
terminology of the Berne Convention for the Protection of
Literary and Artistic Works (as amended on September 28,
1979), the Rome Convention of 1961, the WIPO Copyright
Treaty of 1996, the WIPO Performances and Phonograms
Treaty of 1996 and the Universal Copyright Convention (as
revised on July 24, 1971). These rights and subject
matter take effect in the relevant jurisdiction in which
the License terms are sought to be enforced according to
the corresponding provisions of the implementation of
those treaty provisions in the applicable national law.
If the standard suite of rights granted under applicable
copyright law includes additional rights not granted
under this License, such additional rights are deemed to
be included in the License; this License is not intended
to restrict the license of any rights under applicable
law.
\end{enumerate}
 
\begin{quotation}
\subsubsection{Creative Commons Notice}
\par Creative Commons is not a party to this License, and
makes no warranty whatsoever in connection with the Work.
Creative Commons will not be liable to You or any party
on any legal theory for any damages whatsoever, including
without limitation any general, special, incidental or
consequential damages arising in connection to this
license. Notwithstanding the foregoing two (2) sentences,
if Creative Commons has expressly identified itself as
the Licensor hereunder, it shall have all rights and
obligations of Licensor.
\par Except for the limited purpose of indicating to the
public that the Work is licensed under the CCPL, Creative
Commons does not authorize the use by either party of the
trademark ``Creative Commons'' or any related trademark or
logo of Creative Commons without the prior written
consent of Creative Commons. Any permitted use will be in
compliance with Creative Commons' then-current trademark
usage guidelines, as may be published on its website or
otherwise made available upon request from time to time.
For the avoidance of doubt, this trademark restriction
does not form part of the License.
\par Creative Commons may be contacted at \url{https://creativecommons.org/}.
\end{quotation} 



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nc-3.0-plaintext.tex <==
Creative Commons Legal Code

Attribution-NonCommercial 3.0 Unported

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR
    DAMAGES RESULTING FROM ITS USE.

License

THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS OF THIS CREATIVE
COMMONS PUBLIC LICENSE ("CCPL" OR "LICENSE"). THE WORK IS PROTECTED BY
COPYRIGHT AND/OR OTHER APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS PROHIBITED.

BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU ACCEPT AND AGREE
TO BE BOUND BY THE TERMS OF THIS LICENSE. TO THE EXTENT THIS LICENSE MAY
BE CONSIDERED TO BE A CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS
CONTAINED HERE IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.

1. Definitions

 a. "Adaptation" means a work based upon the Work, or upon the Work and
    other pre-existing works, such as a translation, adaptation,
    derivative work, arrangement of music or other alterations of a
    literary or artistic work, or phonogram or performance and includes
    cinematographic adaptations or any other form in which the Work may be
    recast, transformed, or adapted including in any form recognizably
    derived from the original, except that a work that constitutes a
    Collection will not be considered an Adaptation for the purpose of
    this License. For the avoidance of doubt, where the Work is a musical
    work, performance or phonogram, the synchronization of the Work in
    timed-relation with a moving image ("synching") will be considered an
    Adaptation for the purpose of this License.
 b. "Collection" means a collection of literary or artistic works, such as
    encyclopedias and anthologies, or performances, phonograms or
    broadcasts, or other works or subject matter other than works listed
    in Section 1(f) below, which, by reason of the selection and
    arrangement of their contents, constitute intellectual creations, in
    which the Work is included in its entirety in unmodified form along
    with one or more other contributions, each constituting separate and
    independent works in themselves, which together are assembled into a
    collective whole. A work that constitutes a Collection will not be
    considered an Adaptation (as defined above) for the purposes of this
    License.
 c. "Distribute" means to make available to the public the original and
    copies of the Work or Adaptation, as appropriate, through sale or
    other transfer of ownership.
 d. "Licensor" means the individual, individuals, entity or entities that
    offer(s) the Work under the terms of this License.
 e. "Original Author" means, in the case of a literary or artistic work,
    the individual, individuals, entity or entities who created the Work
    or if no individual or entity can be identified, the publisher; and in
    addition (i) in the case of a performance the actors, singers,
    musicians, dancers, and other persons who act, sing, deliver, declaim,
    play in, interpret or otherwise perform literary or artistic works or
    expressions of folklore; (ii) in the case of a phonogram the producer
    being the person or legal entity who first fixes the sounds of a
    performance or other sounds; and, (iii) in the case of broadcasts, the
    organization that transmits the broadcast.
 f. "Work" means the literary and/or artistic work offered under the terms
    of this License including without limitation any production in the
    literary, scientific and artistic domain, whatever may be the mode or
    form of its expression including digital form, such as a book,
    pamphlet and other writing; a lecture, address, sermon or other work
    of the same nature; a dramatic or dramatico-musical work; a
    choreographic work or entertainment in dumb show; a musical
    composition with or without words; a cinematographic work to which are
    assimilated works expressed by a process analogous to cinematography;
    a work of drawing, painting, architecture, sculpture, engraving or
    lithography; a photographic work to which are assimilated works
    expressed by a process analogous to photography; a work of applied
    art; an illustration, map, plan, sketch or three-dimensional work
    relative to geography, topography, architecture or science; a
    performance; a broadcast; a phonogram; a compilation of data to the
    extent it is protected as a copyrightable work; or a work performed by
    a variety or circus performer to the extent it is not otherwise
    considered a literary or artistic work.
 g. "You" means an individual or entity exercising rights under this
    License who has not previously violated the terms of this License with
    respect to the Work, or who has received express permission from the
    Licensor to exercise rights under this License despite a previous
    violation.
 h. "Publicly Perform" means to perform public recitations of the Work and
    to communicate to the public those public recitations, by any means or
    process, including by wire or wireless means or public digital
    performances; to make available to the public Works in such a way that
    members of the public may access these Works from a place and at a
    place individually chosen by them; to perform the Work to the public
    by any means or process and the communication to the public of the
    performances of the Work, including by public digital performance; to
    broadcast and rebroadcast the Work by any means including signs,
    sounds or images.
 i. "Reproduce" means to make copies of the Work by any means including
    without limitation by sound or visual recordings and the right of
    fixation and reproducing fixations of the Work, including storage of a
    protected performance or phonogram in digital form or other electronic
    medium.

2. Fair Dealing Rights. Nothing in this License is intended to reduce,
limit, or restrict any uses free from copyright or rights arising from
limitations or exceptions that are provided for in connection with the
copyright protection under copyright law or other applicable laws.

3. License Grant. Subject to the terms and conditions of this License,
Licensor hereby grants You a worldwide, royalty-free, non-exclusive,
perpetual (for the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:

 a. to Reproduce the Work, to incorporate the Work into one or more
    Collections, and to Reproduce the Work as incorporated in the
    Collections;
 b. to create and Reproduce Adaptations provided that any such Adaptation,
    including any translation in any medium, takes reasonable steps to
    clearly label, demarcate or otherwise identify that changes were made
    to the original Work. For example, a translation could be marked "The
    original work was translated from English to Spanish," or a
    modification could indicate "The original work has been modified.";
 c. to Distribute and Publicly Perform the Work including as incorporated
    in Collections; and,
 d. to Distribute and Publicly Perform Adaptations.

The above rights may be exercised in all media and formats whether now
known or hereafter devised. The above rights include the right to make
such modifications as are technically necessary to exercise the rights in
other media and formats. Subject to Section 8(f), all rights not expressly
granted by Licensor are hereby reserved, including but not limited to the
rights set forth in Section 4(d).

4. Restrictions. The license granted in Section 3 above is expressly made
subject to and limited by the following restrictions:

 a. You may Distribute or Publicly Perform the Work only under the terms
    of this License. You must include a copy of, or the Uniform Resource
    Identifier (URI) for, this License with every copy of the Work You
    Distribute or Publicly Perform. You may not offer or impose any terms
    on the Work that restrict the terms of this License or the ability of
    the recipient of the Work to exercise the rights granted to that
    recipient under the terms of the License. You may not sublicense the
    Work. You must keep intact all notices that refer to this License and
    to the disclaimer of warranties with every copy of the Work You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Work, You may not impose any effective technological
    measures on the Work that restrict the ability of a recipient of the
    Work from You to exercise the rights granted to that recipient under
    the terms of the License. This Section 4(a) applies to the Work as
    incorporated in a Collection, but this does not require the Collection
    apart from the Work itself to be made subject to the terms of this
    License. If You create a Collection, upon notice from any Licensor You
    must, to the extent practicable, remove from the Collection any credit
    as required by Section 4(c), as requested. If You create an
    Adaptation, upon notice from any Licensor You must, to the extent
    practicable, remove from the Adaptation any credit as required by
    Section 4(c), as requested.
 b. You may not exercise any of the rights granted to You in Section 3
    above in any manner that is primarily intended for or directed toward
    commercial advantage or private monetary compensation. The exchange of
    the Work for other copyrighted works by means of digital file-sharing
    or otherwise shall not be considered to be intended for or directed
    toward commercial advantage or private monetary compensation, provided
    there is no payment of any monetary compensation in connection with
    the exchange of copyrighted works.
 c. If You Distribute, or Publicly Perform the Work or any Adaptations or
    Collections, You must, unless a request has been made pursuant to
    Section 4(a), keep intact all copyright notices for the Work and
    provide, reasonable to the medium or means You are utilizing: (i) the
    name of the Original Author (or pseudonym, if applicable) if supplied,
    and/or if the Original Author and/or Licensor designate another party
    or parties (e.g., a sponsor institute, publishing entity, journal) for
    attribution ("Attribution Parties") in Licensor's copyright notice,
    terms of service or by other reasonable means, the name of such party
    or parties; (ii) the title of the Work if supplied; (iii) to the
    extent reasonably practicable, the URI, if any, that Licensor
    specifies to be associated with the Work, unless such URI does not
    refer to the copyright notice or licensing information for the Work;
    and, (iv) consistent with Section 3(b), in the case of an Adaptation,
    a credit identifying the use of the Work in the Adaptation (e.g.,
    "French translation of the Work by Original Author," or "Screenplay
    based on original Work by Original Author"). The credit required by
    this Section 4(c) may be implemented in any reasonable manner;
    provided, however, that in the case of a Adaptation or Collection, at
    a minimum such credit will appear, if a credit for all contributing
    authors of the Adaptation or Collection appears, then as part of these
    credits and in a manner at least as prominent as the credits for the
    other contributing authors. For the avoidance of doubt, You may only
    use the credit required by this Section for the purpose of attribution
    in the manner set out above and, by exercising Your rights under this
    License, You may not implicitly or explicitly assert or imply any
    connection with, sponsorship or endorsement by the Original Author,
    Licensor and/or Attribution Parties, as appropriate, of You or Your
    use of the Work, without the separate, express prior written
    permission of the Original Author, Licensor and/or Attribution
    Parties.
 d. For the avoidance of doubt:

     i. Non-waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme cannot be waived, the Licensor
        reserves the exclusive right to collect such royalties for any
        exercise by You of the rights granted under this License;
    ii. Waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme can be waived, the Licensor reserves
        the exclusive right to collect such royalties for any exercise by
        You of the rights granted under this License if Your exercise of
        such rights is for a purpose or use which is otherwise than
        noncommercial as permitted under Section 4(b) and otherwise waives
        the right to collect royalties through any statutory or compulsory
        licensing scheme; and,
   iii. Voluntary License Schemes. The Licensor reserves the right to
        collect royalties, whether individually or, in the event that the
        Licensor is a member of a collecting society that administers
        voluntary licensing schemes, via that society, from any exercise
        by You of the rights granted under this License that is for a
        purpose or use which is otherwise than noncommercial as permitted
        under Section 4(c).
 e. Except as otherwise agreed in writing by the Licensor or as may be
    otherwise permitted by applicable law, if You Reproduce, Distribute or
    Publicly Perform the Work either by itself or as part of any
    Adaptations or Collections, You must not distort, mutilate, modify or
    take other derogatory action in relation to the Work which would be
    prejudicial to the Original Author's honor or reputation. Licensor
    agrees that in those jurisdictions (e.g. Japan), in which any exercise
    of the right granted in Section 3(b) of this License (the right to
    make Adaptations) would be deemed to be a distortion, mutilation,
    modification or other derogatory action prejudicial to the Original
    Author's honor and reputation, the Licensor will waive or not assert,
    as appropriate, this Section, to the fullest extent permitted by the
    applicable national law, to enable You to reasonably exercise Your
    right under Section 3(b) of this License (right to make Adaptations)
    but not otherwise.

5. Representations, Warranties and Disclaimer

UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN WRITING, LICENSOR
OFFERS THE WORK AS-IS AND MAKES NO REPRESENTATIONS OR WARRANTIES OF ANY
KIND CONCERNING THE WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE,
INCLUDING, WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE ABSENCE OF
LATENT OR OTHER DEFECTS, ACCURACY, OR THE PRESENCE OF ABSENCE OF ERRORS,
WHETHER OR NOT DISCOVERABLE. SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION
OF IMPLIED WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.

6. Limitation on Liability. EXCEPT TO THE EXTENT REQUIRED BY APPLICABLE
LAW, IN NO EVENT WILL LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR
ANY SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY DAMAGES
ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK, EVEN IF LICENSOR HAS
BEEN ADVISED OF THE POSSIBILITY OF SUCH DAMAGES.

7. Termination

 a. This License and the rights granted hereunder will terminate
    automatically upon any breach by You of the terms of this License.
    Individuals or entities who have received Adaptations or Collections
    from You under this License, however, will not have their licenses
    terminated provided such individuals or entities remain in full
    compliance with those licenses. Sections 1, 2, 5, 6, 7, and 8 will
    survive any termination of this License.
 b. Subject to the above terms and conditions, the license granted here is
    perpetual (for the duration of the applicable copyright in the Work).
    Notwithstanding the above, Licensor reserves the right to release the
    Work under different license terms or to stop distributing the Work at
    any time; provided, however that any such election will not serve to
    withdraw this License (or any other license that has been, or is
    required to be, granted under the terms of this License), and this
    License will continue in full force and effect unless terminated as
    stated above.

8. Miscellaneous

 a. Each time You Distribute or Publicly Perform the Work or a Collection,
    the Licensor offers to the recipient a license to the Work on the same
    terms and conditions as the license granted to You under this License.
 b. Each time You Distribute or Publicly Perform an Adaptation, Licensor
    offers to the recipient a license to the original Work on the same
    terms and conditions as the license granted to You under this License.
 c. If any provision of this License is invalid or unenforceable under
    applicable law, it shall not affect the validity or enforceability of
    the remainder of the terms of this License, and without further action
    by the parties to this agreement, such provision shall be reformed to
    the minimum extent necessary to make such provision valid and
    enforceable.
 d. No term or provision of this License shall be deemed waived and no
    breach consented to unless such waiver or consent shall be in writing
    and signed by the party to be charged with such waiver or consent.
 e. This License constitutes the entire agreement between the parties with
    respect to the Work licensed here. There are no understandings,
    agreements or representations with respect to the Work not specified
    here. Licensor shall not be bound by any additional provisions that
    may appear in any communication from You. This License may not be
    modified without the mutual written agreement of the Licensor and You.
 f. The rights granted under, and the subject matter referenced, in this
    License were drafted utilizing the terminology of the Berne Convention
    for the Protection of Literary and Artistic Works (as amended on
    September 28, 1979), the Rome Convention of 1961, the WIPO Copyright
    Treaty of 1996, the WIPO Performances and Phonograms Treaty of 1996
    and the Universal Copyright Convention (as revised on July 24, 1971).
    These rights and subject matter take effect in the relevant
    jurisdiction in which the License terms are sought to be enforced
    according to the corresponding provisions of the implementation of
    those treaty provisions in the applicable national law. If the
    standard suite of rights granted under applicable copyright law
    includes additional rights not granted under this License, such
    additional rights are deemed to be included in the License; this
    License is not intended to restrict the license of any rights under
    applicable law.


Creative Commons Notice

    Creative Commons is not a party to this License, and makes no warranty
    whatsoever in connection with the Work. Creative Commons will not be
    liable to You or any party on any legal theory for any damages
    whatsoever, including without limitation any general, special,
    incidental or consequential damages arising in connection to this
    license. Notwithstanding the foregoing two (2) sentences, if Creative
    Commons has expressly identified itself as the Licensor hereunder, it
    shall have all rights and obligations of Licensor.

    Except for the limited purpose of indicating to the public that the
    Work is licensed under the CCPL, Creative Commons does not authorize
    the use by either party of the trademark "Creative Commons" or any
    related trademark or logo of Creative Commons without the prior
    written consent of Creative Commons. Any permitted use will be in
    compliance with Creative Commons' then-current trademark usage
    guidelines, as may be published on its website or otherwise made
    available upon request from time to time. For the avoidance of doubt,
    this trademark restriction does not form part of the License.

    Creative Commons may be contacted at https://creativecommons.org/.


==> license-texts/doclicense-CC-by-nc-4.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NonCommercial 4.0 International}







Official translations of this license are available in other languages.



\par Creative Commons Corporation (“Creative Commons”) is not a law firm and does not provide legal services or legal advice. Distribution of Creative Commons public licenses does not create a lawyer-client or other relationship. Creative Commons makes its licenses and related information available on an “as-is” basis. Creative Commons gives no warranties regarding its licenses, any material licensed under their terms and conditions, or any related information. Creative Commons disclaims all liability for damages resulting from their use to the fullest extent possible.


\par \textbf{Using Creative Commons Public Licenses}
\par Creative Commons public licenses provide a standard set of terms and conditions that creators and other rights holders may use to share original works of authorship and other material subject to copyright and certain other rights specified in the public license below. The following considerations are for informational purposes only, are not exhaustive, and do not form part of our licenses.
\begin{quotation}\textbf{Considerations for licensors:} Our public licenses are intended for use by those authorized to give the public permission to use material in ways otherwise restricted by copyright and certain other rights. Our licenses are irrevocable. Licensors should read and understand the terms and conditions of the license they choose before applying it. Licensors should also secure all rights necessary before applying our licenses so that the public can reuse the material as expected. Licensors should clearly mark any material not subject to the license. This includes other CC-licensed material, or material used under an exception or limitation to copyright. More considerations for licensors.\end{quotation}
\begin{quotation}\textbf{Considerations for the public:} By using one of our public licenses, a licensor grants the public permission to use the licensed material under specified terms and conditions. If the licensor’s permission is not necessary for any reason–for example, because of any applicable exception or limitation to copyright–then that use is not regulated by the license. Our licenses grant only permissions under copyright and certain other rights that a licensor has authority to grant. Use of the licensed material may still be restricted for other reasons, including because others have copyright or other rights in the material. A licensor may make special requests, such as asking that all changes be marked or described. Although not required by our licenses, you are encouraged to respect those requests where reasonable.
More considerations for the public.\end{quotation}

\subsubsection{Creative Commons Attribution-NonCommercial 4.0 International Public License}
\par By exercising the Licensed Rights (defined below), You accept and agree to be bound by the terms and conditions of this Creative Commons Attribution-NonCommercial 4.0 International Public License (``Public License''). To the extent this Public License may be interpreted as a contract, You are granted the Licensed Rights in consideration of Your acceptance of these terms and conditions, and the Licensor grants You such rights in consideration of benefits the Licensor receives from making the Licensed Material available under these terms and conditions.
\par \textbf{Section 1 – Definitions.}
\begin{enumerate}
\item \textbf{Adapted Material} means material subject to Copyright and Similar Rights that is derived from or based upon the Licensed Material and in which the Licensed Material is translated, altered, arranged, transformed, or otherwise modified in a manner requiring permission under the Copyright and Similar Rights held by the Licensor. For purposes of this Public License, where the Licensed Material is a musical work, performance, or sound recording, Adapted Material is always produced where the Licensed Material is synched in timed relation with a moving image.
\item \textbf{Adapter's License} means the license You apply to Your Copyright and Similar Rights in Your contributions to Adapted Material in accordance with the terms and conditions of this Public License.
\item \textbf{Copyright and Similar Rights} means copyright and/or similar rights closely related to copyright including, without limitation, performance, broadcast, sound recording, and Sui Generis Database Rights, without regard to how the rights are labeled or categorized. For purposes of this Public License, the rights specified in Section 2(b)(1)-(2) are not Copyright and Similar Rights.
\item \textbf{Effective Technological Measures} means those measures that, in the absence of proper authority, may not
be circumvented under laws fulfilling obligations under Article 11 of the WIPO Copyright Treaty adopted on December 20, 1996, and/or similar
international agreements.
\item \textbf{Exceptions and Limitations} means fair use, fair dealing, and/or any other exception or limitation to Copyright and Similar Rights that applies to Your use of the Licensed Material.
\item \textbf{Licensed Material} means the artistic or literary work, database, or other material to which the Licensor applied this Public License.
\item \textbf{Licensed Rights} means the rights granted to You subject to the terms and conditions of this Public License, which are limited to all Copyright and Similar Rights that apply to Your use of the Licensed Material and that the Licensor has authority to license.
\item \textbf{Licensor} means the individual(s) or entity(ies) granting rights under this Public License.
\item \textbf{NonCommercial} means not primarily intended for or directed towards commercial advantage or monetary compensation. For purposes of this Public License, the exchange of the Licensed Material for other material subject to Copyright and Similar Rights by digital file-sharing or similar means is NonCommercial provided there is no payment of monetary compensation in connection with the exchange.
\item \textbf{Share} means to provide material to the public by any means or process that requires permission under the Licensed Rights, such as reproduction, public display, public performance, distribution, dissemination, communication, or importation, and to make material available to the public including in ways that members of the public may access the material from a place and at a time individually chosen by them.
\item \textbf{Sui Generis Database Rights} means rights other than copyright resulting from Directive 96/9/EC of the European Parliament and of the Council of 11 March 1996 on the legal protection of databases, as amended and/or succeeded, as well as other essentially equivalent rights anywhere in the world.
\item \textbf{You} means the individual or entity exercising the Licensed Rights under this Public License. \textbf{Your} has a corresponding meaning.
\end{enumerate}
\par \textbf{Section 2 – Scope.}
\begin{enumerate}
\item \textbf{License grant}.
\begin{enumerate}
\item Subject to the terms and conditions of this Public License, the Licensor hereby grants You a worldwide, royalty-free, non-sublicensable, non-exclusive, irrevocable license to exercise the Licensed Rights in the Licensed Material to:
\begin{enumerate}
\item reproduce and Share the Licensed Material, in whole or in part, for NonCommercial purposes only; and
\item produce, reproduce, and Share Adapted Material for NonCommercial purposes only.
\end{enumerate}
\item Exceptions and Limitations. For the avoidance of doubt, where Exceptions and Limitations apply to Your use, this Public License does not apply, and You do not need to comply with its terms and conditions.
\item Term. The term of this Public License is specified in Section 6(a).
\item Media and formats; technical modifications allowed. The Licensor authorizes You to exercise the Licensed Rights in all media and formats whether now known or hereafter created, and to make technical modifications necessary to do so. The Licensor waives and/or agrees not to assert any right or authority to forbid You from making technical modifications necessary to exercise the Licensed Rights, including technical modifications necessary to circumvent Effective Technological Measures. For purposes of this Public License, simply making modifications authorized by this Section 2(a)(4) never produces Adapted Material.
\item Downstream recipients.

\begin{enumerate}
\item Offer from the Licensor – Licensed Material. Every recipient of the Licensed Material automatically receives an offer from the Licensor to exercise the Licensed Rights under the terms and conditions of this Public License.
\item No downstream restrictions. You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, the Licensed Material if doing so restricts exercise of the Licensed Rights by any recipient of the Licensed Material.
\end{enumerate}

\item No endorsement. Nothing in this Public License constitutes or may be construed as permission to assert or imply that You are, or that Your use of the Licensed Material is, connected with, or sponsored, endorsed, or granted official status by, the Licensor or others designated to receive attribution as provided in Section 3(a)(1)(A)(i).
\end{enumerate}
\item \par \textbf{Other rights}.
\begin{enumerate}
\item Moral rights, such as the right of integrity, are not licensed under this Public License, nor are publicity, privacy, and/or other similar personality rights; however, to the extent possible, the Licensor waives and/or agrees not to assert any such rights held by the Licensor to the limited extent necessary to allow You to exercise the Licensed Rights, but not otherwise.
\item Patent and trademark rights are not licensed under this Public License.
\item To the extent possible, the Licensor waives any right to collect royalties from You for the exercise of the Licensed Rights, whether directly or through a collecting society under any voluntary or waivable statutory or compulsory licensing scheme. In all other cases the Licensor expressly reserves any right to collect such royalties, including when the Licensed Material is used other than for NonCommercial purposes.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 3 – License Conditions.}
\par Your exercise of the Licensed Rights is expressly made subject to the following conditions.
\begin{enumerate}
\item \par \textbf{Attribution}.
\begin{enumerate}
\item \par If You Share the Licensed Material (including in modified form), You must:
\begin{enumerate}
\item retain the following if it is supplied by the Licensor with the Licensed Material:
\begin{enumerate}
\item identification of the creator(s) of the Licensed Material and any others designated to receive attribution, in any reasonable manner requested by the Licensor (including by pseudonym if designated);
\item a copyright notice;
\item a notice that refers to this Public License; 
\item a notice that refers to the disclaimer of warranties;
\item a URI or hyperlink to the Licensed Material to the extent reasonably practicable;
\end{enumerate}
\item indicate if You modified the Licensed Material and retain an indication of any previous modifications; and
\item indicate the Licensed Material is licensed under this Public License,
and include the text of, or the URI or hyperlink to, this Public
License.
\end{enumerate}

\item You may satisfy the conditions in Section 3(a)(1) in any reasonable manner based on the medium, means, and context in which You Share the Licensed Material. For example, it may be reasonable to satisfy the conditions by providing a URI or hyperlink to a resource that includes the required information.
\item If requested by the Licensor, You must remove any of the information required by Section 3(a)(1)(A) to the extent reasonably practicable.
\item If You Share Adapted Material You produce, the Adapter's License You apply must not prevent recipients of the Adapted Material from complying with this Public License.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 4 – Sui Generis Database Rights.}
\par Where the Licensed Rights include Sui Generis Database Rights that apply to Your use of the Licensed Material:
\begin{enumerate}
\item for the avoidance of doubt, Section 2(a)(1) grants You the right to extract, reuse, reproduce, and Share all or a substantial portion of the contents of the database for NonCommercial purposes only;
\item if You include all or a substantial portion of the database contents in a database in which You have Sui Generis Database Rights, then the database in which You have Sui Generis Database Rights (but not its individual contents) is Adapted Material; and
\item You must comply with the conditions in Section 3(a) if You Share all or a substantial portion of the contents of the database.
\end{enumerate}
For the avoidance of doubt, this Section 4 supplements and does not replace Your obligations under this Public License where the Licensed Rights include other Copyright and Similar Rights.
\par \textbf{Section 5 – Disclaimer of Warranties and Limitation of Liability.}
\begin{enumerate}
\item \textbf{Unless otherwise separately undertaken by the Licensor, to the extent possible, the Licensor offers the Licensed Material as-is and as-available, and makes no representations or warranties of any kind concerning the Licensed Material, whether express, implied, statutory, or other. This includes, without limitation, warranties of title, merchantability, fitness for a particular purpose, non-infringement, absence of latent or other defects, accuracy, or the presence or absence of errors, whether or not known or discoverable. Where disclaimers of warranties are not allowed in full or in part, this disclaimer may not apply to You.}
\item \textbf{To the extent possible, in no event will the Licensor be liable to You on any legal theory (including, without limitation, negligence) or otherwise for any direct, special, indirect, incidental, consequential, punitive, exemplary, or other losses, costs, expenses, or damages arising out of this Public License or use of the Licensed Material, even if the Licensor has been advised of the possibility of such losses, costs, expenses, or damages. Where a limitation of liability is not allowed in full or in part, this limitation may not apply to You.}
\end{enumerate}
\begin{enumerate}
\item The disclaimer of warranties and limitation of liability provided above shall be interpreted in a manner that, to the extent possible, most closely approximates an absolute disclaimer and waiver of all liability.
\end{enumerate}
\par \textbf{Section 6 – Term and Termination.}
\begin{enumerate}
\item This Public License applies for the term of the Copyright and Similar Rights licensed here. However, if You fail to comply with this Public License, then Your rights under this Public License terminate automatically.
\item 
\par Where Your right to use the Licensed Material has terminated under Section 6(a), it reinstates:
\begin{enumerate}
\item automatically as of the date the violation is cured, provided it is cured within 30 days of Your discovery of the violation; or
\item upon express reinstatement by the Licensor.
\end{enumerate}
For the avoidance of doubt, this Section 6(b) does not affect any right the Licensor may have to seek remedies for Your violations of this Public License.
\item For the avoidance of doubt, the Licensor may also offer the Licensed Material under separate terms or conditions or stop distributing the Licensed Material at any time; however, doing so will not terminate this Public License.
\item Sections 1, 5, 6, 7, and 8 survive termination of this Public License.
\end{enumerate}
\par \textbf{Section 7 – Other Terms and Conditions.}
\begin{enumerate}
\item The Licensor shall not be bound by any additional or different terms or conditions communicated by You unless expressly agreed.
\item Any arrangements, understandings, or agreements regarding the Licensed Material not stated herein are separate from and independent of the terms and conditions of this Public License.
\end{enumerate}
\par \textbf{Section 8 – Interpretation.}
\begin{enumerate}
\item For the avoidance of doubt, this Public License does not, and shall not be interpreted to, reduce, limit, restrict, or impose conditions on any use of the Licensed Material that could lawfully be made without permission under this Public License.
\item To the extent possible, if any provision of this Public License is deemed unenforceable, it shall be automatically reformed to the minimum extent necessary to make it enforceable. If the provision cannot be reformed, it shall be severed from this Public License without affecting the enforceability of the remaining terms and conditions.
\item No term or condition of this Public License will be waived and no failure to comply consented to unless expressly agreed to by the Licensor.
\item Nothing in this Public License constitutes or may be interpreted as a limitation upon, or waiver of, any privileges and immunities that apply to the Licensor or You, including from the legal processes of any jurisdiction or authority.
\end{enumerate}
\par Creative Commons is not a party to its public licenses. Notwithstanding, Creative Commons may elect to apply one of its public licenses to material it publishes and in those instances will be considered the “Licensor.” The text of the Creative Commons public licenses is dedicated to the public domain under the CC0 Public Domain Dedication. Except for the limited purpose of indicating that material is shared under a Creative Commons public license or as otherwise permitted by the Creative Commons policies published at creativecommons.org/policies, Creative Commons does not authorize the use of the trademark “Creative Commons” or any other trademark or logo of Creative Commons without its prior written consent including, without limitation, in connection with any unauthorized modifications to any of its public licenses or any other arrangements, understandings, or agreements concerning use of licensed material. For the avoidance of doubt, this paragraph does not form part of the public licenses.\\\\
Creative Commons may be contacted at creativecommons.org.
\par Additional languages available: Bahasa Indonesia, Nederlands, norsk, suomeksi, te reo Māori, українська, 日本語. Please read the FAQ for more information about official translations.



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nc-4.0-plaintext.tex <==
Attribution-NonCommercial 4.0 International

=======================================================================

Creative Commons Corporation ("Creative Commons") is not a law firm and
does not provide legal services or legal advice. Distribution of
Creative Commons public licenses does not create a lawyer-client or
other relationship. Creative Commons makes its licenses and related
information available on an "as-is" basis. Creative Commons gives no
warranties regarding its licenses, any material licensed under their
terms and conditions, or any related information. Creative Commons
disclaims all liability for damages resulting from their use to the
fullest extent possible.

Using Creative Commons Public Licenses

Creative Commons public licenses provide a standard set of terms and
conditions that creators and other rights holders may use to share
original works of authorship and other material subject to copyright
and certain other rights specified in the public license below. The
following considerations are for informational purposes only, are not
exhaustive, and do not form part of our licenses.

     Considerations for licensors: Our public licenses are
     intended for use by those authorized to give the public
     permission to use material in ways otherwise restricted by
     copyright and certain other rights. Our licenses are
     irrevocable. Licensors should read and understand the terms
     and conditions of the license they choose before applying it.
     Licensors should also secure all rights necessary before
     applying our licenses so that the public can reuse the
     material as expected. Licensors should clearly mark any
     material not subject to the license. This includes other CC-
     licensed material, or material used under an exception or
     limitation to copyright. More considerations for licensors:
	wiki.creativecommons.org/Considerations_for_licensors

     Considerations for the public: By using one of our public
     licenses, a licensor grants the public permission to use the
     licensed material under specified terms and conditions. If
     the licensor's permission is not necessary for any reason--for
     example, because of any applicable exception or limitation to
     copyright--then that use is not regulated by the license. Our
     licenses grant only permissions under copyright and certain
     other rights that a licensor has authority to grant. Use of
     the licensed material may still be restricted for other
     reasons, including because others have copyright or other
     rights in the material. A licensor may make special requests,
     such as asking that all changes be marked or described.
     Although not required by our licenses, you are encouraged to
     respect those requests where reasonable. More_considerations
     for the public: 
	wiki.creativecommons.org/Considerations_for_licensees

=======================================================================

Creative Commons Attribution-NonCommercial 4.0 International Public
License

By exercising the Licensed Rights (defined below), You accept and agree
to be bound by the terms and conditions of this Creative Commons
Attribution-NonCommercial 4.0 International Public License ("Public
License"). To the extent this Public License may be interpreted as a
contract, You are granted the Licensed Rights in consideration of Your
acceptance of these terms and conditions, and the Licensor grants You
such rights in consideration of benefits the Licensor receives from
making the Licensed Material available under these terms and
conditions.


Section 1 -- Definitions.

  a. Adapted Material means material subject to Copyright and Similar
     Rights that is derived from or based upon the Licensed Material
     and in which the Licensed Material is translated, altered,
     arranged, transformed, or otherwise modified in a manner requiring
     permission under the Copyright and Similar Rights held by the
     Licensor. For purposes of this Public License, where the Licensed
     Material is a musical work, performance, or sound recording,
     Adapted Material is always produced where the Licensed Material is
     synched in timed relation with a moving image.

  b. Adapter's License means the license You apply to Your Copyright
     and Similar Rights in Your contributions to Adapted Material in
     accordance with the terms and conditions of this Public License.

  c. Copyright and Similar Rights means copyright and/or similar rights
     closely related to copyright including, without limitation,
     performance, broadcast, sound recording, and Sui Generis Database
     Rights, without regard to how the rights are labeled or
     categorized. For purposes of this Public License, the rights
     specified in Section 2(b)(1)-(2) are not Copyright and Similar
     Rights.
  d. Effective Technological Measures means those measures that, in the
     absence of proper authority, may not be circumvented under laws
     fulfilling obligations under Article 11 of the WIPO Copyright
     Treaty adopted on December 20, 1996, and/or similar international
     agreements.

  e. Exceptions and Limitations means fair use, fair dealing, and/or
     any other exception or limitation to Copyright and Similar Rights
     that applies to Your use of the Licensed Material.

  f. Licensed Material means the artistic or literary work, database,
     or other material to which the Licensor applied this Public
     License.

  g. Licensed Rights means the rights granted to You subject to the
     terms and conditions of this Public License, which are limited to
     all Copyright and Similar Rights that apply to Your use of the
     Licensed Material and that the Licensor has authority to license.

  h. Licensor means the individual(s) or entity(ies) granting rights
     under this Public License.

  i. NonCommercial means not primarily intended for or directed towards
     commercial advantage or monetary compensation. For purposes of
     this Public License, the exchange of the Licensed Material for
     other material subject to Copyright and Similar Rights by digital
     file-sharing or similar means is NonCommercial provided there is
     no payment of monetary compensation in connection with the
     exchange.

  j. Share means to provide material to the public by any means or
     process that requires permission under the Licensed Rights, such
     as reproduction, public display, public performance, distribution,
     dissemination, communication, or importation, and to make material
     available to the public including in ways that members of the
     public may access the material from a place and at a time
     individually chosen by them.

  k. Sui Generis Database Rights means rights other than copyright
     resulting from Directive 96/9/EC of the European Parliament and of
     the Council of 11 March 1996 on the legal protection of databases,
     as amended and/or succeeded, as well as other essentially
     equivalent rights anywhere in the world.

  l. You means the individual or entity exercising the Licensed Rights
     under this Public License. Your has a corresponding meaning.


Section 2 -- Scope.

  a. License grant.

       1. Subject to the terms and conditions of this Public License,
          the Licensor hereby grants You a worldwide, royalty-free,
          non-sublicensable, non-exclusive, irrevocable license to
          exercise the Licensed Rights in the Licensed Material to:

            a. reproduce and Share the Licensed Material, in whole or
               in part, for NonCommercial purposes only; and

            b. produce, reproduce, and Share Adapted Material for
               NonCommercial purposes only.

       2. Exceptions and Limitations. For the avoidance of doubt, where
          Exceptions and Limitations apply to Your use, this Public
          License does not apply, and You do not need to comply with
          its terms and conditions.

       3. Term. The term of this Public License is specified in Section
          6(a).

       4. Media and formats; technical modifications allowed. The
          Licensor authorizes You to exercise the Licensed Rights in
          all media and formats whether now known or hereafter created,
          and to make technical modifications necessary to do so. The
          Licensor waives and/or agrees not to assert any right or
          authority to forbid You from making technical modifications
          necessary to exercise the Licensed Rights, including
          technical modifications necessary to circumvent Effective
          Technological Measures. For purposes of this Public License,
          simply making modifications authorized by this Section 2(a)
          (4) never produces Adapted Material.

       5. Downstream recipients.

            a. Offer from the Licensor -- Licensed Material. Every
               recipient of the Licensed Material automatically
               receives an offer from the Licensor to exercise the
               Licensed Rights under the terms and conditions of this
               Public License.

            b. No downstream restrictions. You may not offer or impose
               any additional or different terms or conditions on, or
               apply any Effective Technological Measures to, the
               Licensed Material if doing so restricts exercise of the
               Licensed Rights by any recipient of the Licensed
               Material.

       6. No endorsement. Nothing in this Public License constitutes or
          may be construed as permission to assert or imply that You
          are, or that Your use of the Licensed Material is, connected
          with, or sponsored, endorsed, or granted official status by,
          the Licensor or others designated to receive attribution as
          provided in Section 3(a)(1)(A)(i).

  b. Other rights.

       1. Moral rights, such as the right of integrity, are not
          licensed under this Public License, nor are publicity,
          privacy, and/or other similar personality rights; however, to
          the extent possible, the Licensor waives and/or agrees not to
          assert any such rights held by the Licensor to the limited
          extent necessary to allow You to exercise the Licensed
          Rights, but not otherwise.

       2. Patent and trademark rights are not licensed under this
          Public License.

       3. To the extent possible, the Licensor waives any right to
          collect royalties from You for the exercise of the Licensed
          Rights, whether directly or through a collecting society
          under any voluntary or waivable statutory or compulsory
          licensing scheme. In all other cases the Licensor expressly
          reserves any right to collect such royalties, including when
          the Licensed Material is used other than for NonCommercial
          purposes.


Section 3 -- License Conditions.

Your exercise of the Licensed Rights is expressly made subject to the
following conditions.

  a. Attribution.

       1. If You Share the Licensed Material (including in modified
          form), You must:

            a. retain the following if it is supplied by the Licensor
               with the Licensed Material:

                 i. identification of the creator(s) of the Licensed
                    Material and any others designated to receive
                    attribution, in any reasonable manner requested by
                    the Licensor (including by pseudonym if
                    designated);

                ii. a copyright notice;

               iii. a notice that refers to this Public License;

                iv. a notice that refers to the disclaimer of
                    warranties;

                 v. a URI or hyperlink to the Licensed Material to the
                    extent reasonably practicable;

            b. indicate if You modified the Licensed Material and
               retain an indication of any previous modifications; and

            c. indicate the Licensed Material is licensed under this
               Public License, and include the text of, or the URI or
               hyperlink to, this Public License.

       2. You may satisfy the conditions in Section 3(a)(1) in any
          reasonable manner based on the medium, means, and context in
          which You Share the Licensed Material. For example, it may be
          reasonable to satisfy the conditions by providing a URI or
          hyperlink to a resource that includes the required
          information.

       3. If requested by the Licensor, You must remove any of the
          information required by Section 3(a)(1)(A) to the extent
          reasonably practicable.

       4. If You Share Adapted Material You produce, the Adapter's
          License You apply must not prevent recipients of the Adapted
          Material from complying with this Public License.


Section 4 -- Sui Generis Database Rights.

Where the Licensed Rights include Sui Generis Database Rights that
apply to Your use of the Licensed Material:

  a. for the avoidance of doubt, Section 2(a)(1) grants You the right
     to extract, reuse, reproduce, and Share all or a substantial
     portion of the contents of the database for NonCommercial purposes
     only;

  b. if You include all or a substantial portion of the database
     contents in a database in which You have Sui Generis Database
     Rights, then the database in which You have Sui Generis Database
     Rights (but not its individual contents) is Adapted Material; and

  c. You must comply with the conditions in Section 3(a) if You Share
     all or a substantial portion of the contents of the database.

For the avoidance of doubt, this Section 4 supplements and does not
replace Your obligations under this Public License where the Licensed
Rights include other Copyright and Similar Rights.


Section 5 -- Disclaimer of Warranties and Limitation of Liability.

  a. UNLESS OTHERWISE SEPARATELY UNDERTAKEN BY THE LICENSOR, TO THE
     EXTENT POSSIBLE, THE LICENSOR OFFERS THE LICENSED MATERIAL AS-IS
     AND AS-AVAILABLE, AND MAKES NO REPRESENTATIONS OR WARRANTIES OF
     ANY KIND CONCERNING THE LICENSED MATERIAL, WHETHER EXPRESS,
     IMPLIED, STATUTORY, OR OTHER. THIS INCLUDES, WITHOUT LIMITATION,
     WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
     PURPOSE, NON-INFRINGEMENT, ABSENCE OF LATENT OR OTHER DEFECTS,
     ACCURACY, OR THE PRESENCE OR ABSENCE OF ERRORS, WHETHER OR NOT
     KNOWN OR DISCOVERABLE. WHERE DISCLAIMERS OF WARRANTIES ARE NOT
     ALLOWED IN FULL OR IN PART, THIS DISCLAIMER MAY NOT APPLY TO YOU.

  b. TO THE EXTENT POSSIBLE, IN NO EVENT WILL THE LICENSOR BE LIABLE
     TO YOU ON ANY LEGAL THEORY (INCLUDING, WITHOUT LIMITATION,
     NEGLIGENCE) OR OTHERWISE FOR ANY DIRECT, SPECIAL, INDIRECT,
     INCIDENTAL, CONSEQUENTIAL, PUNITIVE, EXEMPLARY, OR OTHER LOSSES,
     COSTS, EXPENSES, OR DAMAGES ARISING OUT OF THIS PUBLIC LICENSE OR
     USE OF THE LICENSED MATERIAL, EVEN IF THE LICENSOR HAS BEEN
     ADVISED OF THE POSSIBILITY OF SUCH LOSSES, COSTS, EXPENSES, OR
     DAMAGES. WHERE A LIMITATION OF LIABILITY IS NOT ALLOWED IN FULL OR
     IN PART, THIS LIMITATION MAY NOT APPLY TO YOU.

  c. The disclaimer of warranties and limitation of liability provided
     above shall be interpreted in a manner that, to the extent
     possible, most closely approximates an absolute disclaimer and
     waiver of all liability.


Section 6 -- Term and Termination.

  a. This Public License applies for the term of the Copyright and
     Similar Rights licensed here. However, if You fail to comply with
     this Public License, then Your rights under this Public License
     terminate automatically.

  b. Where Your right to use the Licensed Material has terminated under
     Section 6(a), it reinstates:

       1. automatically as of the date the violation is cured, provided
          it is cured within 30 days of Your discovery of the
          violation; or

       2. upon express reinstatement by the Licensor.

     For the avoidance of doubt, this Section 6(b) does not affect any
     right the Licensor may have to seek remedies for Your violations
     of this Public License.

  c. For the avoidance of doubt, the Licensor may also offer the
     Licensed Material under separate terms or conditions or stop
     distributing the Licensed Material at any time; however, doing so
     will not terminate this Public License.

  d. Sections 1, 5, 6, 7, and 8 survive termination of this Public
     License.


Section 7 -- Other Terms and Conditions.

  a. The Licensor shall not be bound by any additional or different
     terms or conditions communicated by You unless expressly agreed.

  b. Any arrangements, understandings, or agreements regarding the
     Licensed Material not stated herein are separate from and
     independent of the terms and conditions of this Public License.


Section 8 -- Interpretation.

  a. For the avoidance of doubt, this Public License does not, and
     shall not be interpreted to, reduce, limit, restrict, or impose
     conditions on any use of the Licensed Material that could lawfully
     be made without permission under this Public License.

  b. To the extent possible, if any provision of this Public License is
     deemed unenforceable, it shall be automatically reformed to the
     minimum extent necessary to make it enforceable. If the provision
     cannot be reformed, it shall be severed from this Public License
     without affecting the enforceability of the remaining terms and
     conditions.

  c. No term or condition of this Public License will be waived and no
     failure to comply consented to unless expressly agreed to by the
     Licensor.

  d. Nothing in this Public License constitutes or may be interpreted
     as a limitation upon, or waiver of, any privileges and immunities
     that apply to the Licensor or You, including from the legal
     processes of any jurisdiction or authority.

=======================================================================

Creative Commons is not a party to its public licenses.
Notwithstanding, Creative Commons may elect to apply one of its public
licenses to material it publishes and in those instances will be
considered the "Licensor." Except for the limited purpose of indicating
that material is shared under a Creative Commons public license or as
otherwise permitted by the Creative Commons policies published at
creativecommons.org/policies, Creative Commons does not authorize the
use of the trademark "Creative Commons" or any other trademark or logo
of Creative Commons without its prior written consent including,
without limitation, in connection with any unauthorized modifications
to any of its public licenses or any other arrangements,
understandings, or agreements concerning use of licensed material. For
the avoidance of doubt, this paragraph does not form part of the public
licenses.

Creative Commons may be contacted at creativecommons.org.


==> license-texts/doclicense-CC-by-nc-nd-3.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NonCommercial-NoDerivs 3.0 Unported}





\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES
NOT PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE
DOES NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE
COMMONS PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS.
CREATIVE COMMONS MAKES NO WARRANTIES REGARDING THE
INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR DAMAGES
RESULTING FROM ITS USE.
\end{quotation}
\subsubsection{\emph{License}}
\par THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS
OF THIS CREATIVE COMMONS PUBLIC LICENSE (``CCPL'' OR
``LICENSE''). THE WORK IS PROTECTED BY COPYRIGHT AND/OR OTHER
APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS
PROHIBITED.
\par BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU
ACCEPT AND AGREE TO BE BOUND BY THE TERMS OF THIS LICENSE.
TO THE EXTENT THIS LICENSE MAY BE CONSIDERED TO BE A
CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS CONTAINED HERE
IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.
\par \textbf{1. Definitions}
\begin{enumerate}
\item \textbf{``Adaptation''} means a work based upon
the Work, or upon the Work and other pre-existing works,
such as a translation, adaptation, derivative work,
arrangement of music or other alterations of a literary
or artistic work, or phonogram or performance and
includes cinematographic adaptations or any other form in
which the Work may be recast, transformed, or adapted
including in any form recognizably derived from the
original, except that a work that constitutes a
Collection will not be considered an Adaptation for the
purpose of this License. For the avoidance of doubt,
where the Work is a musical work, performance or
phonogram, the synchronization of the Work in
timed-relation with a moving image (``synching'') will be
considered an Adaptation for the purpose of this
License.
\item \textbf{``Collection''} means a collection of
literary or artistic works, such as encyclopedias and
anthologies, or performances, phonograms or broadcasts,
or other works or subject matter other than works listed
in Section 1(f) below, which, by reason of the selection
and arrangement of their contents, constitute
intellectual creations, in which the Work is included in
its entirety in unmodified form along with one or more
other contributions, each constituting separate and
independent works in themselves, which together are
assembled into a collective whole. A work that
constitutes a Collection will not be considered an
Adaptation (as defined above) for the purposes of this
License.
\item \textbf{``Distribute''} means to make available
to the public the original and copies of the Work through
sale or other transfer of ownership.
\item \textbf{``Licensor''} means the individual,
individuals, entity or entities that offer(s) the Work
under the terms of this License.
\item \textbf{``Original Author''} means, in the case
of a literary or artistic work, the individual,
individuals, entity or entities who created the Work or
if no individual or entity can be identified, the
publisher; and in addition (i) in the case of a
performance the actors, singers, musicians, dancers, and
other persons who act, sing, deliver, declaim, play in,
interpret or otherwise perform literary or artistic works
or expressions of folklore; (ii) in the case of a
phonogram the producer being the person or legal entity
who first fixes the sounds of a performance or other
sounds; and, (iii) in the case of broadcasts, the
organization that transmits the broadcast.
\item \textbf{``Work''} means the literary and/or
artistic work offered under the terms of this License
including without limitation any production in the
literary, scientific and artistic domain, whatever may be
the mode or form of its expression including digital
form, such as a book, pamphlet and other writing; a
lecture, address, sermon or other work of the same
nature; a dramatic or dramatico-musical work; a
choreographic work or entertainment in dumb show; a
musical composition with or without words; a
cinematographic work to which are assimilated works
expressed by a process analogous to cinematography; a
work of drawing, painting, architecture, sculpture,
engraving or lithography; a photographic work to which
are assimilated works expressed by a process analogous to
photography; a work of applied art; an illustration, map,
plan, sketch or three-dimensional work relative to
geography, topography, architecture or science; a
performance; a broadcast; a phonogram; a compilation of
data to the extent it is protected as a copyrightable
work; or a work performed by a variety or circus
performer to the extent it is not otherwise considered a
literary or artistic work.
\item \textbf{``You''} means an individual or entity
exercising rights under this License who has not
previously violated the terms of this License with
respect to the Work, or who has received express
permission from the Licensor to exercise rights under
this License despite a previous violation.
\item \textbf{``Publicly Perform''} means to perform
public recitations of the Work and to communicate to the
public those public recitations, by any means or process,
including by wire or wireless means or public digital
performances; to make available to the public Works in
such a way that members of the public may access these
Works from a place and at a place individually chosen by
them; to perform the Work to the public by any means or
process and the communication to the public of the
performances of the Work, including by public digital
performance; to broadcast and rebroadcast the Work by any
means including signs, sounds or images.
\item \textbf{``Reproduce''} means to make copies of
the Work by any means including without limitation by
sound or visual recordings and the right of fixation and
reproducing fixations of the Work, including storage of a
protected performance or phonogram in digital form or
other electronic medium.
\end{enumerate}
\par \textbf{2. Fair Dealing Rights.} Nothing in this
License is intended to reduce, limit, or restrict any uses
free from copyright or rights arising from limitations or
exceptions that are provided for in connection with the
copyright protection under copyright law or other
applicable laws.
\par \textbf{3. License Grant.} Subject to the terms
and conditions of this License, Licensor hereby grants You
a worldwide, royalty-free, non-exclusive, perpetual (for
the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:
\begin{enumerate}
\item to Reproduce the Work, to incorporate the Work into
one or more Collections, and to Reproduce the Work as
incorporated in the Collections; and,
\item to Distribute and Publicly Perform the Work including
as incorporated in Collections.
\end{enumerate}
\par The above rights may be exercised in all media and
formats whether now known or hereafter devised. The above
rights include the right to make such modifications as are
technically necessary to exercise the rights in other media
and formats, but otherwise you have no rights to make
Adaptations. Subject to 8(f), all rights not expressly
granted by Licensor are hereby reserved, including but not
limited to the rights set forth in Section 4(d).
\par \textbf{4. Restrictions.} The license granted in
Section 3 above is expressly made subject to and limited by
the following restrictions:
\begin{enumerate}
\item You may Distribute or Publicly Perform the Work only
under the terms of this License. You must include a copy
of, or the Uniform Resource Identifier (URI) for, this
License with every copy of the Work You Distribute or
Publicly Perform. You may not offer or impose any terms
on the Work that restrict the terms of this License or
the ability of the recipient of the Work to exercise the
rights granted to that recipient under the terms of the
License. You may not sublicense the Work. You must keep
intact all notices that refer to this License and to the
disclaimer of warranties with every copy of the Work You
Distribute or Publicly Perform. When You Distribute or
Publicly Perform the Work, You may not impose any
effective technological measures on the Work that
restrict the ability of a recipient of the Work from You
to exercise the rights granted to that recipient under
the terms of the License. This Section 4(a) applies to
the Work as incorporated in a Collection, but this does
not require the Collection apart from the Work itself to
be made subject to the terms of this License. If You
create a Collection, upon notice from any Licensor You
must, to the extent practicable, remove from the
Collection any credit as required by Section 4(c), as
requested.
\item You may not exercise any of the rights granted to You
in Section 3 above in any manner that is primarily
intended for or directed toward commercial advantage or
private monetary compensation. The exchange of the Work
for other copyrighted works by means of digital
file-sharing or otherwise shall not be considered to be
intended for or directed toward commercial advantage or
private monetary compensation, provided there is no
payment of any monetary compensation in connection with
the exchange of copyrighted works.
\item If You Distribute, or Publicly Perform the Work or
Collections, You must, unless a request has been made
pursuant to Section 4(a), keep intact all copyright
notices for the Work and provide, reasonable to the
medium or means You are utilizing: (i) the name of the
Original Author (or pseudonym, if applicable) if
supplied, and/or if the Original Author and/or Licensor
designate another party or parties (e.g., a sponsor
institute, publishing entity, journal) for attribution
(``Attribution Parties'') in Licensor's copyright notice,
terms of service or by other reasonable means, the name
of such party or parties; (ii) the title of the Work if
supplied; (iii) to the extent reasonably practicable, the
URI, if any, that Licensor specifies to be associated
with the Work, unless such URI does not refer to the
copyright notice or licensing information for the Work.
The credit required by this Section 4(c) may be
implemented in any reasonable manner; provided, however,
that in the case of a Collection, at a minimum such
credit will appear, if a credit for all contributing
authors of Collection appears, then as part of these
credits and in a manner at least as prominent as the
credits for the other contributing authors. For the
avoidance of doubt, You may only use the credit required
by this Section for the purpose of attribution in the
manner set out above and, by exercising Your rights under
this License, You may not implicitly or explicitly assert
or imply any connection with, sponsorship or endorsement
by the Original Author, Licensor and/or Attribution
Parties, as appropriate, of You or Your use of the Work,
without the separate, express prior written permission of
the Original Author, Licensor and/or Attribution
Parties.
\item 
\par For the avoidance of doubt:
\begin{enumerate}
\item \textbf{Non-waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme cannot be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License;
\item \textbf{Waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme can be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License if Your exercise of such
rights is for a purpose or use which is otherwise
than noncommercial as permitted under Section 4(b)
and otherwise waives the right to collect royalties
through any statutory or compulsory licensing scheme;
and,
\item \textbf{Voluntary License Schemes}. The
Licensor reserves the right to collect royalties,
whether individually or, in the event that the
Licensor is a member of a collecting society that
administers voluntary licensing schemes, via that
society, from any exercise by You of the rights
granted under this License that is for a purpose or
use which is otherwise than noncommercial as
permitted under Section 4(b).
\end{enumerate}

\item Except as otherwise agreed in writing by the Licensor
or as may be otherwise permitted by applicable law, if
You Reproduce, Distribute or Publicly Perform the Work
either by itself or as part of any Collections, You must
not distort, mutilate, modify or take other derogatory
action in relation to the Work which would be prejudicial
to the Original Author's honor or reputation.
\end{enumerate}
\par \textbf{5. Representations, Warranties and
Disclaimer}
\par UNLESS OTHERWISE MUTUALLY AGREED BY THE PARTIES IN
WRITING, LICENSOR OFFERS THE WORK AS-IS AND MAKES NO
REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING,
WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE
ABSENCE OF LATENT OR OTHER DEFECTS, ACCURACY, OR THE
PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT DISCOVERABLE.
SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.
\par \textbf{6. Limitation on Liability.} EXCEPT TO
THE EXTENT REQUIRED BY APPLICABLE LAW, IN NO EVENT WILL
LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR ANY
SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY
DAMAGES ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK,
EVEN IF LICENSOR HAS BEEN ADVISED OF THE POSSIBILITY OF
SUCH DAMAGES.
\par \textbf{7. Termination}
\begin{enumerate}
\item This License and the rights granted hereunder will
terminate automatically upon any breach by You of the
terms of this License. Individuals or entities who have
received Collections from You under this License,
however, will not have their licenses terminated provided
such individuals or entities remain in full compliance
with those licenses. Sections 1, 2, 5, 6, 7, and 8 will
survive any termination of this License.
\item Subject to the above terms and conditions, the
license granted here is perpetual (for the duration of
the applicable copyright in the Work). Notwithstanding
the above, Licensor reserves the right to release the
Work under different license terms or to stop
distributing the Work at any time; provided, however that
any such election will not serve to withdraw this License
(or any other license that has been, or is required to
be, granted under the terms of this License), and this
License will continue in full force and effect unless
terminated as stated above.
\end{enumerate}
\par \textbf{8. Miscellaneous}
\begin{enumerate}
\item Each time You Distribute or Publicly Perform the Work
or a Collection, the Licensor offers to the recipient a
license to the Work on the same terms and conditions as
the license granted to You under this License.
\item If any provision of this License is invalid or
unenforceable under applicable law, it shall not affect
the validity or enforceability of the remainder of the
terms of this License, and without further action by the
parties to this agreement, such provision shall be
reformed to the minimum extent necessary to make such
provision valid and enforceable.
\item No term or provision of this License shall be deemed
waived and no breach consented to unless such waiver or
consent shall be in writing and signed by the party to be
charged with such waiver or consent.
\item This License constitutes the entire agreement between
the parties with respect to the Work licensed here. There
are no understandings, agreements or representations with
respect to the Work not specified here. Licensor shall
not be bound by any additional provisions that may appear
in any communication from You. This License may not be
modified without the mutual written agreement of the
Licensor and You.
\item The rights granted under, and the subject matter
referenced, in this License were drafted utilizing the
terminology of the Berne Convention for the Protection of
Literary and Artistic Works (as amended on September 28,
1979), the Rome Convention of 1961, the WIPO Copyright
Treaty of 1996, the WIPO Performances and Phonograms
Treaty of 1996 and the Universal Copyright Convention (as
revised on July 24, 1971). These rights and subject
matter take effect in the relevant jurisdiction in which
the License terms are sought to be enforced according to
the corresponding provisions of the implementation of
those treaty provisions in the applicable national law.
If the standard suite of rights granted under applicable
copyright law includes additional rights not granted
under this License, such additional rights are deemed to
be included in the License; this License is not intended
to restrict the license of any rights under applicable
law.
\end{enumerate}
 
\begin{quotation}
\subsubsection{Creative Commons Notice}
\par Creative Commons is not a party to this License, and
makes no warranty whatsoever in connection with the Work.
Creative Commons will not be liable to You or any party
on any legal theory for any damages whatsoever, including
without limitation any general, special, incidental or
consequential damages arising in connection to this
license. Notwithstanding the foregoing two (2) sentences,
if Creative Commons has expressly identified itself as
the Licensor hereunder, it shall have all rights and
obligations of Licensor.
\par Except for the limited purpose of indicating to the
public that the Work is licensed under the CCPL, Creative
Commons does not authorize the use by either party of the
trademark ``Creative Commons'' or any related trademark or
logo of Creative Commons without the prior written
consent of Creative Commons. Any permitted use will be in
compliance with Creative Commons' then-current trademark
usage guidelines, as may be published on its website or
otherwise made available upon request from time to time.
For the avoidance of doubt, this trademark restriction
does not form part of this License.
\par Creative Commons may be contacted at \url{https://creativecommons.org/}.
\end{quotation}



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nc-nd-3.0-plaintext.tex <==
Creative Commons Legal Code

Attribution-NonCommercial-NoDerivs 3.0 Unported

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR
    DAMAGES RESULTING FROM ITS USE.

License

THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS OF THIS CREATIVE
COMMONS PUBLIC LICENSE ("CCPL" OR "LICENSE"). THE WORK IS PROTECTED BY
COPYRIGHT AND/OR OTHER APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS PROHIBITED.

BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU ACCEPT AND AGREE
TO BE BOUND BY THE TERMS OF THIS LICENSE. TO THE EXTENT THIS LICENSE MAY
BE CONSIDERED TO BE A CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS
CONTAINED HERE IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.

1. Definitions

 a. "Adaptation" means a work based upon the Work, or upon the Work and
    other pre-existing works, such as a translation, adaptation,
    derivative work, arrangement of music or other alterations of a
    literary or artistic work, or phonogram or performance and includes
    cinematographic adaptations or any other form in which the Work may be
    recast, transformed, or adapted including in any form recognizably
    derived from the original, except that a work that constitutes a
    Collection will not be considered an Adaptation for the purpose of
    this License. For the avoidance of doubt, where the Work is a musical
    work, performance or phonogram, the synchronization of the Work in
    timed-relation with a moving image ("synching") will be considered an
    Adaptation for the purpose of this License.
 b. "Collection" means a collection of literary or artistic works, such as
    encyclopedias and anthologies, or performances, phonograms or
    broadcasts, or other works or subject matter other than works listed
    in Section 1(f) below, which, by reason of the selection and
    arrangement of their contents, constitute intellectual creations, in
    which the Work is included in its entirety in unmodified form along
    with one or more other contributions, each constituting separate and
    independent works in themselves, which together are assembled into a
    collective whole. A work that constitutes a Collection will not be
    considered an Adaptation (as defined above) for the purposes of this
    License.
 c. "Distribute" means to make available to the public the original and
    copies of the Work through sale or other transfer of ownership.
 d. "Licensor" means the individual, individuals, entity or entities that
    offer(s) the Work under the terms of this License.
 e. "Original Author" means, in the case of a literary or artistic work,
    the individual, individuals, entity or entities who created the Work
    or if no individual or entity can be identified, the publisher; and in
    addition (i) in the case of a performance the actors, singers,
    musicians, dancers, and other persons who act, sing, deliver, declaim,
    play in, interpret or otherwise perform literary or artistic works or
    expressions of folklore; (ii) in the case of a phonogram the producer
    being the person or legal entity who first fixes the sounds of a
    performance or other sounds; and, (iii) in the case of broadcasts, the
    organization that transmits the broadcast.
 f. "Work" means the literary and/or artistic work offered under the terms
    of this License including without limitation any production in the
    literary, scientific and artistic domain, whatever may be the mode or
    form of its expression including digital form, such as a book,
    pamphlet and other writing; a lecture, address, sermon or other work
    of the same nature; a dramatic or dramatico-musical work; a
    choreographic work or entertainment in dumb show; a musical
    composition with or without words; a cinematographic work to which are
    assimilated works expressed by a process analogous to cinematography;
    a work of drawing, painting, architecture, sculpture, engraving or
    lithography; a photographic work to which are assimilated works
    expressed by a process analogous to photography; a work of applied
    art; an illustration, map, plan, sketch or three-dimensional work
    relative to geography, topography, architecture or science; a
    performance; a broadcast; a phonogram; a compilation of data to the
    extent it is protected as a copyrightable work; or a work performed by
    a variety or circus performer to the extent it is not otherwise
    considered a literary or artistic work.
 g. "You" means an individual or entity exercising rights under this
    License who has not previously violated the terms of this License with
    respect to the Work, or who has received express permission from the
    Licensor to exercise rights under this License despite a previous
    violation.
 h. "Publicly Perform" means to perform public recitations of the Work and
    to communicate to the public those public recitations, by any means or
    process, including by wire or wireless means or public digital
    performances; to make available to the public Works in such a way that
    members of the public may access these Works from a place and at a
    place individually chosen by them; to perform the Work to the public
    by any means or process and the communication to the public of the
    performances of the Work, including by public digital performance; to
    broadcast and rebroadcast the Work by any means including signs,
    sounds or images.
 i. "Reproduce" means to make copies of the Work by any means including
    without limitation by sound or visual recordings and the right of
    fixation and reproducing fixations of the Work, including storage of a
    protected performance or phonogram in digital form or other electronic
    medium.

2. Fair Dealing Rights. Nothing in this License is intended to reduce,
limit, or restrict any uses free from copyright or rights arising from
limitations or exceptions that are provided for in connection with the
copyright protection under copyright law or other applicable laws.

3. License Grant. Subject to the terms and conditions of this License,
Licensor hereby grants You a worldwide, royalty-free, non-exclusive,
perpetual (for the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:

 a. to Reproduce the Work, to incorporate the Work into one or more
    Collections, and to Reproduce the Work as incorporated in the
    Collections; and,
 b. to Distribute and Publicly Perform the Work including as incorporated
    in Collections.

The above rights may be exercised in all media and formats whether now
known or hereafter devised. The above rights include the right to make
such modifications as are technically necessary to exercise the rights in
other media and formats, but otherwise you have no rights to make
Adaptations. Subject to 8(f), all rights not expressly granted by Licensor
are hereby reserved, including but not limited to the rights set forth in
Section 4(d).

4. Restrictions. The license granted in Section 3 above is expressly made
subject to and limited by the following restrictions:

 a. You may Distribute or Publicly Perform the Work only under the terms
    of this License. You must include a copy of, or the Uniform Resource
    Identifier (URI) for, this License with every copy of the Work You
    Distribute or Publicly Perform. You may not offer or impose any terms
    on the Work that restrict the terms of this License or the ability of
    the recipient of the Work to exercise the rights granted to that
    recipient under the terms of the License. You may not sublicense the
    Work. You must keep intact all notices that refer to this License and
    to the disclaimer of warranties with every copy of the Work You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Work, You may not impose any effective technological
    measures on the Work that restrict the ability of a recipient of the
    Work from You to exercise the rights granted to that recipient under
    the terms of the License. This Section 4(a) applies to the Work as
    incorporated in a Collection, but this does not require the Collection
    apart from the Work itself to be made subject to the terms of this
    License. If You create a Collection, upon notice from any Licensor You
    must, to the extent practicable, remove from the Collection any credit
    as required by Section 4(c), as requested.
 b. You may not exercise any of the rights granted to You in Section 3
    above in any manner that is primarily intended for or directed toward
    commercial advantage or private monetary compensation. The exchange of
    the Work for other copyrighted works by means of digital file-sharing
    or otherwise shall not be considered to be intended for or directed
    toward commercial advantage or private monetary compensation, provided
    there is no payment of any monetary compensation in connection with
    the exchange of copyrighted works.
 c. If You Distribute, or Publicly Perform the Work or Collections, You
    must, unless a request has been made pursuant to Section 4(a), keep
    intact all copyright notices for the Work and provide, reasonable to
    the medium or means You are utilizing: (i) the name of the Original
    Author (or pseudonym, if applicable) if supplied, and/or if the
    Original Author and/or Licensor designate another party or parties
    (e.g., a sponsor institute, publishing entity, journal) for
    attribution ("Attribution Parties") in Licensor's copyright notice,
    terms of service or by other reasonable means, the name of such party
    or parties; (ii) the title of the Work if supplied; (iii) to the
    extent reasonably practicable, the URI, if any, that Licensor
    specifies to be associated with the Work, unless such URI does not
    refer to the copyright notice or licensing information for the Work.
    The credit required by this Section 4(c) may be implemented in any
    reasonable manner; provided, however, that in the case of a
    Collection, at a minimum such credit will appear, if a credit for all
    contributing authors of Collection appears, then as part of these
    credits and in a manner at least as prominent as the credits for the
    other contributing authors. For the avoidance of doubt, You may only
    use the credit required by this Section for the purpose of attribution
    in the manner set out above and, by exercising Your rights under this
    License, You may not implicitly or explicitly assert or imply any
    connection with, sponsorship or endorsement by the Original Author,
    Licensor and/or Attribution Parties, as appropriate, of You or Your
    use of the Work, without the separate, express prior written
    permission of the Original Author, Licensor and/or Attribution
    Parties.
 d. For the avoidance of doubt:

     i. Non-waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme cannot be waived, the Licensor
        reserves the exclusive right to collect such royalties for any
        exercise by You of the rights granted under this License;
    ii. Waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme can be waived, the Licensor reserves
        the exclusive right to collect such royalties for any exercise by
        You of the rights granted under this License if Your exercise of
        such rights is for a purpose or use which is otherwise than
        noncommercial as permitted under Section 4(b) and otherwise waives
        the right to collect royalties through any statutory or compulsory
        licensing scheme; and,
   iii. Voluntary License Schemes. The Licensor reserves the right to
        collect royalties, whether individually or, in the event that the
        Licensor is a member of a collecting society that administers
        voluntary licensing schemes, via that society, from any exercise
        by You of the rights granted under this License that is for a
        purpose or use which is otherwise than noncommercial as permitted
        under Section 4(b).
 e. Except as otherwise agreed in writing by the Licensor or as may be
    otherwise permitted by applicable law, if You Reproduce, Distribute or
    Publicly Perform the Work either by itself or as part of any
    Collections, You must not distort, mutilate, modify or take other
    derogatory action in relation to the Work which would be prejudicial
    to the Original Author's honor or reputation.

5. Representations, Warranties and Disclaimer

UNLESS OTHERWISE MUTUALLY AGREED BY THE PARTIES IN WRITING, LICENSOR
OFFERS THE WORK AS-IS AND MAKES NO REPRESENTATIONS OR WARRANTIES OF ANY
KIND CONCERNING THE WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE,
INCLUDING, WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE ABSENCE OF
LATENT OR OTHER DEFECTS, ACCURACY, OR THE PRESENCE OF ABSENCE OF ERRORS,
WHETHER OR NOT DISCOVERABLE. SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION
OF IMPLIED WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.

6. Limitation on Liability. EXCEPT TO THE EXTENT REQUIRED BY APPLICABLE
LAW, IN NO EVENT WILL LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR
ANY SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY DAMAGES
ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK, EVEN IF LICENSOR HAS
BEEN ADVISED OF THE POSSIBILITY OF SUCH DAMAGES.

7. Termination

 a. This License and the rights granted hereunder will terminate
    automatically upon any breach by You of the terms of this License.
    Individuals or entities who have received Collections from You under
    this License, however, will not have their licenses terminated
    provided such individuals or entities remain in full compliance with
    those licenses. Sections 1, 2, 5, 6, 7, and 8 will survive any
    termination of this License.
 b. Subject to the above terms and conditions, the license granted here is
    perpetual (for the duration of the applicable copyright in the Work).
    Notwithstanding the above, Licensor reserves the right to release the
    Work under different license terms or to stop distributing the Work at
    any time; provided, however that any such election will not serve to
    withdraw this License (or any other license that has been, or is
    required to be, granted under the terms of this License), and this
    License will continue in full force and effect unless terminated as
    stated above.

8. Miscellaneous

 a. Each time You Distribute or Publicly Perform the Work or a Collection,
    the Licensor offers to the recipient a license to the Work on the same
    terms and conditions as the license granted to You under this License.
 b. If any provision of this License is invalid or unenforceable under
    applicable law, it shall not affect the validity or enforceability of
    the remainder of the terms of this License, and without further action
    by the parties to this agreement, such provision shall be reformed to
    the minimum extent necessary to make such provision valid and
    enforceable.
 c. No term or provision of this License shall be deemed waived and no
    breach consented to unless such waiver or consent shall be in writing
    and signed by the party to be charged with such waiver or consent.
 d. This License constitutes the entire agreement between the parties with
    respect to the Work licensed here. There are no understandings,
    agreements or representations with respect to the Work not specified
    here. Licensor shall not be bound by any additional provisions that
    may appear in any communication from You. This License may not be
    modified without the mutual written agreement of the Licensor and You.
 e. The rights granted under, and the subject matter referenced, in this
    License were drafted utilizing the terminology of the Berne Convention
    for the Protection of Literary and Artistic Works (as amended on
    September 28, 1979), the Rome Convention of 1961, the WIPO Copyright
    Treaty of 1996, the WIPO Performances and Phonograms Treaty of 1996
    and the Universal Copyright Convention (as revised on July 24, 1971).
    These rights and subject matter take effect in the relevant
    jurisdiction in which the License terms are sought to be enforced
    according to the corresponding provisions of the implementation of
    those treaty provisions in the applicable national law. If the
    standard suite of rights granted under applicable copyright law
    includes additional rights not granted under this License, such
    additional rights are deemed to be included in the License; this
    License is not intended to restrict the license of any rights under
    applicable law.


Creative Commons Notice

    Creative Commons is not a party to this License, and makes no warranty
    whatsoever in connection with the Work. Creative Commons will not be
    liable to You or any party on any legal theory for any damages
    whatsoever, including without limitation any general, special,
    incidental or consequential damages arising in connection to this
    license. Notwithstanding the foregoing two (2) sentences, if Creative
    Commons has expressly identified itself as the Licensor hereunder, it
    shall have all rights and obligations of Licensor.

    Except for the limited purpose of indicating to the public that the
    Work is licensed under the CCPL, Creative Commons does not authorize
    the use by either party of the trademark "Creative Commons" or any
    related trademark or logo of Creative Commons without the prior
    written consent of Creative Commons. Any permitted use will be in
    compliance with Creative Commons' then-current trademark usage
    guidelines, as may be published on its website or otherwise made
    available upon request from time to time. For the avoidance of doubt,
    this trademark restriction does not form part of this License.

    Creative Commons may be contacted at https://creativecommons.org/.


==> license-texts/doclicense-CC-by-nc-nd-4.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NonCommercial-NoDerivatives 4.0 International}







Official translations of this license are available in other languages.



\par Creative Commons Corporation (“Creative Commons”) is not a law firm and does not provide legal services or legal advice. Distribution of Creative Commons public licenses does not create a lawyer-client or other relationship. Creative Commons makes its licenses and related information available on an “as-is” basis. Creative Commons gives no warranties regarding its licenses, any material licensed under their terms and conditions, or any related information. Creative Commons disclaims all liability for damages resulting from their use to the fullest extent possible.


\par \textbf{Using Creative Commons Public Licenses}
\par Creative Commons public licenses provide a standard set of terms and conditions that creators and other rights holders may use to share original works of authorship and other material subject to copyright and certain other rights specified in the public license below. The following considerations are for informational purposes only, are not exhaustive, and do not form part of our licenses.
\begin{quotation}\textbf{Considerations for licensors:} Our public licenses are intended for use by those authorized to give the public permission to use material in ways otherwise restricted by copyright and certain other rights. Our licenses are irrevocable. Licensors should read and understand the terms and conditions of the license they choose before applying it. Licensors should also secure all rights necessary before applying our licenses so that the public can reuse the material as expected. Licensors should clearly mark any material not subject to the license. This includes other CC-licensed material, or material used under an exception or limitation to copyright. More considerations for licensors.\end{quotation}
\begin{quotation}\textbf{Considerations for the public:} By using one of our public licenses, a licensor grants the public permission to use the licensed material under specified terms and conditions. If the licensor’s permission is not necessary for any reason–for example, because of any applicable exception or limitation to copyright–then that use is not regulated by the license. Our licenses grant only permissions under copyright and certain other rights that a licensor has authority to grant. Use of the licensed material may still be restricted for other reasons, including because others have copyright or other rights in the material. A licensor may make special requests, such as asking that all changes be marked or described. Although not required by our licenses, you are encouraged to respect those requests where reasonable.
More considerations for the public.\end{quotation}

\subsubsection{Creative Commons Attribution-NonCommercial-NoDerivatives 4.0 International Public License}
\par By exercising the Licensed Rights (defined below), You accept and agree to be bound by the terms and conditions of this Creative Commons Attribution-NonCommercial-NoDerivatives 4.0 International Public License (``Public License''). To the extent this Public License may be interpreted as a contract, You are granted the Licensed Rights in consideration of Your acceptance of these terms and conditions, and the Licensor grants You such rights in consideration of benefits the Licensor receives from making the Licensed Material available under these terms and conditions.
\par \textbf{Section 1 – Definitions.}
\begin{enumerate}
\item \textbf{Adapted Material} means material subject to Copyright and Similar Rights that is derived from or based upon the Licensed Material and in which the Licensed Material is translated, altered, arranged, transformed, or otherwise modified in a manner requiring permission under the Copyright and Similar Rights held by the Licensor. For purposes of this Public License, where the Licensed Material is a musical work, performance, or sound recording, Adapted Material is always produced where the Licensed Material is synched in timed relation with a moving image.
\item \textbf{Copyright and Similar Rights} means copyright and/or similar rights closely related to copyright including, without limitation, performance, broadcast, sound recording, and Sui Generis Database Rights, without regard to how the rights are labeled or categorized. For purposes of this Public License, the rights specified in Section 2(b)(1)-(2) are not Copyright and Similar Rights.
\item \textbf{Effective Technological Measures} means those measures that, in the absence of proper authority, may not
be circumvented under laws fulfilling obligations under Article 11 of the WIPO Copyright Treaty adopted on December 20, 1996, and/or similar
international agreements.
\item \textbf{Exceptions and Limitations} means fair use, fair dealing, and/or any other exception or limitation to Copyright and Similar Rights that applies to Your use of the Licensed Material.
\item \textbf{Licensed Material} means the artistic or literary work, database, or other material to which the Licensor applied this Public License.
\item \textbf{Licensed Rights} means the rights granted to You subject to the terms and conditions of this Public License, which are limited to all Copyright and Similar Rights that apply to Your use of the Licensed Material and that the Licensor has authority to license.
\item \textbf{Licensor} means the individual(s) or entity(ies) granting rights under this Public License.
\item \textbf{NonCommercial} means not primarily intended for or directed towards commercial advantage or monetary compensation. For purposes of this Public License, the exchange of the Licensed Material for other material subject to Copyright and Similar Rights by digital file-sharing or similar means is NonCommercial provided there is no payment of monetary compensation in connection with the exchange.
\item \textbf{Share} means to provide material to the public by any means or process that requires permission under the Licensed Rights, such as reproduction, public display, public performance, distribution, dissemination, communication, or importation, and to make material available to the public including in ways that members of the public may access the material from a place and at a time individually chosen by them.
\item \textbf{Sui Generis Database Rights} means rights other than copyright resulting from Directive 96/9/EC of the European Parliament and of the Council of 11 March 1996 on the legal protection of databases, as amended and/or succeeded, as well as other essentially equivalent rights anywhere in the world.
\item \textbf{You} means the individual or entity exercising the Licensed Rights under this Public License. \textbf{Your} has a corresponding meaning.
\end{enumerate}
\par \textbf{Section 2 – Scope.}
\begin{enumerate}
\item \textbf{License grant}.
\begin{enumerate}
\item Subject to the terms and conditions of this Public License, the Licensor hereby grants You a worldwide, royalty-free, non-sublicensable, non-exclusive, irrevocable license to exercise the Licensed Rights in the Licensed Material to:
\begin{enumerate}
\item reproduce and Share the Licensed Material, in whole or in part, for NonCommercial purposes only; and
\item produce and reproduce, but not Share, Adapted Material for NonCommercial purposes only.
\end{enumerate}
\item Exceptions and Limitations. For the avoidance of doubt, where Exceptions and Limitations apply to Your use, this Public License does not apply, and You do not need to comply with its terms and conditions.
\item Term. The term of this Public License is specified in Section 6(a).
\item Media and formats; technical modifications allowed. The Licensor authorizes You to exercise the Licensed Rights in all media and formats whether now known or hereafter created, and to make technical modifications necessary to do so. The Licensor waives and/or agrees not to assert any right or authority to forbid You from making technical modifications necessary to exercise the Licensed Rights, including technical modifications necessary to circumvent Effective Technological Measures. For purposes of this Public License, simply making modifications authorized by this Section 2(a)(4) never produces Adapted Material.
\item Downstream recipients.

\begin{enumerate}
\item Offer from the Licensor – Licensed Material. Every recipient of the Licensed Material automatically receives an offer from the Licensor to exercise the Licensed Rights under the terms and conditions of this Public License.
\item No downstream restrictions. You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, the Licensed Material if doing so restricts exercise of the Licensed Rights by any recipient of the Licensed Material.
\end{enumerate}

\item No endorsement. Nothing in this Public License constitutes or may be construed as permission to assert or imply that You are, or that Your use of the Licensed Material is, connected with, or sponsored, endorsed, or granted official status by, the Licensor or others designated to receive attribution as provided in Section 3(a)(1)(A)(i).
\end{enumerate}
\item \par \textbf{Other rights}.
\begin{enumerate}
\item Moral rights, such as the right of integrity, are not licensed under this Public License, nor are publicity, privacy, and/or other similar personality rights; however, to the extent possible, the Licensor waives and/or agrees not to assert any such rights held by the Licensor to the limited extent necessary to allow You to exercise the Licensed Rights, but not otherwise.
\item Patent and trademark rights are not licensed under this Public License.
\item To the extent possible, the Licensor waives any right to collect royalties from You for the exercise of the Licensed Rights, whether directly or through a collecting society under any voluntary or waivable statutory or compulsory licensing scheme. In all other cases the Licensor expressly reserves any right to collect such royalties, including when the Licensed Material is used other than for NonCommercial purposes.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 3 – License Conditions.}
\par Your exercise of the Licensed Rights is expressly made subject to the following conditions.
\begin{enumerate}
\item \par \textbf{Attribution}.
\begin{enumerate}
\item \par If You Share the Licensed Material, You must:
\begin{enumerate}
\item retain the following if it is supplied by the Licensor with the Licensed Material:
\begin{enumerate}
\item identification of the creator(s) of the Licensed Material and any others designated to receive attribution, in any reasonable manner requested by the Licensor (including by pseudonym if designated);
\item a copyright notice;
\item a notice that refers to this Public License; 
\item a notice that refers to the disclaimer of warranties;
\item a URI or hyperlink to the Licensed Material to the extent reasonably practicable;
\end{enumerate}
\item indicate if You modified the Licensed Material and retain an indication of any previous modifications; and
\item indicate the Licensed Material is licensed under this Public License,
and include the text of, or the URI or hyperlink to, this Public
License.
\end{enumerate}
For the avoidance of doubt, You do not have permission under this Public License to Share Adapted Material.

\item You may satisfy the conditions in Section 3(a)(1) in any reasonable manner based on the medium, means, and context in which You Share the Licensed Material. For example, it may be reasonable to satisfy the conditions by providing a URI or hyperlink to a resource that includes the required information.
\item If requested by the Licensor, You must remove any of the information required by Section 3(a)(1)(A) to the extent reasonably practicable.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 4 – Sui Generis Database Rights.}
\par Where the Licensed Rights include Sui Generis Database Rights that apply to Your use of the Licensed Material:
\begin{enumerate}
\item for the avoidance of doubt, Section 2(a)(1) grants You the right to extract, reuse, reproduce, and Share all or a substantial portion of the contents of the database for NonCommercial purposes only and provided You do not Share Adapted Material;
\item if You include all or a substantial portion of the database contents in a database in which You have Sui Generis Database Rights, then the database in which You have Sui Generis Database Rights (but not its individual contents) is Adapted Material; and
\item You must comply with the conditions in Section 3(a) if You Share all or a substantial portion of the contents of the database.
\end{enumerate}
For the avoidance of doubt, this Section 4 supplements and does not replace Your obligations under this Public License where the Licensed Rights include other Copyright and Similar Rights.
\par \textbf{Section 5 – Disclaimer of Warranties and Limitation of Liability.}
\begin{enumerate}
\item \textbf{Unless otherwise separately undertaken by the Licensor, to the extent possible, the Licensor offers the Licensed Material as-is and as-available, and makes no representations or warranties of any kind concerning the Licensed Material, whether express, implied, statutory, or other. This includes, without limitation, warranties of title, merchantability, fitness for a particular purpose, non-infringement, absence of latent or other defects, accuracy, or the presence or absence of errors, whether or not known or discoverable. Where disclaimers of warranties are not allowed in full or in part, this disclaimer may not apply to You.}
\item \textbf{To the extent possible, in no event will the Licensor be liable to You on any legal theory (including, without limitation, negligence) or otherwise for any direct, special, indirect, incidental, consequential, punitive, exemplary, or other losses, costs, expenses, or damages arising out of this Public License or use of the Licensed Material, even if the Licensor has been advised of the possibility of such losses, costs, expenses, or damages. Where a limitation of liability is not allowed in full or in part, this limitation may not apply to You.}
\end{enumerate}
\begin{enumerate}
\item The disclaimer of warranties and limitation of liability provided above shall be interpreted in a manner that, to the extent possible, most closely approximates an absolute disclaimer and waiver of all liability.
\end{enumerate}
\par \textbf{Section 6 – Term and Termination.}
\begin{enumerate}
\item This Public License applies for the term of the Copyright and Similar Rights licensed here. However, if You fail to comply with this Public License, then Your rights under this Public License terminate automatically.
\item 
\par Where Your right to use the Licensed Material has terminated under Section 6(a), it reinstates:
\begin{enumerate}
\item automatically as of the date the violation is cured, provided it is cured within 30 days of Your discovery of the violation; or
\item upon express reinstatement by the Licensor.
\end{enumerate}
For the avoidance of doubt, this Section 6(b) does not affect any right the Licensor may have to seek remedies for Your violations of this Public License.
\item For the avoidance of doubt, the Licensor may also offer the Licensed Material under separate terms or conditions or stop distributing the Licensed Material at any time; however, doing so will not terminate this Public License.
\item Sections 1, 5, 6, 7, and 8 survive termination of this Public License.
\end{enumerate}
\par \textbf{Section 7 – Other Terms and Conditions.}
\begin{enumerate}
\item The Licensor shall not be bound by any additional or different terms or conditions communicated by You unless expressly agreed.
\item Any arrangements, understandings, or agreements regarding the Licensed Material not stated herein are separate from and independent of the terms and conditions of this Public License.
\end{enumerate}
\par \textbf{Section 8 – Interpretation.}
\begin{enumerate}
\item For the avoidance of doubt, this Public License does not, and shall not be interpreted to, reduce, limit, restrict, or impose conditions on any use of the Licensed Material that could lawfully be made without permission under this Public License.
\item To the extent possible, if any provision of this Public License is deemed unenforceable, it shall be automatically reformed to the minimum extent necessary to make it enforceable. If the provision cannot be reformed, it shall be severed from this Public License without affecting the enforceability of the remaining terms and conditions.
\item No term or condition of this Public License will be waived and no failure to comply consented to unless expressly agreed to by the Licensor.
\item Nothing in this Public License constitutes or may be interpreted as a limitation upon, or waiver of, any privileges and immunities that apply to the Licensor or You, including from the legal processes of any jurisdiction or authority.
\end{enumerate}
\par Creative Commons is not a party to its public licenses. Notwithstanding, Creative Commons may elect to apply one of its public licenses to material it publishes and in those instances will be considered the “Licensor.” The text of the Creative Commons public licenses is dedicated to the public domain under the CC0 Public Domain Dedication. Except for the limited purpose of indicating that material is shared under a Creative Commons public license or as otherwise permitted by the Creative Commons policies published at creativecommons.org/policies, Creative Commons does not authorize the use of the trademark “Creative Commons” or any other trademark or logo of Creative Commons without its prior written consent including, without limitation, in connection with any unauthorized modifications to any of its public licenses or any other arrangements, understandings, or agreements concerning use of licensed material. For the avoidance of doubt, this paragraph does not form part of the public licenses.\\\\
Creative Commons may be contacted at creativecommons.org.
\par Additional languages available: Bahasa Indonesia, Nederlands, norsk, suomeksi, te reo Māori, українська, 日本語. Please read the FAQ for more information about official translations.



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nc-nd-4.0-plaintext.tex <==
Attribution-NonCommercial-NoDerivatives 4.0 International

=======================================================================

Creative Commons Corporation ("Creative Commons") is not a law firm and
does not provide legal services or legal advice. Distribution of
Creative Commons public licenses does not create a lawyer-client or
other relationship. Creative Commons makes its licenses and related
information available on an "as-is" basis. Creative Commons gives no
warranties regarding its licenses, any material licensed under their
terms and conditions, or any related information. Creative Commons
disclaims all liability for damages resulting from their use to the
fullest extent possible.

Using Creative Commons Public Licenses

Creative Commons public licenses provide a standard set of terms and
conditions that creators and other rights holders may use to share
original works of authorship and other material subject to copyright
and certain other rights specified in the public license below. The
following considerations are for informational purposes only, are not
exhaustive, and do not form part of our licenses.

     Considerations for licensors: Our public licenses are
     intended for use by those authorized to give the public
     permission to use material in ways otherwise restricted by
     copyright and certain other rights. Our licenses are
     irrevocable. Licensors should read and understand the terms
     and conditions of the license they choose before applying it.
     Licensors should also secure all rights necessary before
     applying our licenses so that the public can reuse the
     material as expected. Licensors should clearly mark any
     material not subject to the license. This includes other CC-
     licensed material, or material used under an exception or
     limitation to copyright. More considerations for licensors:
	wiki.creativecommons.org/Considerations_for_licensors

     Considerations for the public: By using one of our public
     licenses, a licensor grants the public permission to use the
     licensed material under specified terms and conditions. If
     the licensor's permission is not necessary for any reason--for
     example, because of any applicable exception or limitation to
     copyright--then that use is not regulated by the license. Our
     licenses grant only permissions under copyright and certain
     other rights that a licensor has authority to grant. Use of
     the licensed material may still be restricted for other
     reasons, including because others have copyright or other
     rights in the material. A licensor may make special requests,
     such as asking that all changes be marked or described.
     Although not required by our licenses, you are encouraged to
     respect those requests where reasonable. More_considerations
     for the public: 
	wiki.creativecommons.org/Considerations_for_licensees

=======================================================================

Creative Commons Attribution-NonCommercial-NoDerivatives 4.0
International Public License

By exercising the Licensed Rights (defined below), You accept and agree
to be bound by the terms and conditions of this Creative Commons
Attribution-NonCommercial-NoDerivatives 4.0 International Public
License ("Public License"). To the extent this Public License may be
interpreted as a contract, You are granted the Licensed Rights in
consideration of Your acceptance of these terms and conditions, and the
Licensor grants You such rights in consideration of benefits the
Licensor receives from making the Licensed Material available under
these terms and conditions.


Section 1 -- Definitions.

  a. Adapted Material means material subject to Copyright and Similar
     Rights that is derived from or based upon the Licensed Material
     and in which the Licensed Material is translated, altered,
     arranged, transformed, or otherwise modified in a manner requiring
     permission under the Copyright and Similar Rights held by the
     Licensor. For purposes of this Public License, where the Licensed
     Material is a musical work, performance, or sound recording,
     Adapted Material is always produced where the Licensed Material is
     synched in timed relation with a moving image.

  b. Copyright and Similar Rights means copyright and/or similar rights
     closely related to copyright including, without limitation,
     performance, broadcast, sound recording, and Sui Generis Database
     Rights, without regard to how the rights are labeled or
     categorized. For purposes of this Public License, the rights
     specified in Section 2(b)(1)-(2) are not Copyright and Similar
     Rights.

  c. Effective Technological Measures means those measures that, in the
     absence of proper authority, may not be circumvented under laws
     fulfilling obligations under Article 11 of the WIPO Copyright
     Treaty adopted on December 20, 1996, and/or similar international
     agreements.

  d. Exceptions and Limitations means fair use, fair dealing, and/or
     any other exception or limitation to Copyright and Similar Rights
     that applies to Your use of the Licensed Material.

  e. Licensed Material means the artistic or literary work, database,
     or other material to which the Licensor applied this Public
     License.

  f. Licensed Rights means the rights granted to You subject to the
     terms and conditions of this Public License, which are limited to
     all Copyright and Similar Rights that apply to Your use of the
     Licensed Material and that the Licensor has authority to license.

  g. Licensor means the individual(s) or entity(ies) granting rights
     under this Public License.

  h. NonCommercial means not primarily intended for or directed towards
     commercial advantage or monetary compensation. For purposes of
     this Public License, the exchange of the Licensed Material for
     other material subject to Copyright and Similar Rights by digital
     file-sharing or similar means is NonCommercial provided there is
     no payment of monetary compensation in connection with the
     exchange.

  i. Share means to provide material to the public by any means or
     process that requires permission under the Licensed Rights, such
     as reproduction, public display, public performance, distribution,
     dissemination, communication, or importation, and to make material
     available to the public including in ways that members of the
     public may access the material from a place and at a time
     individually chosen by them.

  j. Sui Generis Database Rights means rights other than copyright
     resulting from Directive 96/9/EC of the European Parliament and of
     the Council of 11 March 1996 on the legal protection of databases,
     as amended and/or succeeded, as well as other essentially
     equivalent rights anywhere in the world.

  k. You means the individual or entity exercising the Licensed Rights
     under this Public License. Your has a corresponding meaning.


Section 2 -- Scope.

  a. License grant.

       1. Subject to the terms and conditions of this Public License,
          the Licensor hereby grants You a worldwide, royalty-free,
          non-sublicensable, non-exclusive, irrevocable license to
          exercise the Licensed Rights in the Licensed Material to:

            a. reproduce and Share the Licensed Material, in whole or
               in part, for NonCommercial purposes only; and

            b. produce and reproduce, but not Share, Adapted Material
               for NonCommercial purposes only.

       2. Exceptions and Limitations. For the avoidance of doubt, where
          Exceptions and Limitations apply to Your use, this Public
          License does not apply, and You do not need to comply with
          its terms and conditions.

       3. Term. The term of this Public License is specified in Section
          6(a).

       4. Media and formats; technical modifications allowed. The
          Licensor authorizes You to exercise the Licensed Rights in
          all media and formats whether now known or hereafter created,
          and to make technical modifications necessary to do so. The
          Licensor waives and/or agrees not to assert any right or
          authority to forbid You from making technical modifications
          necessary to exercise the Licensed Rights, including
          technical modifications necessary to circumvent Effective
          Technological Measures. For purposes of this Public License,
          simply making modifications authorized by this Section 2(a)
          (4) never produces Adapted Material.

       5. Downstream recipients.

            a. Offer from the Licensor -- Licensed Material. Every
               recipient of the Licensed Material automatically
               receives an offer from the Licensor to exercise the
               Licensed Rights under the terms and conditions of this
               Public License.

            b. No downstream restrictions. You may not offer or impose
               any additional or different terms or conditions on, or
               apply any Effective Technological Measures to, the
               Licensed Material if doing so restricts exercise of the
               Licensed Rights by any recipient of the Licensed
               Material.

       6. No endorsement. Nothing in this Public License constitutes or
          may be construed as permission to assert or imply that You
          are, or that Your use of the Licensed Material is, connected
          with, or sponsored, endorsed, or granted official status by,
          the Licensor or others designated to receive attribution as
          provided in Section 3(a)(1)(A)(i).

  b. Other rights.

       1. Moral rights, such as the right of integrity, are not
          licensed under this Public License, nor are publicity,
          privacy, and/or other similar personality rights; however, to
          the extent possible, the Licensor waives and/or agrees not to
          assert any such rights held by the Licensor to the limited
          extent necessary to allow You to exercise the Licensed
          Rights, but not otherwise.

       2. Patent and trademark rights are not licensed under this
          Public License.

       3. To the extent possible, the Licensor waives any right to
          collect royalties from You for the exercise of the Licensed
          Rights, whether directly or through a collecting society
          under any voluntary or waivable statutory or compulsory
          licensing scheme. In all other cases the Licensor expressly
          reserves any right to collect such royalties, including when
          the Licensed Material is used other than for NonCommercial
          purposes.


Section 3 -- License Conditions.

Your exercise of the Licensed Rights is expressly made subject to the
following conditions.

  a. Attribution.

       1. If You Share the Licensed Material, You must:

            a. retain the following if it is supplied by the Licensor
               with the Licensed Material:

                 i. identification of the creator(s) of the Licensed
                    Material and any others designated to receive
                    attribution, in any reasonable manner requested by
                    the Licensor (including by pseudonym if
                    designated);

                ii. a copyright notice;

               iii. a notice that refers to this Public License;

                iv. a notice that refers to the disclaimer of
                    warranties;

                 v. a URI or hyperlink to the Licensed Material to the
                    extent reasonably practicable;

            b. indicate if You modified the Licensed Material and
               retain an indication of any previous modifications; and

            c. indicate the Licensed Material is licensed under this
               Public License, and include the text of, or the URI or
               hyperlink to, this Public License.

          For the avoidance of doubt, You do not have permission under
          this Public License to Share Adapted Material.

       2. You may satisfy the conditions in Section 3(a)(1) in any
          reasonable manner based on the medium, means, and context in
          which You Share the Licensed Material. For example, it may be
          reasonable to satisfy the conditions by providing a URI or
          hyperlink to a resource that includes the required
          information.

       3. If requested by the Licensor, You must remove any of the
          information required by Section 3(a)(1)(A) to the extent
          reasonably practicable.


Section 4 -- Sui Generis Database Rights.

Where the Licensed Rights include Sui Generis Database Rights that
apply to Your use of the Licensed Material:

  a. for the avoidance of doubt, Section 2(a)(1) grants You the right
     to extract, reuse, reproduce, and Share all or a substantial
     portion of the contents of the database for NonCommercial purposes
     only and provided You do not Share Adapted Material;

  b. if You include all or a substantial portion of the database
     contents in a database in which You have Sui Generis Database
     Rights, then the database in which You have Sui Generis Database
     Rights (but not its individual contents) is Adapted Material; and

  c. You must comply with the conditions in Section 3(a) if You Share
     all or a substantial portion of the contents of the database.

For the avoidance of doubt, this Section 4 supplements and does not
replace Your obligations under this Public License where the Licensed
Rights include other Copyright and Similar Rights.


Section 5 -- Disclaimer of Warranties and Limitation of Liability.

  a. UNLESS OTHERWISE SEPARATELY UNDERTAKEN BY THE LICENSOR, TO THE
     EXTENT POSSIBLE, THE LICENSOR OFFERS THE LICENSED MATERIAL AS-IS
     AND AS-AVAILABLE, AND MAKES NO REPRESENTATIONS OR WARRANTIES OF
     ANY KIND CONCERNING THE LICENSED MATERIAL, WHETHER EXPRESS,
     IMPLIED, STATUTORY, OR OTHER. THIS INCLUDES, WITHOUT LIMITATION,
     WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
     PURPOSE, NON-INFRINGEMENT, ABSENCE OF LATENT OR OTHER DEFECTS,
     ACCURACY, OR THE PRESENCE OR ABSENCE OF ERRORS, WHETHER OR NOT
     KNOWN OR DISCOVERABLE. WHERE DISCLAIMERS OF WARRANTIES ARE NOT
     ALLOWED IN FULL OR IN PART, THIS DISCLAIMER MAY NOT APPLY TO YOU.

  b. TO THE EXTENT POSSIBLE, IN NO EVENT WILL THE LICENSOR BE LIABLE
     TO YOU ON ANY LEGAL THEORY (INCLUDING, WITHOUT LIMITATION,
     NEGLIGENCE) OR OTHERWISE FOR ANY DIRECT, SPECIAL, INDIRECT,
     INCIDENTAL, CONSEQUENTIAL, PUNITIVE, EXEMPLARY, OR OTHER LOSSES,
     COSTS, EXPENSES, OR DAMAGES ARISING OUT OF THIS PUBLIC LICENSE OR
     USE OF THE LICENSED MATERIAL, EVEN IF THE LICENSOR HAS BEEN
     ADVISED OF THE POSSIBILITY OF SUCH LOSSES, COSTS, EXPENSES, OR
     DAMAGES. WHERE A LIMITATION OF LIABILITY IS NOT ALLOWED IN FULL OR
     IN PART, THIS LIMITATION MAY NOT APPLY TO YOU.

  c. The disclaimer of warranties and limitation of liability provided
     above shall be interpreted in a manner that, to the extent
     possible, most closely approximates an absolute disclaimer and
     waiver of all liability.


Section 6 -- Term and Termination.

  a. This Public License applies for the term of the Copyright and
     Similar Rights licensed here. However, if You fail to comply with
     this Public License, then Your rights under this Public License
     terminate automatically.

  b. Where Your right to use the Licensed Material has terminated under
     Section 6(a), it reinstates:

       1. automatically as of the date the violation is cured, provided
          it is cured within 30 days of Your discovery of the
          violation; or

       2. upon express reinstatement by the Licensor.

     For the avoidance of doubt, this Section 6(b) does not affect any
     right the Licensor may have to seek remedies for Your violations
     of this Public License.

  c. For the avoidance of doubt, the Licensor may also offer the
     Licensed Material under separate terms or conditions or stop
     distributing the Licensed Material at any time; however, doing so
     will not terminate this Public License.

  d. Sections 1, 5, 6, 7, and 8 survive termination of this Public
     License.


Section 7 -- Other Terms and Conditions.

  a. The Licensor shall not be bound by any additional or different
     terms or conditions communicated by You unless expressly agreed.

  b. Any arrangements, understandings, or agreements regarding the
     Licensed Material not stated herein are separate from and
     independent of the terms and conditions of this Public License.


Section 8 -- Interpretation.

  a. For the avoidance of doubt, this Public License does not, and
     shall not be interpreted to, reduce, limit, restrict, or impose
     conditions on any use of the Licensed Material that could lawfully
     be made without permission under this Public License.

  b. To the extent possible, if any provision of this Public License is
     deemed unenforceable, it shall be automatically reformed to the
     minimum extent necessary to make it enforceable. If the provision
     cannot be reformed, it shall be severed from this Public License
     without affecting the enforceability of the remaining terms and
     conditions.

  c. No term or condition of this Public License will be waived and no
     failure to comply consented to unless expressly agreed to by the
     Licensor.

  d. Nothing in this Public License constitutes or may be interpreted
     as a limitation upon, or waiver of, any privileges and immunities
     that apply to the Licensor or You, including from the legal
     processes of any jurisdiction or authority.

=======================================================================

Creative Commons is not a party to its public licenses.
Notwithstanding, Creative Commons may elect to apply one of its public
licenses to material it publishes and in those instances will be
considered the "Licensor." Except for the limited purpose of indicating
that material is shared under a Creative Commons public license or as
otherwise permitted by the Creative Commons policies published at
creativecommons.org/policies, Creative Commons does not authorize the
use of the trademark "Creative Commons" or any other trademark or logo
of Creative Commons without its prior written consent including,
without limitation, in connection with any unauthorized modifications
to any of its public licenses or any other arrangements,
understandings, or agreements concerning use of licensed material. For
the avoidance of doubt, this paragraph does not form part of the public
licenses.

Creative Commons may be contacted at creativecommons.org.


==> license-texts/doclicense-CC-by-nc-sa-3.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NonCommercial-ShareAlike 3.0 Unported}





\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES
NOT PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE
DOES NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE
COMMONS PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS.
CREATIVE COMMONS MAKES NO WARRANTIES REGARDING THE
INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR DAMAGES
RESULTING FROM ITS USE.
\end{quotation}
\subsubsection{\emph{License}}
\par THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS
OF THIS CREATIVE COMMONS PUBLIC LICENSE (``CCPL'' OR
``LICENSE''). THE WORK IS PROTECTED BY COPYRIGHT AND/OR OTHER
APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS
PROHIBITED.
\par BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU
ACCEPT AND AGREE TO BE BOUND BY THE TERMS OF THIS LICENSE.
TO THE EXTENT THIS LICENSE MAY BE CONSIDERED TO BE A
CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS CONTAINED HERE
IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.
\par \textbf{1. Definitions}
\begin{enumerate}
\item \textbf{``Adaptation''} means a work based upon
the Work, or upon the Work and other pre-existing works,
such as a translation, adaptation, derivative work,
arrangement of music or other alterations of a literary
or artistic work, or phonogram or performance and
includes cinematographic adaptations or any other form in
which the Work may be recast, transformed, or adapted
including in any form recognizably derived from the
original, except that a work that constitutes a
Collection will not be considered an Adaptation for the
purpose of this License. For the avoidance of doubt,
where the Work is a musical work, performance or
phonogram, the synchronization of the Work in
timed-relation with a moving image (``synching'') will be
considered an Adaptation for the purpose of this
License.
\item \textbf{``Collection''} means a collection of
literary or artistic works, such as encyclopedias and
anthologies, or performances, phonograms or broadcasts,
or other works or subject matter other than works listed
in Section 1(g) below, which, by reason of the selection
and arrangement of their contents, constitute
intellectual creations, in which the Work is included in
its entirety in unmodified form along with one or more
other contributions, each constituting separate and
independent works in themselves, which together are
assembled into a collective whole. A work that
constitutes a Collection will not be considered an
Adaptation (as defined above) for the purposes of this
License.
\item \textbf{``Distribute''} means to make available
to the public the original and copies of the Work or
Adaptation, as appropriate, through sale or other
transfer of ownership.
\item \textbf{``License Elements''} means the
following high-level license attributes as selected by
Licensor and indicated in the title of this License:
Attribution, Noncommercial, ShareAlike.
\item \textbf{``Licensor''} means the individual,
individuals, entity or entities that offer(s) the Work
under the terms of this License.
\item \textbf{``Original Author''} means, in the case
of a literary or artistic work, the individual,
individuals, entity or entities who created the Work or
if no individual or entity can be identified, the
publisher; and in addition (i) in the case of a
performance the actors, singers, musicians, dancers, and
other persons who act, sing, deliver, declaim, play in,
interpret or otherwise perform literary or artistic works
or expressions of folklore; (ii) in the case of a
phonogram the producer being the person or legal entity
who first fixes the sounds of a performance or other
sounds; and, (iii) in the case of broadcasts, the
organization that transmits the broadcast.
\item \textbf{``Work''} means the literary and/or
artistic work offered under the terms of this License
including without limitation any production in the
literary, scientific and artistic domain, whatever may be
the mode or form of its expression including digital
form, such as a book, pamphlet and other writing; a
lecture, address, sermon or other work of the same
nature; a dramatic or dramatico-musical work; a
choreographic work or entertainment in dumb show; a
musical composition with or without words; a
cinematographic work to which are assimilated works
expressed by a process analogous to cinematography; a
work of drawing, painting, architecture, sculpture,
engraving or lithography; a photographic work to which
are assimilated works expressed by a process analogous to
photography; a work of applied art; an illustration, map,
plan, sketch or three-dimensional work relative to
geography, topography, architecture or science; a
performance; a broadcast; a phonogram; a compilation of
data to the extent it is protected as a copyrightable
work; or a work performed by a variety or circus
performer to the extent it is not otherwise considered a
literary or artistic work.
\item \textbf{``You''} means an individual or entity
exercising rights under this License who has not
previously violated the terms of this License with
respect to the Work, or who has received express
permission from the Licensor to exercise rights under
this License despite a previous violation.
\item \textbf{``Publicly Perform''} means to perform
public recitations of the Work and to communicate to the
public those public recitations, by any means or process,
including by wire or wireless means or public digital
performances; to make available to the public Works in
such a way that members of the public may access these
Works from a place and at a place individually chosen by
them; to perform the Work to the public by any means or
process and the communication to the public of the
performances of the Work, including by public digital
performance; to broadcast and rebroadcast the Work by any
means including signs, sounds or images.
\item \textbf{``Reproduce''} means to make copies of
the Work by any means including without limitation by
sound or visual recordings and the right of fixation and
reproducing fixations of the Work, including storage of a
protected performance or phonogram in digital form or
other electronic medium.
\end{enumerate}
\par \textbf{2. Fair Dealing Rights.} Nothing in this
License is intended to reduce, limit, or restrict any uses
free from copyright or rights arising from limitations or
exceptions that are provided for in connection with the
copyright protection under copyright law or other
applicable laws.
\par \textbf{3. License Grant.} Subject to the terms
and conditions of this License, Licensor hereby grants You
a worldwide, royalty-free, non-exclusive, perpetual (for
the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:
\begin{enumerate}
\item to Reproduce the Work, to incorporate the Work into
one or more Collections, and to Reproduce the Work as
incorporated in the Collections;
\item to create and Reproduce Adaptations provided that any
such Adaptation, including any translation in any medium,
takes reasonable steps to clearly label, demarcate or
otherwise identify that changes were made to the original
Work. For example, a translation could be marked ``The
original work was translated from English to Spanish,'' or
a modification could indicate ``The original work has been
modified.'';
\item to Distribute and Publicly Perform the Work including
as incorporated in Collections; and,
\item to Distribute and Publicly Perform Adaptations.
\end{enumerate}
\par The above rights may be exercised in all media and
formats whether now known or hereafter devised. The above
rights include the right to make such modifications as are
technically necessary to exercise the rights in other media
and formats. Subject to Section 8(f), all rights not
expressly granted by Licensor are hereby reserved,
including but not limited to the rights described in
Section 4(e).
\par \textbf{4. Restrictions.} The license granted in
Section 3 above is expressly made subject to and limited by
the following restrictions:
\begin{enumerate}
\item You may Distribute or Publicly Perform the Work only
under the terms of this License. You must include a copy
of, or the Uniform Resource Identifier (URI) for, this
License with every copy of the Work You Distribute or
Publicly Perform. You may not offer or impose any terms
on the Work that restrict the terms of this License or
the ability of the recipient of the Work to exercise the
rights granted to that recipient under the terms of the
License. You may not sublicense the Work. You must keep
intact all notices that refer to this License and to the
disclaimer of warranties with every copy of the Work You
Distribute or Publicly Perform. When You Distribute or
Publicly Perform the Work, You may not impose any
effective technological measures on the Work that
restrict the ability of a recipient of the Work from You
to exercise the rights granted to that recipient under
the terms of the License. This Section 4(a) applies to
the Work as incorporated in a Collection, but this does
not require the Collection apart from the Work itself to
be made subject to the terms of this License. If You
create a Collection, upon notice from any Licensor You
must, to the extent practicable, remove from the
Collection any credit as required by Section 4(d), as
requested. If You create an Adaptation, upon notice from
any Licensor You must, to the extent practicable, remove
from the Adaptation any credit as required by Section
4(d), as requested.
\item You may Distribute or Publicly Perform an Adaptation
only under: (i) the terms of this License; (ii) a later
version of this License with the same License Elements as
this License; (iii) a Creative Commons jurisdiction
license (either this or a later license version) that
contains the same License Elements as this License (e.g.,
Attribution-NonCommercial-ShareAlike 3.0 US) (``Applicable
License''). You must include a copy of, or the URI, for
Applicable License with every copy of each Adaptation You
Distribute or Publicly Perform. You may not offer or
impose any terms on the Adaptation that restrict the
terms of the Applicable License or the ability of the
recipient of the Adaptation to exercise the rights
granted to that recipient under the terms of the
Applicable License. You must keep intact all notices that
refer to the Applicable License and to the disclaimer of
warranties with every copy of the Work as included in the
Adaptation You Distribute or Publicly Perform. When You
Distribute or Publicly Perform the Adaptation, You may
not impose any effective technological measures on the
Adaptation that restrict the ability of a recipient of
the Adaptation from You to exercise the rights granted to
that recipient under the terms of the Applicable License.
This Section 4(b) applies to the Adaptation as
incorporated in a Collection, but this does not require
the Collection apart from the Adaptation itself to be
made subject to the terms of the Applicable License.
\item You may not exercise any of the rights granted to You
in Section 3 above in any manner that is primarily
intended for or directed toward commercial advantage or
private monetary compensation. The exchange of the Work
for other copyrighted works by means of digital
file-sharing or otherwise shall not be considered to be
intended for or directed toward commercial advantage or
private monetary compensation, provided there is no
payment of any monetary compensation in con-nection with
the exchange of copyrighted works.
\item If You Distribute, or Publicly Perform the Work or
any Adaptations or Collections, You must, unless a
request has been made pursuant to Section 4(a), keep
intact all copyright notices for the Work and provide,
reasonable to the medium or means You are utilizing: (i)
the name of the Original Author (or pseudonym, if
applicable) if supplied, and/or if the Original Author
and/or Licensor designate another party or parties (e.g.,
a sponsor institute, publishing entity, journal) for
attribution (``Attribution Parties'') in Licensor's
copyright notice, terms of service or by other reasonable
means, the name of such party or parties; (ii) the title
of the Work if supplied; (iii) to the extent reasonably
practicable, the URI, if any, that Licensor specifies to
be associated with the Work, unless such URI does not
refer to the copyright notice or licensing information
for the Work; and, (iv) consistent with Section 3(b), in
the case of an Adaptation, a credit identifying the use
of the Work in the Adaptation (e.g., ``French translation
of the Work by Original Author,'' or ``Screenplay based on
original Work by Original Author''). The credit required
by this Section 4(d) may be implemented in any reasonable
manner; provided, however, that in the case of a
Adaptation or Collection, at a minimum such credit will
appear, if a credit for all contributing authors of the
Adaptation or Collection appears, then as part of these
credits and in a manner at least as prominent as the
credits for the other contributing authors. For the
avoidance of doubt, You may only use the credit required
by this Section for the purpose of attribution in the
manner set out above and, by exercising Your rights under
this License, You may not implicitly or explicitly assert
or imply any connection with, sponsorship or endorsement
by the Original Author, Licensor and/or Attribution
Parties, as appropriate, of You or Your use of the Work,
without the separate, express prior written permission of
the Original Author, Licensor and/or Attribution
Parties.
\item 
\par For the avoidance of doubt:
\begin{enumerate}
\item \textbf{Non-waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme cannot be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License;
\item \textbf{Waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme can be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License if Your exercise of such
rights is for a purpose or use which is otherwise
than noncommercial as permitted under Section 4(c)
and otherwise waives the right to collect royalties
through any statutory or compulsory licensing scheme;
and,
\item \textbf{Voluntary License Schemes}. The
Licensor reserves the right to collect royalties,
whether individually or, in the event that the
Licensor is a member of a collecting society that
administers voluntary licensing schemes, via that
society, from any exercise by You of the rights
granted under this License that is for a purpose or
use which is otherwise than noncommercial as
permitted under Section 4(c).
\end{enumerate}

\item Except as otherwise agreed in writing by the Licensor
or as may be otherwise permitted by applicable law, if
You Reproduce, Distribute or Publicly Perform the Work
either by itself or as part of any Adaptations or
Collections, You must not distort, mutilate, modify or
take other derogatory action in relation to the Work
which would be prejudicial to the Original Author's honor
or reputation. Licensor agrees that in those
jurisdictions (e.g. Japan), in which any exercise of the
right granted in Section 3(b) of this License (the right
to make Adaptations) would be deemed to be a distortion,
mutilation, modification or other derogatory action
prejudicial to the Original Author's honor and
reputation, the Licensor will waive or not assert, as
appropriate, this Section, to the fullest extent
permitted by the applicable national law, to enable You
to reasonably exercise Your right under Section 3(b) of
this License (right to make Adaptations) but not
otherwise.
\end{enumerate}
\par \textbf{5. Representations, Warranties and
Disclaimer}
\par UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN
WRITING AND TO THE FULLEST EXTENT PERMITTED BY APPLICABLE
LAW, LICENSOR OFFERS THE WORK AS-IS AND MAKES NO
REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING,
WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTABILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE
ABSENCE OF LATENT OR OTHER DEFECTS, ACCURACY, OR THE
PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT DISCOVERABLE.
SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO THIS EXCLUSION MAY NOT APPLY TO YOU.
\par \textbf{6. Limitation on Liability.} EXCEPT TO
THE EXTENT REQUIRED BY APPLICABLE LAW, IN NO EVENT WILL
LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR ANY
SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY
DAMAGES ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK,
EVEN IF LICENSOR HAS BEEN ADVISED OF THE POSSIBILITY OF
SUCH DAMAGES.
\par \textbf{7. Termination}
\begin{enumerate}
\item This License and the rights granted hereunder will
terminate automatically upon any breach by You of the
terms of this License. Individuals or entities who have
received Adaptations or Collections from You under this
License, however, will not have their licenses terminated
provided such individuals or entities remain in full
compliance with those licenses. Sections 1, 2, 5, 6, 7,
and 8 will survive any termination of this License.
\item Subject to the above terms and conditions, the
license granted here is perpetual (for the duration of
the applicable copyright in the Work). Notwithstanding
the above, Licensor reserves the right to release the
Work under different license terms or to stop
distributing the Work at any time; provided, however that
any such election will not serve to withdraw this License
(or any other license that has been, or is required to
be, granted under the terms of this License), and this
License will continue in full force and effect unless
terminated as stated above.
\end{enumerate}
\par \textbf{8. Miscellaneous}
\begin{enumerate}
\item Each time You Distribute or Publicly Perform the Work
or a Collection, the Licensor offers to the recipient a
license to the Work on the same terms and conditions as
the license granted to You under this License.
\item Each time You Distribute or Publicly Perform an
Adaptation, Licensor offers to the recipient a license to
the original Work on the same terms and conditions as the
license granted to You under this License.
\item If any provision of this License is invalid or
unenforceable under applicable law, it shall not affect
the validity or enforceability of the remainder of the
terms of this License, and without further action by the
parties to this agreement, such provision shall be
reformed to the minimum extent necessary to make such
provision valid and enforceable.
\item No term or provision of this License shall be deemed
waived and no breach consented to unless such waiver or
consent shall be in writing and signed by the party to be
charged with such waiver or consent.
\item This License constitutes the entire agreement between
the parties with respect to the Work licensed here. There
are no understandings, agreements or representations with
respect to the Work not specified here. Licensor shall
not be bound by any additional provisions that may appear
in any communication from You. This License may not be
modified without the mutual written agreement of the
Licensor and You.
\item The rights granted under, and the subject matter
referenced, in this License were drafted utilizing the
terminology of the Berne Convention for the Protection of
Literary and Artistic Works (as amended on September 28,
1979), the Rome Convention of 1961, the WIPO Copyright
Treaty of 1996, the WIPO Performances and Phonograms
Treaty of 1996 and the Universal Copyright Convention (as
revised on July 24, 1971). These rights and subject
matter take effect in the relevant jurisdiction in which
the License terms are sought to be enforced according to
the corresponding provisions of the implementation of
those treaty provisions in the applicable national law.
If the standard suite of rights granted under applicable
copyright law includes additional rights not granted
under this License, such additional rights are deemed to
be included in the License; this License is not intended
to restrict the license of any rights under applicable
law.
\end{enumerate}
 
\begin{quotation}
\subsubsection{Creative Commons Notice}
\par Creative Commons is not a party to this License, and
makes no warranty whatsoever in connection with the Work.
Creative Commons will not be liable to You or any party
on any legal theory for any damages whatsoever, including
without limitation any general, special, incidental or
consequential damages arising in connection to this
license. Notwithstanding the foregoing two (2) sentences,
if Creative Commons has expressly identified itself as
the Licensor hereunder, it shall have all rights and
obligations of Licensor.
\par Except for the limited purpose of indicating to the
public that the Work is licensed under the CCPL, Creative
Commons does not authorize the use by either party of the
trademark ``Creative Commons'' or any related trademark or
logo of Creative Commons without the prior written
consent of Creative Commons. Any permitted use will be in
compliance with Creative Commons' then-current trademark
usage guidelines, as may be published on its website or
otherwise made available upon request from time to time.
For the avoidance of doubt, this trademark restriction
does not form part of this License.
\par Creative Commons may be contacted at \url{https://creativecommons.org/}.
\end{quotation}



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nc-sa-3.0-plaintext.tex <==
Creative Commons Legal Code

Attribution-NonCommercial-ShareAlike 3.0 Unported

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR
    DAMAGES RESULTING FROM ITS USE.

License

THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS OF THIS CREATIVE
COMMONS PUBLIC LICENSE ("CCPL" OR "LICENSE"). THE WORK IS PROTECTED BY
COPYRIGHT AND/OR OTHER APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS PROHIBITED.

BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU ACCEPT AND AGREE
TO BE BOUND BY THE TERMS OF THIS LICENSE. TO THE EXTENT THIS LICENSE MAY
BE CONSIDERED TO BE A CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS
CONTAINED HERE IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.

1. Definitions

 a. "Adaptation" means a work based upon the Work, or upon the Work and
    other pre-existing works, such as a translation, adaptation,
    derivative work, arrangement of music or other alterations of a
    literary or artistic work, or phonogram or performance and includes
    cinematographic adaptations or any other form in which the Work may be
    recast, transformed, or adapted including in any form recognizably
    derived from the original, except that a work that constitutes a
    Collection will not be considered an Adaptation for the purpose of
    this License. For the avoidance of doubt, where the Work is a musical
    work, performance or phonogram, the synchronization of the Work in
    timed-relation with a moving image ("synching") will be considered an
    Adaptation for the purpose of this License.
 b. "Collection" means a collection of literary or artistic works, such as
    encyclopedias and anthologies, or performances, phonograms or
    broadcasts, or other works or subject matter other than works listed
    in Section 1(g) below, which, by reason of the selection and
    arrangement of their contents, constitute intellectual creations, in
    which the Work is included in its entirety in unmodified form along
    with one or more other contributions, each constituting separate and
    independent works in themselves, which together are assembled into a
    collective whole. A work that constitutes a Collection will not be
    considered an Adaptation (as defined above) for the purposes of this
    License.
 c. "Distribute" means to make available to the public the original and
    copies of the Work or Adaptation, as appropriate, through sale or
    other transfer of ownership.
 d. "License Elements" means the following high-level license attributes
    as selected by Licensor and indicated in the title of this License:
    Attribution, Noncommercial, ShareAlike.
 e. "Licensor" means the individual, individuals, entity or entities that
    offer(s) the Work under the terms of this License.
 f. "Original Author" means, in the case of a literary or artistic work,
    the individual, individuals, entity or entities who created the Work
    or if no individual or entity can be identified, the publisher; and in
    addition (i) in the case of a performance the actors, singers,
    musicians, dancers, and other persons who act, sing, deliver, declaim,
    play in, interpret or otherwise perform literary or artistic works or
    expressions of folklore; (ii) in the case of a phonogram the producer
    being the person or legal entity who first fixes the sounds of a
    performance or other sounds; and, (iii) in the case of broadcasts, the
    organization that transmits the broadcast.
 g. "Work" means the literary and/or artistic work offered under the terms
    of this License including without limitation any production in the
    literary, scientific and artistic domain, whatever may be the mode or
    form of its expression including digital form, such as a book,
    pamphlet and other writing; a lecture, address, sermon or other work
    of the same nature; a dramatic or dramatico-musical work; a
    choreographic work or entertainment in dumb show; a musical
    composition with or without words; a cinematographic work to which are
    assimilated works expressed by a process analogous to cinematography;
    a work of drawing, painting, architecture, sculpture, engraving or
    lithography; a photographic work to which are assimilated works
    expressed by a process analogous to photography; a work of applied
    art; an illustration, map, plan, sketch or three-dimensional work
    relative to geography, topography, architecture or science; a
    performance; a broadcast; a phonogram; a compilation of data to the
    extent it is protected as a copyrightable work; or a work performed by
    a variety or circus performer to the extent it is not otherwise
    considered a literary or artistic work.
 h. "You" means an individual or entity exercising rights under this
    License who has not previously violated the terms of this License with
    respect to the Work, or who has received express permission from the
    Licensor to exercise rights under this License despite a previous
    violation.
 i. "Publicly Perform" means to perform public recitations of the Work and
    to communicate to the public those public recitations, by any means or
    process, including by wire or wireless means or public digital
    performances; to make available to the public Works in such a way that
    members of the public may access these Works from a place and at a
    place individually chosen by them; to perform the Work to the public
    by any means or process and the communication to the public of the
    performances of the Work, including by public digital performance; to
    broadcast and rebroadcast the Work by any means including signs,
    sounds or images.
 j. "Reproduce" means to make copies of the Work by any means including
    without limitation by sound or visual recordings and the right of
    fixation and reproducing fixations of the Work, including storage of a
    protected performance or phonogram in digital form or other electronic
    medium.

2. Fair Dealing Rights. Nothing in this License is intended to reduce,
limit, or restrict any uses free from copyright or rights arising from
limitations or exceptions that are provided for in connection with the
copyright protection under copyright law or other applicable laws.

3. License Grant. Subject to the terms and conditions of this License,
Licensor hereby grants You a worldwide, royalty-free, non-exclusive,
perpetual (for the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:

 a. to Reproduce the Work, to incorporate the Work into one or more
    Collections, and to Reproduce the Work as incorporated in the
    Collections;
 b. to create and Reproduce Adaptations provided that any such Adaptation,
    including any translation in any medium, takes reasonable steps to
    clearly label, demarcate or otherwise identify that changes were made
    to the original Work. For example, a translation could be marked "The
    original work was translated from English to Spanish," or a
    modification could indicate "The original work has been modified.";
 c. to Distribute and Publicly Perform the Work including as incorporated
    in Collections; and,
 d. to Distribute and Publicly Perform Adaptations.

The above rights may be exercised in all media and formats whether now
known or hereafter devised. The above rights include the right to make
such modifications as are technically necessary to exercise the rights in
other media and formats. Subject to Section 8(f), all rights not expressly
granted by Licensor are hereby reserved, including but not limited to the
rights described in Section 4(e).

4. Restrictions. The license granted in Section 3 above is expressly made
subject to and limited by the following restrictions:

 a. You may Distribute or Publicly Perform the Work only under the terms
    of this License. You must include a copy of, or the Uniform Resource
    Identifier (URI) for, this License with every copy of the Work You
    Distribute or Publicly Perform. You may not offer or impose any terms
    on the Work that restrict the terms of this License or the ability of
    the recipient of the Work to exercise the rights granted to that
    recipient under the terms of the License. You may not sublicense the
    Work. You must keep intact all notices that refer to this License and
    to the disclaimer of warranties with every copy of the Work You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Work, You may not impose any effective technological
    measures on the Work that restrict the ability of a recipient of the
    Work from You to exercise the rights granted to that recipient under
    the terms of the License. This Section 4(a) applies to the Work as
    incorporated in a Collection, but this does not require the Collection
    apart from the Work itself to be made subject to the terms of this
    License. If You create a Collection, upon notice from any Licensor You
    must, to the extent practicable, remove from the Collection any credit
    as required by Section 4(d), as requested. If You create an
    Adaptation, upon notice from any Licensor You must, to the extent
    practicable, remove from the Adaptation any credit as required by
    Section 4(d), as requested.
 b. You may Distribute or Publicly Perform an Adaptation only under: (i)
    the terms of this License; (ii) a later version of this License with
    the same License Elements as this License; (iii) a Creative Commons
    jurisdiction license (either this or a later license version) that
    contains the same License Elements as this License (e.g.,
    Attribution-NonCommercial-ShareAlike 3.0 US) ("Applicable License").
    You must include a copy of, or the URI, for Applicable License with
    every copy of each Adaptation You Distribute or Publicly Perform. You
    may not offer or impose any terms on the Adaptation that restrict the
    terms of the Applicable License or the ability of the recipient of the
    Adaptation to exercise the rights granted to that recipient under the
    terms of the Applicable License. You must keep intact all notices that
    refer to the Applicable License and to the disclaimer of warranties
    with every copy of the Work as included in the Adaptation You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Adaptation, You may not impose any effective technological
    measures on the Adaptation that restrict the ability of a recipient of
    the Adaptation from You to exercise the rights granted to that
    recipient under the terms of the Applicable License. This Section 4(b)
    applies to the Adaptation as incorporated in a Collection, but this
    does not require the Collection apart from the Adaptation itself to be
    made subject to the terms of the Applicable License.
 c. You may not exercise any of the rights granted to You in Section 3
    above in any manner that is primarily intended for or directed toward
    commercial advantage or private monetary compensation. The exchange of
    the Work for other copyrighted works by means of digital file-sharing
    or otherwise shall not be considered to be intended for or directed
    toward commercial advantage or private monetary compensation, provided
    there is no payment of any monetary compensation in con-nection with
    the exchange of copyrighted works.
 d. If You Distribute, or Publicly Perform the Work or any Adaptations or
    Collections, You must, unless a request has been made pursuant to
    Section 4(a), keep intact all copyright notices for the Work and
    provide, reasonable to the medium or means You are utilizing: (i) the
    name of the Original Author (or pseudonym, if applicable) if supplied,
    and/or if the Original Author and/or Licensor designate another party
    or parties (e.g., a sponsor institute, publishing entity, journal) for
    attribution ("Attribution Parties") in Licensor's copyright notice,
    terms of service or by other reasonable means, the name of such party
    or parties; (ii) the title of the Work if supplied; (iii) to the
    extent reasonably practicable, the URI, if any, that Licensor
    specifies to be associated with the Work, unless such URI does not
    refer to the copyright notice or licensing information for the Work;
    and, (iv) consistent with Section 3(b), in the case of an Adaptation,
    a credit identifying the use of the Work in the Adaptation (e.g.,
    "French translation of the Work by Original Author," or "Screenplay
    based on original Work by Original Author"). The credit required by
    this Section 4(d) may be implemented in any reasonable manner;
    provided, however, that in the case of a Adaptation or Collection, at
    a minimum such credit will appear, if a credit for all contributing
    authors of the Adaptation or Collection appears, then as part of these
    credits and in a manner at least as prominent as the credits for the
    other contributing authors. For the avoidance of doubt, You may only
    use the credit required by this Section for the purpose of attribution
    in the manner set out above and, by exercising Your rights under this
    License, You may not implicitly or explicitly assert or imply any
    connection with, sponsorship or endorsement by the Original Author,
    Licensor and/or Attribution Parties, as appropriate, of You or Your
    use of the Work, without the separate, express prior written
    permission of the Original Author, Licensor and/or Attribution
    Parties.
 e. For the avoidance of doubt:

     i. Non-waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme cannot be waived, the Licensor
        reserves the exclusive right to collect such royalties for any
        exercise by You of the rights granted under this License;
    ii. Waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme can be waived, the Licensor reserves
        the exclusive right to collect such royalties for any exercise by
        You of the rights granted under this License if Your exercise of
        such rights is for a purpose or use which is otherwise than
        noncommercial as permitted under Section 4(c) and otherwise waives
        the right to collect royalties through any statutory or compulsory
        licensing scheme; and,
   iii. Voluntary License Schemes. The Licensor reserves the right to
        collect royalties, whether individually or, in the event that the
        Licensor is a member of a collecting society that administers
        voluntary licensing schemes, via that society, from any exercise
        by You of the rights granted under this License that is for a
        purpose or use which is otherwise than noncommercial as permitted
        under Section 4(c).
 f. Except as otherwise agreed in writing by the Licensor or as may be
    otherwise permitted by applicable law, if You Reproduce, Distribute or
    Publicly Perform the Work either by itself or as part of any
    Adaptations or Collections, You must not distort, mutilate, modify or
    take other derogatory action in relation to the Work which would be
    prejudicial to the Original Author's honor or reputation. Licensor
    agrees that in those jurisdictions (e.g. Japan), in which any exercise
    of the right granted in Section 3(b) of this License (the right to
    make Adaptations) would be deemed to be a distortion, mutilation,
    modification or other derogatory action prejudicial to the Original
    Author's honor and reputation, the Licensor will waive or not assert,
    as appropriate, this Section, to the fullest extent permitted by the
    applicable national law, to enable You to reasonably exercise Your
    right under Section 3(b) of this License (right to make Adaptations)
    but not otherwise.

5. Representations, Warranties and Disclaimer

UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN WRITING AND TO THE
FULLEST EXTENT PERMITTED BY APPLICABLE LAW, LICENSOR OFFERS THE WORK AS-IS
AND MAKES NO REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING, WITHOUT
LIMITATION, WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
PURPOSE, NONINFRINGEMENT, OR THE ABSENCE OF LATENT OR OTHER DEFECTS,
ACCURACY, OR THE PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT
DISCOVERABLE. SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO THIS EXCLUSION MAY NOT APPLY TO YOU.

6. Limitation on Liability. EXCEPT TO THE EXTENT REQUIRED BY APPLICABLE
LAW, IN NO EVENT WILL LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR
ANY SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY DAMAGES
ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK, EVEN IF LICENSOR HAS
BEEN ADVISED OF THE POSSIBILITY OF SUCH DAMAGES.

7. Termination

 a. This License and the rights granted hereunder will terminate
    automatically upon any breach by You of the terms of this License.
    Individuals or entities who have received Adaptations or Collections
    from You under this License, however, will not have their licenses
    terminated provided such individuals or entities remain in full
    compliance with those licenses. Sections 1, 2, 5, 6, 7, and 8 will
    survive any termination of this License.
 b. Subject to the above terms and conditions, the license granted here is
    perpetual (for the duration of the applicable copyright in the Work).
    Notwithstanding the above, Licensor reserves the right to release the
    Work under different license terms or to stop distributing the Work at
    any time; provided, however that any such election will not serve to
    withdraw this License (or any other license that has been, or is
    required to be, granted under the terms of this License), and this
    License will continue in full force and effect unless terminated as
    stated above.

8. Miscellaneous

 a. Each time You Distribute or Publicly Perform the Work or a Collection,
    the Licensor offers to the recipient a license to the Work on the same
    terms and conditions as the license granted to You under this License.
 b. Each time You Distribute or Publicly Perform an Adaptation, Licensor
    offers to the recipient a license to the original Work on the same
    terms and conditions as the license granted to You under this License.
 c. If any provision of this License is invalid or unenforceable under
    applicable law, it shall not affect the validity or enforceability of
    the remainder of the terms of this License, and without further action
    by the parties to this agreement, such provision shall be reformed to
    the minimum extent necessary to make such provision valid and
    enforceable.
 d. No term or provision of this License shall be deemed waived and no
    breach consented to unless such waiver or consent shall be in writing
    and signed by the party to be charged with such waiver or consent.
 e. This License constitutes the entire agreement between the parties with
    respect to the Work licensed here. There are no understandings,
    agreements or representations with respect to the Work not specified
    here. Licensor shall not be bound by any additional provisions that
    may appear in any communication from You. This License may not be
    modified without the mutual written agreement of the Licensor and You.
 f. The rights granted under, and the subject matter referenced, in this
    License were drafted utilizing the terminology of the Berne Convention
    for the Protection of Literary and Artistic Works (as amended on
    September 28, 1979), the Rome Convention of 1961, the WIPO Copyright
    Treaty of 1996, the WIPO Performances and Phonograms Treaty of 1996
    and the Universal Copyright Convention (as revised on July 24, 1971).
    These rights and subject matter take effect in the relevant
    jurisdiction in which the License terms are sought to be enforced
    according to the corresponding provisions of the implementation of
    those treaty provisions in the applicable national law. If the
    standard suite of rights granted under applicable copyright law
    includes additional rights not granted under this License, such
    additional rights are deemed to be included in the License; this
    License is not intended to restrict the license of any rights under
    applicable law.


Creative Commons Notice

    Creative Commons is not a party to this License, and makes no warranty
    whatsoever in connection with the Work. Creative Commons will not be
    liable to You or any party on any legal theory for any damages
    whatsoever, including without limitation any general, special,
    incidental or consequential damages arising in connection to this
    license. Notwithstanding the foregoing two (2) sentences, if Creative
    Commons has expressly identified itself as the Licensor hereunder, it
    shall have all rights and obligations of Licensor.

    Except for the limited purpose of indicating to the public that the
    Work is licensed under the CCPL, Creative Commons does not authorize
    the use by either party of the trademark "Creative Commons" or any
    related trademark or logo of Creative Commons without the prior
    written consent of Creative Commons. Any permitted use will be in
    compliance with Creative Commons' then-current trademark usage
    guidelines, as may be published on its website or otherwise made
    available upon request from time to time. For the avoidance of doubt,
    this trademark restriction does not form part of this License.

    Creative Commons may be contacted at https://creativecommons.org/.
   


==> license-texts/doclicense-CC-by-nc-sa-4.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NonCommercial-ShareAlike 4.0 International}







Official translations of this license are available in other languages.



\par Creative Commons Corporation (“Creative Commons”) is not a law firm and does not provide legal services or legal advice. Distribution of Creative Commons public licenses does not create a lawyer-client or other relationship. Creative Commons makes its licenses and related information available on an “as-is” basis. Creative Commons gives no warranties regarding its licenses, any material licensed under their terms and conditions, or any related information. Creative Commons disclaims all liability for damages resulting from their use to the fullest extent possible.


\par \textbf{Using Creative Commons Public Licenses}
\par Creative Commons public licenses provide a standard set of terms and conditions that creators and other rights holders may use
to share original works of authorship and other material subject to copyright and certain other rights specified in the public license below. The following considerations are for informational purposes only, are not exhaustive, and do not form part of our licenses.
\begin{quotation}\textbf{Considerations for licensors:} Our public licenses are intended for use by those authorized to give the public permission to use material in ways otherwise restricted by copyright and certain other rights. Our licenses are irrevocable. Licensors should read and understand the terms and conditions of the license they choose before applying it. Licensors should also secure all rights necessary before applying our licenses so that the public can reuse the material as expected. Licensors should clearly mark any material not subject to the license. This includes other CC-licensed material, or material used under an exception or limitation to copyright. More considerations for licensors.\end{quotation}
\begin{quotation}\textbf{Considerations for the public:} By using one of our public licenses, a licensor grants the public permission to use the licensed material under specified terms and conditions. If the licensor’s permission is not necessary for any reason–for example, because of any applicable exception or limitation to copyright–then that use is not regulated by the license. Our licenses grant only permissions under copyright and certain other rights that a licensor has authority to grant. Use of the licensed material may still be restricted for other reasons, including because others have copyright or other rights in the material. A licensor may make special requests, such as asking that all changes be marked or described. Although not required by our licenses, you are encouraged to respect those requests where reasonable.
More considerations for the public.\end{quotation}

\subsubsection{Creative Commons Attribution-NonCommercial-ShareAlike 4.0 International Public License}
\par By exercising the Licensed Rights (defined below), You accept and agree to be bound by the terms and conditions of this Creative Commons Attribution-NonCommercial-ShareAlike 4.0 International Public License (``Public License''). To the extent this Public License may be interpreted as a contract, You are granted the Licensed Rights in consideration of Your acceptance of these terms and conditions, and the Licensor grants You such rights in consideration of benefits the Licensor receives from making the Licensed Material available under these terms and conditions.
\par \textbf{Section 1 – Definitions.}
\begin{enumerate}
\item \textbf{Adapted Material} means material subject to Copyright and Similar Rights that is derived from or based upon the Licensed Material and in which the Licensed Material is translated, altered, arranged, transformed, or otherwise modified in a manner requiring permission under the Copyright and Similar Rights held by the Licensor. For purposes of this Public License, where the Licensed Material is a musical work, performance, or sound recording, Adapted Material is always produced where the Licensed Material is synched in timed relation with a moving image.
\item \textbf{Adapter's License} means the license You apply to Your Copyright and Similar Rights in Your contributions to Adapted Material in accordance with the terms and conditions of this Public License.
\item \textbf{BY-NC-SA Compatible License} means a license listed at  creativecommons.org/compatiblelicenses, approved by Creative Commons as essentially the equivalent of this Public License.
\item \textbf{Copyright and Similar Rights} means copyright and/or similar rights closely related to copyright including, without limitation, performance, broadcast, sound recording, and Sui Generis Database Rights, without regard to how the rights are labeled or categorized. For purposes of this Public License, the rights specified in Section 2(b)(1)-(2) are not Copyright and Similar Rights.
\item \textbf{Effective Technological Measures} means those measures that, in the absence of proper authority, may not
be circumvented under laws fulfilling obligations under Article 11 of the WIPO Copyright Treaty adopted on December 20, 1996, and/or similar
international agreements.
\item \textbf{Exceptions and Limitations} means fair use, fair dealing, and/or any other exception or limitation to Copyright and Similar Rights that applies to Your use of the Licensed Material.
\item \textbf{License Elements} means the license attributes listed in the name of a Creative Commons Public License. The License Elements of this Public License are Attribution, NonCommercial, and ShareAlike.
\item \textbf{Licensed Material} means the artistic or literary work, database, or other material to which the Licensor applied this Public License.
\item \textbf{Licensed Rights} means the rights granted to You subject to the terms and conditions of this Public License, which are limited to all Copyright and Similar Rights that apply to Your use of the Licensed Material and that the Licensor has authority to license.
\item \textbf{Licensor} means the individual(s) or entity(ies) granting rights under this Public License.
\item \textbf{NonCommercial} means not primarily intended for or directed towards commercial advantage or monetary compensation. For purposes of this Public License, the exchange of the Licensed Material for other material subject to Copyright and Similar Rights by digital file-sharing or similar means is NonCommercial provided there is no payment of monetary compensation in connection with the exchange.
\item \textbf{Share} means to provide material to the public by any means or process that requires permission under the Licensed Rights, such as reproduction, public display, public performance, distribution, dissemination, communication, or importation, and to make material available to the public including in ways that members of the public may access the material from a place and at a time individually chosen by them.
\item \textbf{Sui Generis Database Rights} means rights other than copyright resulting from Directive 96/9/EC of the European Parliament and of the Council of 11 March 1996 on the legal protection of databases, as amended and/or succeeded, as well as other essentially equivalent rights anywhere in the world.
\item \textbf{You} means the individual or entity exercising the Licensed Rights under this Public License. \textbf{Your} has a corresponding meaning.
\end{enumerate}
\par \textbf{Section 2 – Scope.}
\begin{enumerate}
\item \textbf{License grant}.
\begin{enumerate}
\item Subject to the terms and conditions of this Public License, the Licensor hereby grants You a worldwide, royalty-free, non-sublicensable, non-exclusive, irrevocable license to exercise the Licensed Rights in the Licensed Material to:
\begin{enumerate}
\item reproduce and Share the Licensed Material, in whole or in part, for NonCommercial purposes only; and
\item produce, reproduce, and Share Adapted Material for NonCommercial purposes only.
\end{enumerate}
\item Exceptions and Limitations. For the avoidance of doubt, where Exceptions and Limitations apply to Your use, this Public License does not apply, and You do not need to comply with its terms and conditions.
\item Term. The term of this Public License is specified in Section 6(a).
\item Media and formats; technical modifications allowed. The Licensor authorizes You to exercise the Licensed Rights in all media and formats whether now known or hereafter created, and to make technical modifications necessary to do so. The Licensor waives and/or agrees not to assert any right or authority to forbid You from making technical modifications necessary to exercise the Licensed Rights, including technical modifications necessary to circumvent Effective Technological Measures. For purposes of this Public License, simply making modifications authorized by this Section 2(a)(4) never produces Adapted Material.
\item Downstream recipients.

\begin{enumerate}
\item Offer from the Licensor – Licensed Material. Every recipient of the Licensed Material automatically receives an offer from the Licensor to exercise the Licensed Rights under the terms and conditions of this Public License.
\item Additional offer from the Licensor – Adapted Material. Every recipient of Adapted Material from You automatically receives an offer from the Licensor to exercise the Licensed Rights in the Adapted Material under the conditions of the Adapter’s License You apply.
\item No downstream restrictions. You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, the Licensed Material if doing so restricts exercise of the Licensed Rights by any recipient of the Licensed Material.
\end{enumerate}

\item No endorsement. Nothing in this Public License constitutes or may be construed as permission to assert or imply that You are, or that Your use of the Licensed Material is, connected with, or sponsored, endorsed, or granted official status by, the Licensor or others designated to receive attribution as provided in Section 3(a)(1)(A)(i).
\end{enumerate}
\item \par \textbf{Other rights}.
\begin{enumerate}
\item Moral rights, such as the right of integrity, are not licensed under this Public License, nor are publicity, privacy, and/or other similar personality rights; however, to the extent possible, the Licensor waives and/or agrees not to assert any such rights held by the Licensor to the limited extent necessary to allow You to exercise the Licensed Rights, but not otherwise.
\item Patent and trademark rights are not licensed under this Public License.
\item To the extent possible, the Licensor waives any right to collect royalties from You for the exercise of the Licensed Rights, whether directly or through a collecting society under any voluntary or waivable statutory or compulsory licensing scheme. In all other cases the Licensor expressly reserves any right to collect such royalties, including when the Licensed Material is used other than for NonCommercial purposes.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 3 – License Conditions.}
\par Your exercise of the Licensed Rights is expressly made subject to the following conditions.
\begin{enumerate}
\item \par \textbf{Attribution}.
\begin{enumerate}
\item \par If You Share the Licensed Material (including in modified form), You must:
\begin{enumerate}
\item retain the following if it is supplied by the Licensor with the Licensed Material:
\begin{enumerate}
\item identification of the creator(s) of the Licensed Material and any others designated to receive attribution, in any reasonable manner requested by the Licensor (including by pseudonym if designated);
\item a copyright notice;
\item a notice that refers to this Public License; 
\item a notice that refers to the disclaimer of warranties;
\item a URI or hyperlink to the Licensed Material to the extent reasonably practicable;
\end{enumerate}
\item indicate if You modified the Licensed Material and retain an indication of any previous modifications; and
\item indicate the Licensed Material is licensed under this Public License,
and include the text of, or the URI or hyperlink to, this Public
License.
\end{enumerate}

\item You may satisfy the conditions in Section 3(a)(1) in any reasonable manner based on the medium, means, and context in which You Share the Licensed Material. For example, it may be reasonable to satisfy the conditions by providing a URI or hyperlink to a resource that includes the required information.
\item If requested by the Licensor, You must remove any of the information required by Section 3(a)(1)(A) to the extent reasonably practicable.
\end{enumerate}

\item \textbf{ShareAlike}.
\par In addition to the conditions in Section 3(a), if You Share Adapted Material You produce, the following conditions also apply.
\begin{enumerate}
\item The Adapter’s License You apply must be a Creative Commons license with the same License Elements, this version or later, or a BY-NC-SA Compatible License.
\item You must include the text of, or the URI or hyperlink to, the Adapter's License You apply. You may satisfy this condition in any reasonable manner based on the medium, means, and context in which You Share Adapted Material.
\item You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, Adapted Material that restrict exercise of the rights granted under the Adapter's License You apply.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 4 – Sui Generis Database Rights.}
\par Where the Licensed Rights include Sui Generis Database Rights that apply to Your use of the Licensed Material:
\begin{enumerate}
\item for the avoidance of doubt, Section 2(a)(1) grants You the right to extract, reuse, reproduce, and Share all or a substantial portion of the contents of the database for NonCommercial purposes only;
\item if You include all or a substantial portion of the database contents in a database in which You have Sui Generis Database Rights, then the database in which You have Sui Generis Database Rights (but not its individual contents) is Adapted Material, including for purposes of Section 3(b); and
\item You must comply with the conditions in Section 3(a) if You Share all or a substantial portion of the contents of the database.
\end{enumerate}
For the avoidance of doubt, this Section 4 supplements and does not replace Your obligations under this Public License where the Licensed Rights include other Copyright and Similar Rights.
\par \textbf{Section 5 – Disclaimer of Warranties and Limitation of Liability.}
\begin{enumerate}
\item \textbf{Unless otherwise separately undertaken by the Licensor, to the extent possible, the Licensor offers the Licensed Material as-is and as-available, and makes no representations or warranties of any kind concerning the Licensed Material, whether express, implied, statutory, or other. This includes, without limitation, warranties of title, merchantability, fitness for a particular purpose, non-infringement, absence of latent or other defects, accuracy, or the presence or absence of errors, whether or not known or discoverable. Where disclaimers of warranties are not allowed in full or in part, this disclaimer may not apply to You.}
\item \textbf{To the extent possible, in no event will the Licensor be liable to You on any legal theory (including, without limitation, negligence) or otherwise for any direct, special, indirect, incidental, consequential, punitive, exemplary, or other losses, costs, expenses, or damages arising out of this Public License or use of the Licensed Material, even if the Licensor has been advised of the possibility of such losses, costs, expenses, or damages. Where a limitation of liability is not allowed in full or in part, this limitation may not apply to You.}
\end{enumerate}
\begin{enumerate}
\item The disclaimer of warranties and limitation of liability provided above shall be interpreted in a manner that, to the extent possible, most closely approximates an absolute disclaimer and waiver of all liability.
\end{enumerate}
\par \textbf{Section 6 – Term and Termination.}
\begin{enumerate}
\item This Public License applies for the term of the Copyright and Similar Rights licensed here. However, if You fail to comply with this Public License, then Your rights under this Public License terminate automatically.
\item 
\par Where Your right to use the Licensed Material has terminated under Section 6(a), it reinstates:
\begin{enumerate}
\item automatically as of the date the violation is cured, provided it is cured within 30 days of Your discovery of the violation; or
\item upon express reinstatement by the Licensor.
\end{enumerate}
For the avoidance of doubt, this Section 6(b) does not affect any right the Licensor may have to seek remedies for Your violations of this Public License.
\item For the avoidance of doubt, the Licensor may also offer the Licensed Material under separate terms or conditions or stop distributing the Licensed Material at any time; however, doing so will not terminate this Public License.
\item Sections 1, 5, 6, 7, and 8 survive termination of this Public License.
\end{enumerate}
\par \textbf{Section 7 – Other Terms and Conditions.}
\begin{enumerate}
\item The Licensor shall not be bound by any additional or different terms or conditions communicated by You unless expressly agreed.
\item Any arrangements, understandings, or agreements regarding the Licensed Material not stated herein are separate from and independent of the terms and conditions of this Public License.
\end{enumerate}
\par \textbf{Section 8 – Interpretation.}
\begin{enumerate}
\item For the avoidance of doubt, this Public License does not, and shall not be interpreted to, reduce, limit, restrict, or impose conditions on any use of the Licensed Material that could lawfully be made without permission under this Public License.
\item To the extent possible, if any provision of this Public License is deemed unenforceable, it shall be automatically reformed to the minimum extent necessary to make it enforceable. If the provision cannot be reformed, it shall be severed from this Public License without affecting the enforceability of the remaining terms and conditions.
\item No term or condition of this Public License will be waived and no failure to comply consented to unless expressly agreed to by the Licensor.
\item Nothing in this Public License constitutes or may be interpreted as a limitation upon, or waiver of, any privileges and immunities that apply to the Licensor or You, including from the legal processes of any jurisdiction or authority.
\end{enumerate}
\par Creative Commons is not a party to its public licenses. Notwithstanding, Creative Commons may elect to apply one of its public licenses to material it publishes and in those instances will be considered the “Licensor.” The text of the Creative Commons public licenses is dedicated to the public domain under the CC0 Public Domain Dedication. Except for the limited purpose of indicating that material is shared under a Creative Commons public license or as otherwise permitted by the Creative Commons policies published at creativecommons.org/policies, Creative Commons does not authorize the use of the trademark “Creative Commons” or any other trademark or logo of Creative Commons without its prior written consent including, without limitation, in connection with any unauthorized modifications to any of its public licenses or any other arrangements, understandings, or agreements concerning use of licensed material. For the avoidance of doubt, this paragraph does not form part of the public licenses.\\\\
Creative Commons may be contacted at creativecommons.org.
\par Additional languages available: Bahasa Indonesia, Nederlands, norsk, suomeksi, te reo Māori, українська, 日本語. Please read the FAQ for more information about official translations. 


\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nc-sa-4.0-plaintext.tex <==
Attribution-NonCommercial-ShareAlike 4.0 International

=======================================================================

Creative Commons Corporation ("Creative Commons") is not a law firm and
does not provide legal services or legal advice. Distribution of
Creative Commons public licenses does not create a lawyer-client or
other relationship. Creative Commons makes its licenses and related
information available on an "as-is" basis. Creative Commons gives no
warranties regarding its licenses, any material licensed under their
terms and conditions, or any related information. Creative Commons
disclaims all liability for damages resulting from their use to the
fullest extent possible.

Using Creative Commons Public Licenses

Creative Commons public licenses provide a standard set of terms and
conditions that creators and other rights holders may use to share
original works of authorship and other material subject to copyright
and certain other rights specified in the public license below. The
following considerations are for informational purposes only, are not
exhaustive, and do not form part of our licenses.

     Considerations for licensors: Our public licenses are
     intended for use by those authorized to give the public
     permission to use material in ways otherwise restricted by
     copyright and certain other rights. Our licenses are
     irrevocable. Licensors should read and understand the terms
     and conditions of the license they choose before applying it.
     Licensors should also secure all rights necessary before
     applying our licenses so that the public can reuse the
     material as expected. Licensors should clearly mark any
     material not subject to the license. This includes other CC-
     licensed material, or material used under an exception or
     limitation to copyright. More considerations for licensors:
	wiki.creativecommons.org/Considerations_for_licensors

     Considerations for the public: By using one of our public
     licenses, a licensor grants the public permission to use the
     licensed material under specified terms and conditions. If
     the licensor's permission is not necessary for any reason--for
     example, because of any applicable exception or limitation to
     copyright--then that use is not regulated by the license. Our
     licenses grant only permissions under copyright and certain
     other rights that a licensor has authority to grant. Use of
     the licensed material may still be restricted for other
     reasons, including because others have copyright or other
     rights in the material. A licensor may make special requests,
     such as asking that all changes be marked or described.
     Although not required by our licenses, you are encouraged to
     respect those requests where reasonable. More_considerations
     for the public: 
	wiki.creativecommons.org/Considerations_for_licensees

=======================================================================

Creative Commons Attribution-NonCommercial-ShareAlike 4.0 International
Public License

By exercising the Licensed Rights (defined below), You accept and agree
to be bound by the terms and conditions of this Creative Commons
Attribution-NonCommercial-ShareAlike 4.0 International Public License
("Public License"). To the extent this Public License may be
interpreted as a contract, You are granted the Licensed Rights in
consideration of Your acceptance of these terms and conditions, and the
Licensor grants You such rights in consideration of benefits the
Licensor receives from making the Licensed Material available under
these terms and conditions.


Section 1 -- Definitions.

  a. Adapted Material means material subject to Copyright and Similar
     Rights that is derived from or based upon the Licensed Material
     and in which the Licensed Material is translated, altered,
     arranged, transformed, or otherwise modified in a manner requiring
     permission under the Copyright and Similar Rights held by the
     Licensor. For purposes of this Public License, where the Licensed
     Material is a musical work, performance, or sound recording,
     Adapted Material is always produced where the Licensed Material is
     synched in timed relation with a moving image.

  b. Adapter's License means the license You apply to Your Copyright
     and Similar Rights in Your contributions to Adapted Material in
     accordance with the terms and conditions of this Public License.

  c. BY-NC-SA Compatible License means a license listed at
     creativecommons.org/compatiblelicenses, approved by Creative
     Commons as essentially the equivalent of this Public License.

  d. Copyright and Similar Rights means copyright and/or similar rights
     closely related to copyright including, without limitation,
     performance, broadcast, sound recording, and Sui Generis Database
     Rights, without regard to how the rights are labeled or
     categorized. For purposes of this Public License, the rights
     specified in Section 2(b)(1)-(2) are not Copyright and Similar
     Rights.

  e. Effective Technological Measures means those measures that, in the
     absence of proper authority, may not be circumvented under laws
     fulfilling obligations under Article 11 of the WIPO Copyright
     Treaty adopted on December 20, 1996, and/or similar international
     agreements.

  f. Exceptions and Limitations means fair use, fair dealing, and/or
     any other exception or limitation to Copyright and Similar Rights
     that applies to Your use of the Licensed Material.

  g. License Elements means the license attributes listed in the name
     of a Creative Commons Public License. The License Elements of this
     Public License are Attribution, NonCommercial, and ShareAlike.

  h. Licensed Material means the artistic or literary work, database,
     or other material to which the Licensor applied this Public
     License.

  i. Licensed Rights means the rights granted to You subject to the
     terms and conditions of this Public License, which are limited to
     all Copyright and Similar Rights that apply to Your use of the
     Licensed Material and that the Licensor has authority to license.

  j. Licensor means the individual(s) or entity(ies) granting rights
     under this Public License.

  k. NonCommercial means not primarily intended for or directed towards
     commercial advantage or monetary compensation. For purposes of
     this Public License, the exchange of the Licensed Material for
     other material subject to Copyright and Similar Rights by digital
     file-sharing or similar means is NonCommercial provided there is
     no payment of monetary compensation in connection with the
     exchange.

  l. Share means to provide material to the public by any means or
     process that requires permission under the Licensed Rights, such
     as reproduction, public display, public performance, distribution,
     dissemination, communication, or importation, and to make material
     available to the public including in ways that members of the
     public may access the material from a place and at a time
     individually chosen by them.

  m. Sui Generis Database Rights means rights other than copyright
     resulting from Directive 96/9/EC of the European Parliament and of
     the Council of 11 March 1996 on the legal protection of databases,
     as amended and/or succeeded, as well as other essentially
     equivalent rights anywhere in the world.

  n. You means the individual or entity exercising the Licensed Rights
     under this Public License. Your has a corresponding meaning.


Section 2 -- Scope.

  a. License grant.

       1. Subject to the terms and conditions of this Public License,
          the Licensor hereby grants You a worldwide, royalty-free,
          non-sublicensable, non-exclusive, irrevocable license to
          exercise the Licensed Rights in the Licensed Material to:

            a. reproduce and Share the Licensed Material, in whole or
               in part, for NonCommercial purposes only; and

            b. produce, reproduce, and Share Adapted Material for
               NonCommercial purposes only.

       2. Exceptions and Limitations. For the avoidance of doubt, where
          Exceptions and Limitations apply to Your use, this Public
          License does not apply, and You do not need to comply with
          its terms and conditions.

       3. Term. The term of this Public License is specified in Section
          6(a).

       4. Media and formats; technical modifications allowed. The
          Licensor authorizes You to exercise the Licensed Rights in
          all media and formats whether now known or hereafter created,
          and to make technical modifications necessary to do so. The
          Licensor waives and/or agrees not to assert any right or
          authority to forbid You from making technical modifications
          necessary to exercise the Licensed Rights, including
          technical modifications necessary to circumvent Effective
          Technological Measures. For purposes of this Public License,
          simply making modifications authorized by this Section 2(a)
          (4) never produces Adapted Material.

       5. Downstream recipients.

            a. Offer from the Licensor -- Licensed Material. Every
               recipient of the Licensed Material automatically
               receives an offer from the Licensor to exercise the
               Licensed Rights under the terms and conditions of this
               Public License.

            b. Additional offer from the Licensor -- Adapted Material.
               Every recipient of Adapted Material from You
               automatically receives an offer from the Licensor to
               exercise the Licensed Rights in the Adapted Material
               under the conditions of the Adapter's License You apply.

            c. No downstream restrictions. You may not offer or impose
               any additional or different terms or conditions on, or
               apply any Effective Technological Measures to, the
               Licensed Material if doing so restricts exercise of the
               Licensed Rights by any recipient of the Licensed
               Material.

       6. No endorsement. Nothing in this Public License constitutes or
          may be construed as permission to assert or imply that You
          are, or that Your use of the Licensed Material is, connected
          with, or sponsored, endorsed, or granted official status by,
          the Licensor or others designated to receive attribution as
          provided in Section 3(a)(1)(A)(i).

  b. Other rights.

       1. Moral rights, such as the right of integrity, are not
          licensed under this Public License, nor are publicity,
          privacy, and/or other similar personality rights; however, to
          the extent possible, the Licensor waives and/or agrees not to
          assert any such rights held by the Licensor to the limited
          extent necessary to allow You to exercise the Licensed
          Rights, but not otherwise.

       2. Patent and trademark rights are not licensed under this
          Public License.

       3. To the extent possible, the Licensor waives any right to
          collect royalties from You for the exercise of the Licensed
          Rights, whether directly or through a collecting society
          under any voluntary or waivable statutory or compulsory
          licensing scheme. In all other cases the Licensor expressly
          reserves any right to collect such royalties, including when
          the Licensed Material is used other than for NonCommercial
          purposes.


Section 3 -- License Conditions.

Your exercise of the Licensed Rights is expressly made subject to the
following conditions.

  a. Attribution.

       1. If You Share the Licensed Material (including in modified
          form), You must:

            a. retain the following if it is supplied by the Licensor
               with the Licensed Material:

                 i. identification of the creator(s) of the Licensed
                    Material and any others designated to receive
                    attribution, in any reasonable manner requested by
                    the Licensor (including by pseudonym if
                    designated);

                ii. a copyright notice;

               iii. a notice that refers to this Public License;

                iv. a notice that refers to the disclaimer of
                    warranties;

                 v. a URI or hyperlink to the Licensed Material to the
                    extent reasonably practicable;

            b. indicate if You modified the Licensed Material and
               retain an indication of any previous modifications; and

            c. indicate the Licensed Material is licensed under this
               Public License, and include the text of, or the URI or
               hyperlink to, this Public License.

       2. You may satisfy the conditions in Section 3(a)(1) in any
          reasonable manner based on the medium, means, and context in
          which You Share the Licensed Material. For example, it may be
          reasonable to satisfy the conditions by providing a URI or
          hyperlink to a resource that includes the required
          information.
       3. If requested by the Licensor, You must remove any of the
          information required by Section 3(a)(1)(A) to the extent
          reasonably practicable.

  b. ShareAlike.

     In addition to the conditions in Section 3(a), if You Share
     Adapted Material You produce, the following conditions also apply.

       1. The Adapter's License You apply must be a Creative Commons
          license with the same License Elements, this version or
          later, or a BY-NC-SA Compatible License.

       2. You must include the text of, or the URI or hyperlink to, the
          Adapter's License You apply. You may satisfy this condition
          in any reasonable manner based on the medium, means, and
          context in which You Share Adapted Material.

       3. You may not offer or impose any additional or different terms
          or conditions on, or apply any Effective Technological
          Measures to, Adapted Material that restrict exercise of the
          rights granted under the Adapter's License You apply.


Section 4 -- Sui Generis Database Rights.

Where the Licensed Rights include Sui Generis Database Rights that
apply to Your use of the Licensed Material:

  a. for the avoidance of doubt, Section 2(a)(1) grants You the right
     to extract, reuse, reproduce, and Share all or a substantial
     portion of the contents of the database for NonCommercial purposes
     only;

  b. if You include all or a substantial portion of the database
     contents in a database in which You have Sui Generis Database
     Rights, then the database in which You have Sui Generis Database
     Rights (but not its individual contents) is Adapted Material,
     including for purposes of Section 3(b); and

  c. You must comply with the conditions in Section 3(a) if You Share
     all or a substantial portion of the contents of the database.

For the avoidance of doubt, this Section 4 supplements and does not
replace Your obligations under this Public License where the Licensed
Rights include other Copyright and Similar Rights.


Section 5 -- Disclaimer of Warranties and Limitation of Liability.

  a. UNLESS OTHERWISE SEPARATELY UNDERTAKEN BY THE LICENSOR, TO THE
     EXTENT POSSIBLE, THE LICENSOR OFFERS THE LICENSED MATERIAL AS-IS
     AND AS-AVAILABLE, AND MAKES NO REPRESENTATIONS OR WARRANTIES OF
     ANY KIND CONCERNING THE LICENSED MATERIAL, WHETHER EXPRESS,
     IMPLIED, STATUTORY, OR OTHER. THIS INCLUDES, WITHOUT LIMITATION,
     WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
     PURPOSE, NON-INFRINGEMENT, ABSENCE OF LATENT OR OTHER DEFECTS,
     ACCURACY, OR THE PRESENCE OR ABSENCE OF ERRORS, WHETHER OR NOT
     KNOWN OR DISCOVERABLE. WHERE DISCLAIMERS OF WARRANTIES ARE NOT
     ALLOWED IN FULL OR IN PART, THIS DISCLAIMER MAY NOT APPLY TO YOU.

  b. TO THE EXTENT POSSIBLE, IN NO EVENT WILL THE LICENSOR BE LIABLE
     TO YOU ON ANY LEGAL THEORY (INCLUDING, WITHOUT LIMITATION,
     NEGLIGENCE) OR OTHERWISE FOR ANY DIRECT, SPECIAL, INDIRECT,
     INCIDENTAL, CONSEQUENTIAL, PUNITIVE, EXEMPLARY, OR OTHER LOSSES,
     COSTS, EXPENSES, OR DAMAGES ARISING OUT OF THIS PUBLIC LICENSE OR
     USE OF THE LICENSED MATERIAL, EVEN IF THE LICENSOR HAS BEEN
     ADVISED OF THE POSSIBILITY OF SUCH LOSSES, COSTS, EXPENSES, OR
     DAMAGES. WHERE A LIMITATION OF LIABILITY IS NOT ALLOWED IN FULL OR
     IN PART, THIS LIMITATION MAY NOT APPLY TO YOU.

  c. The disclaimer of warranties and limitation of liability provided
     above shall be interpreted in a manner that, to the extent
     possible, most closely approximates an absolute disclaimer and
     waiver of all liability.


Section 6 -- Term and Termination.

  a. This Public License applies for the term of the Copyright and
     Similar Rights licensed here. However, if You fail to comply with
     this Public License, then Your rights under this Public License
     terminate automatically.

  b. Where Your right to use the Licensed Material has terminated under
     Section 6(a), it reinstates:

       1. automatically as of the date the violation is cured, provided
          it is cured within 30 days of Your discovery of the
          violation; or

       2. upon express reinstatement by the Licensor.

     For the avoidance of doubt, this Section 6(b) does not affect any
     right the Licensor may have to seek remedies for Your violations
     of this Public License.

  c. For the avoidance of doubt, the Licensor may also offer the
     Licensed Material under separate terms or conditions or stop
     distributing the Licensed Material at any time; however, doing so
     will not terminate this Public License.

  d. Sections 1, 5, 6, 7, and 8 survive termination of this Public
     License.


Section 7 -- Other Terms and Conditions.

  a. The Licensor shall not be bound by any additional or different
     terms or conditions communicated by You unless expressly agreed.

  b. Any arrangements, understandings, or agreements regarding the
     Licensed Material not stated herein are separate from and
     independent of the terms and conditions of this Public License.


Section 8 -- Interpretation.

  a. For the avoidance of doubt, this Public License does not, and
     shall not be interpreted to, reduce, limit, restrict, or impose
     conditions on any use of the Licensed Material that could lawfully
     be made without permission under this Public License.

  b. To the extent possible, if any provision of this Public License is
     deemed unenforceable, it shall be automatically reformed to the
     minimum extent necessary to make it enforceable. If the provision
     cannot be reformed, it shall be severed from this Public License
     without affecting the enforceability of the remaining terms and
     conditions.

  c. No term or condition of this Public License will be waived and no
     failure to comply consented to unless expressly agreed to by the
     Licensor.

  d. Nothing in this Public License constitutes or may be interpreted
     as a limitation upon, or waiver of, any privileges and immunities
     that apply to the Licensor or You, including from the legal
     processes of any jurisdiction or authority.

=======================================================================

Creative Commons is not a party to its public licenses.
Notwithstanding, Creative Commons may elect to apply one of its public
licenses to material it publishes and in those instances will be
considered the "Licensor." Except for the limited purpose of indicating
that material is shared under a Creative Commons public license or as
otherwise permitted by the Creative Commons policies published at
creativecommons.org/policies, Creative Commons does not authorize the
use of the trademark "Creative Commons" or any other trademark or logo
of Creative Commons without its prior written consent including,
without limitation, in connection with any unauthorized modifications
to any of its public licenses or any other arrangements,
understandings, or agreements concerning use of licensed material. For
the avoidance of doubt, this paragraph does not form part of the public
licenses.

Creative Commons may be contacted at creativecommons.org.


==> license-texts/doclicense-CC-by-nd-3.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NoDerivs 3.0 Unported}





\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES
NOT PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE
DOES NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE
COMMONS PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS.
CREATIVE COMMONS MAKES NO WARRANTIES REGARDING THE
INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR DAMAGES
RESULTING FROM ITS USE.
\end{quotation}
\subsubsection{\emph{License}}
\par THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS
OF THIS CREATIVE COMMONS PUBLIC LICENSE (``CCPL'' OR
``LICENSE''). THE WORK IS PROTECTED BY COPYRIGHT AND/OR OTHER
APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS
PROHIBITED.
\par BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU
ACCEPT AND AGREE TO BE BOUND BY THE TERMS OF THIS LICENSE.
TO THE EXTENT THIS LICENSE MAY BE CONSIDERED TO BE A
CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS CONTAINED HERE
IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.
\par \textbf{1. Definitions}
\begin{enumerate}
\item \textbf{``Adaptation''} means a work based upon
the Work, or upon the Work and other pre-existing works,
such as a translation, adaptation, derivative work,
arrangement of music or other alterations of a literary
or artistic work, or phonogram or performance and
includes cinematographic adaptations or any other form in
which the Work may be recast, transformed, or adapted
including in any form recognizably derived from the
original, except that a work that constitutes a
Collection will not be considered an Adaptation for the
purpose of this License. For the avoidance of doubt,
where the Work is a musical work, performance or
phonogram, the synchronization of the Work in
timed-relation with a moving image (``synching'') will be
considered an Adaptation for the purpose of this
License.
\item \textbf{``Collection''} means a collection of
literary or artistic works, such as encyclopedias and
anthologies, or performances, phonograms or broadcasts,
or other works or subject matter other than works listed
in Section 1(f) below, which, by reason of the selection
and arrangement of their contents, constitute
intellectual creations, in which the Work is included in
its entirety in unmodified form along with one or more
other contributions, each constituting separate and
independent works in themselves, which together are
assembled into a collective whole. A work that
constitutes a Collection will not be considered an
Adaptation (as defined above) for the purposes of this
License.
\item \textbf{``Distribute''} means to make available
to the public the original and copies of the Work through
sale or other transfer of ownership.
\item \textbf{``Licensor''} means the individual,
individuals, entity or entities that offer(s) the Work
under the terms of this License.
\item \textbf{``Original Author''} means, in the case
of a literary or artistic work, the individual,
individuals, entity or entities who created the Work or
if no individual or entity can be identified, the
publisher; and in addition (i) in the case of a
performance the actors, singers, musicians, dancers, and
other persons who act, sing, deliver, declaim, play in,
interpret or otherwise perform literary or artistic works
or expressions of folklore; (ii) in the case of a
phonogram the producer being the person or legal entity
who first fixes the sounds of a performance or other
sounds; and, (iii) in the case of broadcasts, the
organization that transmits the broadcast.
\item \textbf{``Work''} means the literary and/or
artistic work offered under the terms of this License
including without limitation any production in the
literary, scientific and artistic domain, whatever may be
the mode or form of its expression including digital
form, such as a book, pamphlet and other writing; a
lecture, address, sermon or other work of the same
nature; a dramatic or dramatico-musical work; a
choreographic work or entertainment in dumb show; a
musical composition with or without words; a
cinematographic work to which are assimilated works
expressed by a process analogous to cinematography; a
work of drawing, painting, architecture, sculpture,
engraving or lithography; a photographic work to which
are assimilated works expressed by a process analogous to
photography; a work of applied art; an illustration, map,
plan, sketch or three-dimensional work relative to
geography, topography, architecture or science; a
performance; a broadcast; a phonogram; a compilation of
data to the extent it is protected as a copyrightable
work; or a work performed by a variety or circus
performer to the extent it is not otherwise considered a
literary or artistic work.
\item \textbf{``You''} means an individual or entity
exercising rights under this License who has not
previously violated the terms of this License with
respect to the Work, or who has received express
permission from the Licensor to exercise rights under
this License despite a previous violation.
\item \textbf{``Publicly Perform''} means to perform
public recitations of the Work and to communicate to the
public those public recitations, by any means or process,
including by wire or wireless means or public digital
performances; to make available to the public Works in
such a way that members of the public may access these
Works from a place and at a place individually chosen by
them; to perform the Work to the public by any means or
process and the communication to the public of the
performances of the Work, including by public digital
performance; to broadcast and rebroadcast the Work by any
means including signs, sounds or images.
\item \textbf{``Reproduce''} means to make copies of
the Work by any means including without limitation by
sound or visual recordings and the right of fixation and
reproducing fixations of the Work, including storage of a
protected performance or phonogram in digital form or
other electronic medium.
\end{enumerate}
\par \textbf{2. Fair Dealing Rights.} Nothing in this
License is intended to reduce, limit, or restrict any uses
free from copyright or rights arising from limitations or
exceptions that are provided for in connection with the
copyright protection under copyright law or other
applicable laws.
\par \textbf{3. License Grant.} Subject to the terms
and conditions of this License, Licensor hereby grants You
a worldwide, royalty-free, non-exclusive, perpetual (for
the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:
\begin{enumerate}
\item to Reproduce the Work, to incorporate the Work into
one or more Collections, and to Reproduce the Work as
incorporated in the Collections; and,
\item to Distribute and Publicly Perform the Work including
as incorporated in Collections.
\item 
\par For the avoidance of doubt:
\begin{enumerate}
\item \textbf{Non-waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme cannot be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License;
\item \textbf{Waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme can be waived, the
Licensor waives the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License; and,
\item \textbf{Voluntary License Schemes}. The
Licensor waives the right to collect royalties,
whether individually or, in the event that the
Licensor is a member of a collecting society that
administers voluntary licensing schemes, via that
society, from any exercise by You of the rights
granted under this License.
\end{enumerate}

\end{enumerate}
\par The above rights may be exercised in all media and
formats whether now known or hereafter devised. The above
rights include the right to make such modifications as are
technically necessary to exercise the rights in other media
and formats, but otherwise you have no rights to make
Adaptations. Subject to Section 8(f), all rights not
expressly granted by Licensor are hereby reserved.
\par \textbf{4. Restrictions.} The license granted in
Section 3 above is expressly made subject to and limited by
the following restrictions:
\begin{enumerate}
\item You may Distribute or Publicly Perform the Work only
under the terms of this License. You must include a copy
of, or the Uniform Resource Identifier (URI) for, this
License with every copy of the Work You Distribute or
Publicly Perform. You may not offer or impose any terms
on the Work that restrict the terms of this License or
the ability of the recipient of the Work to exercise the
rights granted to that recipient under the terms of the
License. You may not sublicense the Work. You must keep
intact all notices that refer to this License and to the
disclaimer of warranties with every copy of the Work You
Distribute or Publicly Perform. When You Distribute or
Publicly Perform the Work, You may not impose any
effective technological measures on the Work that
restrict the ability of a recipient of the Work from You
to exercise the rights granted to that recipient under
the terms of the License. This Section 4(a) applies to
the Work as incorporated in a Collection, but this does
not require the Collection apart from the Work itself to
be made subject to the terms of this License. If You
create a Collection, upon notice from any Licensor You
must, to the extent practicable, remove from the
Collection any credit as required by Section 4(b), as
requested.
\item If You Distribute, or Publicly Perform the Work or
Collections, You must, unless a request has been made
pursuant to Section 4(a), keep intact all copyright
notices for the Work and provide, reasonable to the
medium or means You are utilizing: (i) the name of the
Original Author (or pseudonym, if applicable) if
supplied, and/or if the Original Author and/or Licensor
designate another party or parties (e.g., a sponsor
institute, publishing entity, journal) for attribution
(``Attribution Parties'') in Licensor's copyright notice,
terms of service or by other reasonable means, the name
of such party or parties; (ii) the title of the Work if
supplied; (iii) to the extent reasonably practicable, the
URI, if any, that Licensor specifies to be associated
with the Work, unless such URI does not refer to the
copyright notice or licensing information for the Work.
The credit required by this Section 4(b) may be
implemented in any reasonable manner; provided, however,
that in the case of a Collection, at a minimum such
credit will appear, if a credit for all contributing
authors of the Collection appears, then as part of these
credits and in a manner at least as prominent as the
credits for the other contributing authors. For the
avoidance of doubt, You may only use the credit required
by this Section for the purpose of attribution in the
manner set out above and, by exercising Your rights under
this License, You may not implicitly or explicitly assert
or imply any connection with, sponsorship or endorsement
by the Original Author, Licensor and/or Attribution
Parties, as appropriate, of You or Your use of the Work,
without the separate, express prior written permission of
the Original Author, Licensor and/or Attribution
Parties.
\item Except as otherwise agreed in writing by the Licensor
or as may be otherwise permitted by applicable law, if
You Reproduce, Distribute or Publicly Perform the Work
either by itself or as part of any Collections, You must
not distort, mutilate, modify or take other derogatory
action in relation to the Work which would be prejudicial
to the Original Author's honor or reputation.
\end{enumerate}
\par \textbf{5. Representations, Warranties and
Disclaimer}
\par UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN
WRITING, LICENSOR OFFERS THE WORK AS-IS AND MAKES NO
REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING,
WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE
ABSENCE OF LATENT OR OTHER DEFECTS, ACCURACY, OR THE
PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT DISCOVERABLE.
SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.
\par \textbf{6. Limitation on Liability.} EXCEPT TO
THE EXTENT REQUIRED BY APPLICABLE LAW, IN NO EVENT WILL
LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR ANY
SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY
DAMAGES ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK,
EVEN IF LICENSOR HAS BEEN ADVISED OF THE POSSIBILITY OF
SUCH DAMAGES.
\par \textbf{7. Termination}
\begin{enumerate}
\item This License and the rights granted hereunder will
terminate automatically upon any breach by You of the
terms of this License. Individuals or entities who have
received Collections from You under this License,
however, will not have their licenses terminated provided
such individuals or entities remain in full compliance
with those licenses. Sections 1, 2, 5, 6, 7, and 8 will
survive any termination of this License.
\item Subject to the above terms and conditions, the
license granted here is perpetual (for the duration of
the applicable copyright in the Work). Notwithstanding
the above, Licensor reserves the right to release the
Work under different license terms or to stop
distributing the Work at any time; provided, however that
any such election will not serve to withdraw this License
(or any other license that has been, or is required to
be, granted under the terms of this License), and this
License will continue in full force and effect unless
terminated as stated above.
\end{enumerate}
\par \textbf{8. Miscellaneous}
\begin{enumerate}
\item Each time You Distribute or Publicly Perform the Work
or a Collection, the Licensor offers to the recipient a
license to the Work on the same terms and conditions as
the license granted to You under this License.
\item If any provision of this License is invalid or
unenforceable under applicable law, it shall not affect
the validity or enforceability of the remainder of the
terms of this License, and without further action by the
parties to this agreement, such provision shall be
reformed to the minimum extent necessary to make such
provision valid and enforceable.
\item No term or provision of this License shall be deemed
waived and no breach consented to unless such waiver or
consent shall be in writing and signed by the party to be
charged with such waiver or consent.
\item This License constitutes the entire agreement between
the parties with respect to the Work licensed here. There
are no understandings, agreements or representations with
respect to the Work not specified here. Licensor shall
not be bound by any additional provisions that may appear
in any communication from You. This License may not be
modified without the mutual written agreement of the
Licensor and You.
\item The rights granted under, and the subject matter
referenced, in this License were drafted utilizing the
terminology of the Berne Convention for the Protection of
Literary and Artistic Works (as amended on September 28,
1979), the Rome Convention of 1961, the WIPO Copyright
Treaty of 1996, the WIPO Performances and Phonograms
Treaty of 1996 and the Universal Copyright Convention (as
revised on July 24, 1971). These rights and subject
matter take effect in the relevant jurisdiction in which
the License terms are sought to be enforced according to
the corresponding provisions of the implementation of
those treaty provisions in the applicable national law.
If the standard suite of rights granted under applicable
copyright law includes additional rights not granted
under this License, such additional rights are deemed to
be included in the License; this License is not intended
to restrict the license of any rights under applicable
law.
\end{enumerate}
 
\begin{quotation}
\subsubsection{Creative Commons Notice}
\par Creative Commons is not a party to this License, and
makes no warranty whatsoever in connection with the Work.
Creative Commons will not be liable to You or any party
on any legal theory for any damages whatsoever, including
without limitation any general, special, incidental or
consequential damages arising in connection to this
license. Notwithstanding the foregoing two (2) sentences,
if Creative Commons has expressly identified itself as
the Licensor hereunder, it shall have all rights and
obligations of Licensor.
\par Except for the limited purpose of indicating to the
public that the Work is licensed under the CCPL, Creative
Commons does not authorize the use by either party of the
trademark ``Creative Commons'' or any related trademark or
logo of Creative Commons without the prior written
consent of Creative Commons. Any permitted use will be in
compliance with Creative Commons' then-current trademark
usage guidelines, as may be published on its website or
otherwise made available upon request from time to time.
For the avoidance of doubt, this trademark restriction
does not form part of this License.
\par Creative Commons may be contacted at \url{https://creativecommons.org/}.
\end{quotation} 



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nd-3.0-plaintext.tex <==
Creative Commons Legal Code

Attribution-NoDerivs 3.0 Unported

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR
    DAMAGES RESULTING FROM ITS USE.

License

THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS OF THIS CREATIVE
COMMONS PUBLIC LICENSE ("CCPL" OR "LICENSE"). THE WORK IS PROTECTED BY
COPYRIGHT AND/OR OTHER APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS PROHIBITED.

BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU ACCEPT AND AGREE
TO BE BOUND BY THE TERMS OF THIS LICENSE. TO THE EXTENT THIS LICENSE MAY
BE CONSIDERED TO BE A CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS
CONTAINED HERE IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.

1. Definitions

 a. "Adaptation" means a work based upon the Work, or upon the Work and
    other pre-existing works, such as a translation, adaptation,
    derivative work, arrangement of music or other alterations of a
    literary or artistic work, or phonogram or performance and includes
    cinematographic adaptations or any other form in which the Work may be
    recast, transformed, or adapted including in any form recognizably
    derived from the original, except that a work that constitutes a
    Collection will not be considered an Adaptation for the purpose of
    this License. For the avoidance of doubt, where the Work is a musical
    work, performance or phonogram, the synchronization of the Work in
    timed-relation with a moving image ("synching") will be considered an
    Adaptation for the purpose of this License.
 b. "Collection" means a collection of literary or artistic works, such as
    encyclopedias and anthologies, or performances, phonograms or
    broadcasts, or other works or subject matter other than works listed
    in Section 1(f) below, which, by reason of the selection and
    arrangement of their contents, constitute intellectual creations, in
    which the Work is included in its entirety in unmodified form along
    with one or more other contributions, each constituting separate and
    independent works in themselves, which together are assembled into a
    collective whole. A work that constitutes a Collection will not be
    considered an Adaptation (as defined above) for the purposes of this
    License.
 c. "Distribute" means to make available to the public the original and
    copies of the Work through sale or other transfer of ownership.
 d. "Licensor" means the individual, individuals, entity or entities that
    offer(s) the Work under the terms of this License.
 e. "Original Author" means, in the case of a literary or artistic work,
    the individual, individuals, entity or entities who created the Work
    or if no individual or entity can be identified, the publisher; and in
    addition (i) in the case of a performance the actors, singers,
    musicians, dancers, and other persons who act, sing, deliver, declaim,
    play in, interpret or otherwise perform literary or artistic works or
    expressions of folklore; (ii) in the case of a phonogram the producer
    being the person or legal entity who first fixes the sounds of a
    performance or other sounds; and, (iii) in the case of broadcasts, the
    organization that transmits the broadcast.
 f. "Work" means the literary and/or artistic work offered under the terms
    of this License including without limitation any production in the
    literary, scientific and artistic domain, whatever may be the mode or
    form of its expression including digital form, such as a book,
    pamphlet and other writing; a lecture, address, sermon or other work
    of the same nature; a dramatic or dramatico-musical work; a
    choreographic work or entertainment in dumb show; a musical
    composition with or without words; a cinematographic work to which are
    assimilated works expressed by a process analogous to cinematography;
    a work of drawing, painting, architecture, sculpture, engraving or
    lithography; a photographic work to which are assimilated works
    expressed by a process analogous to photography; a work of applied
    art; an illustration, map, plan, sketch or three-dimensional work
    relative to geography, topography, architecture or science; a
    performance; a broadcast; a phonogram; a compilation of data to the
    extent it is protected as a copyrightable work; or a work performed by
    a variety or circus performer to the extent it is not otherwise
    considered a literary or artistic work.
 g. "You" means an individual or entity exercising rights under this
    License who has not previously violated the terms of this License with
    respect to the Work, or who has received express permission from the
    Licensor to exercise rights under this License despite a previous
    violation.
 h. "Publicly Perform" means to perform public recitations of the Work and
    to communicate to the public those public recitations, by any means or
    process, including by wire or wireless means or public digital
    performances; to make available to the public Works in such a way that
    members of the public may access these Works from a place and at a
    place individually chosen by them; to perform the Work to the public
    by any means or process and the communication to the public of the
    performances of the Work, including by public digital performance; to
    broadcast and rebroadcast the Work by any means including signs,
    sounds or images.
 i. "Reproduce" means to make copies of the Work by any means including
    without limitation by sound or visual recordings and the right of
    fixation and reproducing fixations of the Work, including storage of a
    protected performance or phonogram in digital form or other electronic
    medium.

2. Fair Dealing Rights. Nothing in this License is intended to reduce,
limit, or restrict any uses free from copyright or rights arising from
limitations or exceptions that are provided for in connection with the
copyright protection under copyright law or other applicable laws.

3. License Grant. Subject to the terms and conditions of this License,
Licensor hereby grants You a worldwide, royalty-free, non-exclusive,
perpetual (for the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:

 a. to Reproduce the Work, to incorporate the Work into one or more
    Collections, and to Reproduce the Work as incorporated in the
    Collections; and,
 b. to Distribute and Publicly Perform the Work including as incorporated
    in Collections.
 c. For the avoidance of doubt:

     i. Non-waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme cannot be waived, the Licensor
        reserves the exclusive right to collect such royalties for any
        exercise by You of the rights granted under this License;
    ii. Waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme can be waived, the Licensor waives the
        exclusive right to collect such royalties for any exercise by You
        of the rights granted under this License; and,
   iii. Voluntary License Schemes. The Licensor waives the right to
        collect royalties, whether individually or, in the event that the
        Licensor is a member of a collecting society that administers
        voluntary licensing schemes, via that society, from any exercise
        by You of the rights granted under this License.

The above rights may be exercised in all media and formats whether now
known or hereafter devised. The above rights include the right to make
such modifications as are technically necessary to exercise the rights in
other media and formats, but otherwise you have no rights to make
Adaptations. Subject to Section 8(f), all rights not expressly granted by
Licensor are hereby reserved.

4. Restrictions. The license granted in Section 3 above is expressly made
subject to and limited by the following restrictions:

 a. You may Distribute or Publicly Perform the Work only under the terms
    of this License. You must include a copy of, or the Uniform Resource
    Identifier (URI) for, this License with every copy of the Work You
    Distribute or Publicly Perform. You may not offer or impose any terms
    on the Work that restrict the terms of this License or the ability of
    the recipient of the Work to exercise the rights granted to that
    recipient under the terms of the License. You may not sublicense the
    Work. You must keep intact all notices that refer to this License and
    to the disclaimer of warranties with every copy of the Work You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Work, You may not impose any effective technological
    measures on the Work that restrict the ability of a recipient of the
    Work from You to exercise the rights granted to that recipient under
    the terms of the License. This Section 4(a) applies to the Work as
    incorporated in a Collection, but this does not require the Collection
    apart from the Work itself to be made subject to the terms of this
    License. If You create a Collection, upon notice from any Licensor You
    must, to the extent practicable, remove from the Collection any credit
    as required by Section 4(b), as requested.
 b. If You Distribute, or Publicly Perform the Work or Collections, You
    must, unless a request has been made pursuant to Section 4(a), keep
    intact all copyright notices for the Work and provide, reasonable to
    the medium or means You are utilizing: (i) the name of the Original
    Author (or pseudonym, if applicable) if supplied, and/or if the
    Original Author and/or Licensor designate another party or parties
    (e.g., a sponsor institute, publishing entity, journal) for
    attribution ("Attribution Parties") in Licensor's copyright notice,
    terms of service or by other reasonable means, the name of such party
    or parties; (ii) the title of the Work if supplied; (iii) to the
    extent reasonably practicable, the URI, if any, that Licensor
    specifies to be associated with the Work, unless such URI does not
    refer to the copyright notice or licensing information for the Work.
    The credit required by this Section 4(b) may be implemented in any
    reasonable manner; provided, however, that in the case of a
    Collection, at a minimum such credit will appear, if a credit for all
    contributing authors of the Collection appears, then as part of these
    credits and in a manner at least as prominent as the credits for the
    other contributing authors. For the avoidance of doubt, You may only
    use the credit required by this Section for the purpose of attribution
    in the manner set out above and, by exercising Your rights under this
    License, You may not implicitly or explicitly assert or imply any
    connection with, sponsorship or endorsement by the Original Author,
    Licensor and/or Attribution Parties, as appropriate, of You or Your
    use of the Work, without the separate, express prior written
    permission of the Original Author, Licensor and/or Attribution
    Parties.
 c. Except as otherwise agreed in writing by the Licensor or as may be
    otherwise permitted by applicable law, if You Reproduce, Distribute or
    Publicly Perform the Work either by itself or as part of any
    Collections, You must not distort, mutilate, modify or take other
    derogatory action in relation to the Work which would be prejudicial
    to the Original Author's honor or reputation.

5. Representations, Warranties and Disclaimer

UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN WRITING, LICENSOR
OFFERS THE WORK AS-IS AND MAKES NO REPRESENTATIONS OR WARRANTIES OF ANY
KIND CONCERNING THE WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE,
INCLUDING, WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE ABSENCE OF
LATENT OR OTHER DEFECTS, ACCURACY, OR THE PRESENCE OF ABSENCE OF ERRORS,
WHETHER OR NOT DISCOVERABLE. SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION
OF IMPLIED WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.

6. Limitation on Liability. EXCEPT TO THE EXTENT REQUIRED BY APPLICABLE
LAW, IN NO EVENT WILL LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR
ANY SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY DAMAGES
ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK, EVEN IF LICENSOR HAS
BEEN ADVISED OF THE POSSIBILITY OF SUCH DAMAGES.

7. Termination

 a. This License and the rights granted hereunder will terminate
    automatically upon any breach by You of the terms of this License.
    Individuals or entities who have received Collections from You under
    this License, however, will not have their licenses terminated
    provided such individuals or entities remain in full compliance with
    those licenses. Sections 1, 2, 5, 6, 7, and 8 will survive any
    termination of this License.
 b. Subject to the above terms and conditions, the license granted here is
    perpetual (for the duration of the applicable copyright in the Work).
    Notwithstanding the above, Licensor reserves the right to release the
    Work under different license terms or to stop distributing the Work at
    any time; provided, however that any such election will not serve to
    withdraw this License (or any other license that has been, or is
    required to be, granted under the terms of this License), and this
    License will continue in full force and effect unless terminated as
    stated above.

8. Miscellaneous

 a. Each time You Distribute or Publicly Perform the Work or a Collection,
    the Licensor offers to the recipient a license to the Work on the same
    terms and conditions as the license granted to You under this License.
 b. If any provision of this License is invalid or unenforceable under
    applicable law, it shall not affect the validity or enforceability of
    the remainder of the terms of this License, and without further action
    by the parties to this agreement, such provision shall be reformed to
    the minimum extent necessary to make such provision valid and
    enforceable.
 c. No term or provision of this License shall be deemed waived and no
    breach consented to unless such waiver or consent shall be in writing
    and signed by the party to be charged with such waiver or consent.
 d. This License constitutes the entire agreement between the parties with
    respect to the Work licensed here. There are no understandings,
    agreements or representations with respect to the Work not specified
    here. Licensor shall not be bound by any additional provisions that
    may appear in any communication from You. This License may not be
    modified without the mutual written agreement of the Licensor and You.
 e. The rights granted under, and the subject matter referenced, in this
    License were drafted utilizing the terminology of the Berne Convention
    for the Protection of Literary and Artistic Works (as amended on
    September 28, 1979), the Rome Convention of 1961, the WIPO Copyright
    Treaty of 1996, the WIPO Performances and Phonograms Treaty of 1996
    and the Universal Copyright Convention (as revised on July 24, 1971).
    These rights and subject matter take effect in the relevant
    jurisdiction in which the License terms are sought to be enforced
    according to the corresponding provisions of the implementation of
    those treaty provisions in the applicable national law. If the
    standard suite of rights granted under applicable copyright law
    includes additional rights not granted under this License, such
    additional rights are deemed to be included in the License; this
    License is not intended to restrict the license of any rights under
    applicable law.


Creative Commons Notice

    Creative Commons is not a party to this License, and makes no warranty
    whatsoever in connection with the Work. Creative Commons will not be
    liable to You or any party on any legal theory for any damages
    whatsoever, including without limitation any general, special,
    incidental or consequential damages arising in connection to this
    license. Notwithstanding the foregoing two (2) sentences, if Creative
    Commons has expressly identified itself as the Licensor hereunder, it
    shall have all rights and obligations of Licensor.

    Except for the limited purpose of indicating to the public that the
    Work is licensed under the CCPL, Creative Commons does not authorize
    the use by either party of the trademark "Creative Commons" or any
    related trademark or logo of Creative Commons without the prior
    written consent of Creative Commons. Any permitted use will be in
    compliance with Creative Commons' then-current trademark usage
    guidelines, as may be published on its website or otherwise made
    available upon request from time to time. For the avoidance of doubt,
    this trademark restriction does not form part of this License.

    Creative Commons may be contacted at https://creativecommons.org/.


==> license-texts/doclicense-CC-by-nd-4.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-NoDerivatives 4.0 International}







Official translations of this license are available in other languages.



\par Creative Commons Corporation (“Creative Commons”) is not a law firm and does not provide legal services or legal advice. Distribution of Creative Commons public licenses does not create a lawyer-client or other relationship. Creative Commons makes its licenses and related information available on an “as-is” basis. Creative Commons gives no warranties regarding its licenses, any material licensed under their terms and conditions, or any related information. Creative Commons disclaims all liability for damages resulting from their use to the fullest extent possible.


\par \textbf{Using Creative Commons Public Licenses}
\par Creative Commons public licenses provide a standard set of terms and conditions that creators and other rights holders may use to share original works of authorship and other material subject to copyright and certain other rights specified in the public license below. The following considerations are for informational purposes only, are not exhaustive, and do not form part of our licenses.
\begin{quotation}\textbf{Considerations for licensors:} Our public licenses are intended for use by those authorized to give the public permission to use material in ways otherwise restricted by copyright and certain other rights. Our licenses are irrevocable. Licensors should read and understand the terms and conditions of the license they choose before applying it. Licensors should also secure all rights necessary before applying our licenses so that the public can reuse the material as expected. Licensors should clearly mark any material not subject to the license. This includes other CC-licensed material, or material used under an exception or limitation to copyright. More considerations for licensors.\end{quotation}
\begin{quotation}\textbf{Considerations for the public:} By using one of our public licenses, a licensor grants the public permission to use the licensed material under specified terms and conditions. If the licensor’s permission is not necessary for any reason–for example, because of any applicable exception or limitation to copyright–then that use is not regulated by the license. Our licenses grant only permissions under copyright and certain other rights that a licensor has authority to grant. Use of the licensed material may still be restricted for other reasons, including because others have copyright or other rights in the material. A licensor may make special requests, such as asking that all changes be marked or described. Although not required by our licenses, you are encouraged to respect those requests where reasonable.
More considerations for the public.\end{quotation}

\subsubsection{Creative Commons Attribution-NoDerivatives 4.0 International Public License}
\par By exercising the Licensed Rights (defined below), You accept and agree to be bound by the terms and conditions of this Creative Commons Attribution-NoDerivatives 4.0 International Public License (``Public License''). To the extent this Public License may be interpreted as a contract, You are granted the Licensed Rights in consideration of Your acceptance of these terms and conditions, and the Licensor grants You such rights in consideration of benefits the Licensor receives from making the Licensed Material available under these terms and conditions.
\par \textbf{Section 1 – Definitions.}
\begin{enumerate}
\item \textbf{Adapted Material} means material subject to Copyright and Similar Rights that is derived from or based upon the Licensed Material and in which the Licensed Material is translated, altered, arranged, transformed, or otherwise modified in a manner requiring permission under the Copyright and Similar Rights held by the Licensor. For purposes of this Public License, where the Licensed Material is a musical work, performance, or sound recording, Adapted Material is always produced where the Licensed Material is synched in timed relation with a moving image.
\item \textbf{Copyright and Similar Rights} means copyright and/or similar rights closely related to copyright including, without limitation, performance, broadcast, sound recording, and Sui Generis Database Rights, without regard to how the rights are labeled or categorized. For purposes of this Public License, the rights specified in Section 2(b)(1)-(2) are not Copyright and Similar Rights.
\item \textbf{Effective Technological Measures} means those measures that, in the absence of proper authority, may not
be circumvented under laws fulfilling obligations under Article 11 of the WIPO Copyright Treaty adopted on December 20, 1996, and/or similar
international agreements.
\item \textbf{Exceptions and Limitations} means fair use, fair dealing, and/or any other exception or limitation to Copyright and Similar Rights that applies to Your use of the Licensed Material.
\item \textbf{Licensed Material} means the artistic or literary work, database, or other material to which the Licensor applied this Public License.
\item \textbf{Licensed Rights} means the rights granted to You subject to the terms and conditions of this Public License, which are limited to all Copyright and Similar Rights that apply to Your use of the Licensed Material and that the Licensor has authority to license.
\item \textbf{Licensor} means the individual(s) or entity(ies) granting rights under this Public License.
\item \textbf{Share} means to provide material to the public by any means or process that requires permission under the Licensed Rights, such as reproduction, public display, public performance, distribution, dissemination, communication, or importation, and to make material available to the public including in ways that members of the public may access the material from a place and at a time individually chosen by them.
\item \textbf{Sui Generis Database Rights} means rights other than copyright resulting from Directive 96/9/EC of the European Parliament and of the Council of 11 March 1996 on the legal protection of databases, as amended and/or succeeded, as well as other essentially equivalent rights anywhere in the world.
\item \textbf{You} means the individual or entity exercising the Licensed Rights under this Public License. \textbf{Your} has a corresponding meaning.
\end{enumerate}
\par \textbf{Section 2 – Scope.}
\begin{enumerate}
\item \textbf{License grant}.
\begin{enumerate}
\item Subject to the terms and conditions of this Public License, the Licensor hereby grants You a worldwide, royalty-free, non-sublicensable, non-exclusive, irrevocable license to exercise the Licensed Rights in the Licensed Material to:
\begin{enumerate}
\item reproduce and Share the Licensed Material, in whole or in part; and
\item produce and reproduce, but not Share, Adapted Material.
\end{enumerate}
\item Exceptions and Limitations. For the avoidance of doubt, where Exceptions and Limitations apply to Your use, this Public License does not apply, and You do not need to comply with its terms and conditions.
\item Term. The term of this Public License is specified in Section 6(a).
\item Media and formats; technical modifications allowed. The Licensor authorizes You to exercise the Licensed Rights in all media and formats whether now known or hereafter created, and to make technical modifications necessary to do so. The Licensor waives and/or agrees not to assert any right or authority to forbid You from making technical modifications necessary to exercise the Licensed Rights, including technical modifications necessary to circumvent Effective Technological Measures. For purposes of this Public License, simply making modifications authorized by this Section 2(a)(4) never produces Adapted Material.
\item Downstream recipients.

\begin{enumerate}
\item Offer from the Licensor – Licensed Material. Every recipient of the Licensed Material automatically receives an offer from the Licensor to exercise the Licensed Rights under the terms and conditions of this Public License.
\item No downstream restrictions. You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, the Licensed Material if doing so restricts exercise of the Licensed Rights by any recipient of the Licensed Material.
\end{enumerate}

\item No endorsement. Nothing in this Public License constitutes or may be construed as permission to assert or imply that You are, or that Your use of the Licensed Material is, connected with, or sponsored, endorsed, or granted official status by, the Licensor or others designated to receive attribution as provided in Section 3(a)(1)(A)(i).
\end{enumerate}
\item \par \textbf{Other rights}.
\begin{enumerate}
\item Moral rights, such as the right of integrity, are not licensed under this Public License, nor are publicity, privacy, and/or other similar personality rights; however, to the extent possible, the Licensor waives and/or agrees not to assert any such rights held by the Licensor to the limited extent necessary to allow You to exercise the Licensed Rights, but not otherwise.
\item Patent and trademark rights are not licensed under this Public License.
\item To the extent possible, the Licensor waives any right to collect royalties from You for the exercise of the Licensed Rights, whether directly or through a collecting society under any voluntary or waivable statutory or compulsory licensing scheme. In all other cases the Licensor expressly reserves any right to collect such royalties.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 3 – License Conditions.}
\par Your exercise of the Licensed Rights is expressly made subject to the following conditions.
\begin{enumerate}
\item \par \textbf{Attribution}.
\begin{enumerate}
\item \par If You Share the Licensed Material, You must:
\begin{enumerate}
\item retain the following if it is supplied by the Licensor with the Licensed Material:
\begin{enumerate}
\item identification of the creator(s) of the Licensed Material and any others designated to receive attribution, in any reasonable manner requested by the Licensor (including by pseudonym if designated);
\item a copyright notice;
\item a notice that refers to this Public License; 
\item a notice that refers to the disclaimer of warranties;
\item a URI or hyperlink to the Licensed Material to the extent reasonably practicable;
\end{enumerate}
\item indicate if You modified the Licensed Material and retain an indication of any previous modifications; and
\item indicate the Licensed Material is licensed under this Public License,
and include the text of, or the URI or hyperlink to, this Public
License.
\end{enumerate}
For the avoidance of doubt, You do not have permission under this Public License to Share Adapted Material.

\item You may satisfy the conditions in Section 3(a)(1) in any reasonable manner based on the medium, means, and context in which You Share the Licensed Material. For example, it may be reasonable to satisfy the conditions by providing a URI or hyperlink to a resource that includes the required information.
\item If requested by the Licensor, You must remove any of the information required by Section 3(a)(1)(A) to the extent reasonably practicable.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 4 – Sui Generis Database Rights.}
\par Where the Licensed Rights include Sui Generis Database Rights that apply to Your use of the Licensed Material:
\begin{enumerate}
\item for the avoidance of doubt, Section 2(a)(1) grants You the right to extract, reuse, reproduce, and Share all or a substantial portion of the contents of the database, provided You do not Share Adapted Material;
\item if You include all or a substantial portion of the database contents in a database in which You have Sui Generis Database Rights, then the database in which You have Sui Generis Database Rights (but not its individual contents) is Adapted Material; and
\item You must comply with the conditions in Section 3(a) if You Share all or a substantial portion of the contents of the database.
\end{enumerate}
For the avoidance of doubt, this Section 4 supplements and does not replace Your obligations under this Public License where the Licensed Rights include other Copyright and Similar Rights.
\par \textbf{Section 5 – Disclaimer of Warranties and Limitation of Liability.}
\begin{enumerate}
\item \textbf{Unless otherwise separately undertaken by the Licensor, to the extent possible, the Licensor offers the Licensed Material as-is and as-available, and makes no representations or warranties of any kind concerning the Licensed Material, whether express, implied, statutory, or other. This includes, without limitation, warranties of title, merchantability, fitness for a particular purpose, non-infringement, absence of latent or other defects, accuracy, or the presence or absence of errors, whether or not known or discoverable. Where disclaimers of warranties are not allowed in full or in part, this disclaimer may not apply to You.}
\item \textbf{To the extent possible, in no event will the Licensor be liable to You on any legal theory (including, without limitation, negligence) or otherwise for any direct, special, indirect, incidental, consequential, punitive, exemplary, or other losses, costs, expenses, or damages arising out of this Public License or use of the Licensed Material, even if the Licensor has been advised of the possibility of such losses, costs, expenses, or damages. Where a limitation of liability is not allowed in full or in part, this limitation may not apply to You.}
\end{enumerate}
\begin{enumerate}
\item The disclaimer of warranties and limitation of liability provided above shall be interpreted in a manner that, to the extent possible, most closely approximates an absolute disclaimer and waiver of all liability.
\end{enumerate}
\par \textbf{Section 6 – Term and Termination.}
\begin{enumerate}
\item This Public License applies for the term of the Copyright and Similar Rights licensed here. However, if You fail to comply with this Public License, then Your rights under this Public License terminate automatically.
\item 
\par Where Your right to use the Licensed Material has terminated under Section 6(a), it reinstates:
\begin{enumerate}
\item automatically as of the date the violation is cured, provided it is cured within 30 days of Your discovery of the violation; or
\item upon express reinstatement by the Licensor.
\end{enumerate}
For the avoidance of doubt, this Section 6(b) does not affect any right the Licensor may have to seek remedies for Your violations of this Public License.
\item For the avoidance of doubt, the Licensor may also offer the Licensed Material under separate terms or conditions or stop distributing the Licensed Material at any time; however, doing so will not terminate this Public License.
\item Sections 1, 5, 6, 7, and 8 survive termination of this Public License.
\end{enumerate}
\par \textbf{Section 7 – Other Terms and Conditions.}
\begin{enumerate}
\item The Licensor shall not be bound by any additional or different terms or conditions communicated by You unless expressly agreed.
\item Any arrangements, understandings, or agreements regarding the Licensed Material not stated herein are separate from and independent of the terms and conditions of this Public License.
\end{enumerate}
\par \textbf{Section 8 – Interpretation.}
\begin{enumerate}
\item For the avoidance of doubt, this Public License does not, and shall not be interpreted to, reduce, limit, restrict, or impose conditions on any use of the Licensed Material that could lawfully be made without permission under this Public License.
\item To the extent possible, if any provision of this Public License is deemed unenforceable, it shall be automatically reformed to the minimum extent necessary to make it enforceable. If the provision cannot be reformed, it shall be severed from this Public License without affecting the enforceability of the remaining terms and conditions.
\item No term or condition of this Public License will be waived and no failure to comply consented to unless expressly agreed to by the Licensor.
\item Nothing in this Public License constitutes or may be interpreted as a limitation upon, or waiver of, any privileges and immunities that apply to the Licensor or You, including from the legal processes of any jurisdiction or authority.
\end{enumerate}
\par Creative Commons is not a party to its public licenses. Notwithstanding, Creative Commons may elect to apply one of its public licenses to material it publishes and in those instances will be considered the “Licensor.” The text of the Creative Commons public licenses is dedicated to the public domain under the CC0 Public Domain Dedication. Except for the limited purpose of indicating that material is shared under a Creative Commons public license or as otherwise permitted by the Creative Commons policies published at creativecommons.org/policies, Creative Commons does not authorize the use of the trademark “Creative Commons” or any other trademark or logo of Creative Commons without its prior written consent including, without limitation, in connection with any unauthorized modifications to any of its public licenses or any other arrangements, understandings, or agreements concerning use of licensed material. For the avoidance of doubt, this paragraph does not form part of the public licenses.\\\\
Creative Commons may be contacted at creativecommons.org.
\par Additional languages available: Bahasa Indonesia, Nederlands, norsk, suomeksi, te reo Māori, українська, 日本語. Please read the FAQ for more information about official translations.


\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-nd-4.0-plaintext.tex <==
Attribution-NoDerivatives 4.0 International

=======================================================================

Creative Commons Corporation ("Creative Commons") is not a law firm and
does not provide legal services or legal advice. Distribution of
Creative Commons public licenses does not create a lawyer-client or
other relationship. Creative Commons makes its licenses and related
information available on an "as-is" basis. Creative Commons gives no
warranties regarding its licenses, any material licensed under their
terms and conditions, or any related information. Creative Commons
disclaims all liability for damages resulting from their use to the
fullest extent possible.

Using Creative Commons Public Licenses

Creative Commons public licenses provide a standard set of terms and
conditions that creators and other rights holders may use to share
original works of authorship and other material subject to copyright
and certain other rights specified in the public license below. The
following considerations are for informational purposes only, are not
exhaustive, and do not form part of our licenses.

     Considerations for licensors: Our public licenses are
     intended for use by those authorized to give the public
     permission to use material in ways otherwise restricted by
     copyright and certain other rights. Our licenses are
     irrevocable. Licensors should read and understand the terms
     and conditions of the license they choose before applying it.
     Licensors should also secure all rights necessary before
     applying our licenses so that the public can reuse the
     material as expected. Licensors should clearly mark any
     material not subject to the license. This includes other CC-
     licensed material, or material used under an exception or
     limitation to copyright. More considerations for licensors:
	wiki.creativecommons.org/Considerations_for_licensors

     Considerations for the public: By using one of our public
     licenses, a licensor grants the public permission to use the
     licensed material under specified terms and conditions. If
     the licensor's permission is not necessary for any reason--for
     example, because of any applicable exception or limitation to
     copyright--then that use is not regulated by the license. Our
     licenses grant only permissions under copyright and certain
     other rights that a licensor has authority to grant. Use of
     the licensed material may still be restricted for other
     reasons, including because others have copyright or other
     rights in the material. A licensor may make special requests,
     such as asking that all changes be marked or described.
     Although not required by our licenses, you are encouraged to
     respect those requests where reasonable. More_considerations
     for the public: 
	wiki.creativecommons.org/Considerations_for_licensees
	

=======================================================================

Creative Commons Attribution-NoDerivatives 4.0 International Public
License

By exercising the Licensed Rights (defined below), You accept and agree
to be bound by the terms and conditions of this Creative Commons
Attribution-NoDerivatives 4.0 International Public License ("Public
License"). To the extent this Public License may be interpreted as a
contract, You are granted the Licensed Rights in consideration of Your
acceptance of these terms and conditions, and the Licensor grants You
such rights in consideration of benefits the Licensor receives from
making the Licensed Material available under these terms and
conditions.


Section 1 -- Definitions.

  a. Adapted Material means material subject to Copyright and Similar
     Rights that is derived from or based upon the Licensed Material
     and in which the Licensed Material is translated, altered,
     arranged, transformed, or otherwise modified in a manner requiring
     permission under the Copyright and Similar Rights held by the
     Licensor. For purposes of this Public License, where the Licensed
     Material is a musical work, performance, or sound recording,
     Adapted Material is always produced where the Licensed Material is
     synched in timed relation with a moving image.

  b. Copyright and Similar Rights means copyright and/or similar rights
     closely related to copyright including, without limitation,
     performance, broadcast, sound recording, and Sui Generis Database
     Rights, without regard to how the rights are labeled or
     categorized. For purposes of this Public License, the rights
     specified in Section 2(b)(1)-(2) are not Copyright and Similar
     Rights.

  c. Effective Technological Measures means those measures that, in the
     absence of proper authority, may not be circumvented under laws
     fulfilling obligations under Article 11 of the WIPO Copyright
     Treaty adopted on December 20, 1996, and/or similar international
     agreements.

  d. Exceptions and Limitations means fair use, fair dealing, and/or
     any other exception or limitation to Copyright and Similar Rights
     that applies to Your use of the Licensed Material.

  e. Licensed Material means the artistic or literary work, database,
     or other material to which the Licensor applied this Public
     License.

  f. Licensed Rights means the rights granted to You subject to the
     terms and conditions of this Public License, which are limited to
     all Copyright and Similar Rights that apply to Your use of the
     Licensed Material and that the Licensor has authority to license.

  g. Licensor means the individual(s) or entity(ies) granting rights
     under this Public License.

  h. Share means to provide material to the public by any means or
     process that requires permission under the Licensed Rights, such
     as reproduction, public display, public performance, distribution,
     dissemination, communication, or importation, and to make material
     available to the public including in ways that members of the
     public may access the material from a place and at a time
     individually chosen by them.

  i. Sui Generis Database Rights means rights other than copyright
     resulting from Directive 96/9/EC of the European Parliament and of
     the Council of 11 March 1996 on the legal protection of databases,
     as amended and/or succeeded, as well as other essentially
     equivalent rights anywhere in the world.

  j. You means the individual or entity exercising the Licensed Rights
     under this Public License. Your has a corresponding meaning.


Section 2 -- Scope.

  a. License grant.

       1. Subject to the terms and conditions of this Public License,
          the Licensor hereby grants You a worldwide, royalty-free,
          non-sublicensable, non-exclusive, irrevocable license to
          exercise the Licensed Rights in the Licensed Material to:

            a. reproduce and Share the Licensed Material, in whole or
               in part; and

            b. produce and reproduce, but not Share, Adapted Material.

       2. Exceptions and Limitations. For the avoidance of doubt, where
          Exceptions and Limitations apply to Your use, this Public
          License does not apply, and You do not need to comply with
          its terms and conditions.

       3. Term. The term of this Public License is specified in Section
          6(a).

       4. Media and formats; technical modifications allowed. The
          Licensor authorizes You to exercise the Licensed Rights in
          all media and formats whether now known or hereafter created,
          and to make technical modifications necessary to do so. The
          Licensor waives and/or agrees not to assert any right or
          authority to forbid You from making technical modifications
          necessary to exercise the Licensed Rights, including
          technical modifications necessary to circumvent Effective
          Technological Measures. For purposes of this Public License,
          simply making modifications authorized by this Section 2(a)
          (4) never produces Adapted Material.

       5. Downstream recipients.

            a. Offer from the Licensor -- Licensed Material. Every
               recipient of the Licensed Material automatically
               receives an offer from the Licensor to exercise the
               Licensed Rights under the terms and conditions of this
               Public License.

            b. No downstream restrictions. You may not offer or impose
               any additional or different terms or conditions on, or
               apply any Effective Technological Measures to, the
               Licensed Material if doing so restricts exercise of the
               Licensed Rights by any recipient of the Licensed
               Material.

       6. No endorsement. Nothing in this Public License constitutes or
          may be construed as permission to assert or imply that You
          are, or that Your use of the Licensed Material is, connected
          with, or sponsored, endorsed, or granted official status by,
          the Licensor or others designated to receive attribution as
          provided in Section 3(a)(1)(A)(i).

  b. Other rights.

       1. Moral rights, such as the right of integrity, are not
          licensed under this Public License, nor are publicity,
          privacy, and/or other similar personality rights; however, to
          the extent possible, the Licensor waives and/or agrees not to
          assert any such rights held by the Licensor to the limited
          extent necessary to allow You to exercise the Licensed
          Rights, but not otherwise.

       2. Patent and trademark rights are not licensed under this
          Public License.

       3. To the extent possible, the Licensor waives any right to
          collect royalties from You for the exercise of the Licensed
          Rights, whether directly or through a collecting society
          under any voluntary or waivable statutory or compulsory
          licensing scheme. In all other cases the Licensor expressly
          reserves any right to collect such royalties.


Section 3 -- License Conditions.

Your exercise of the Licensed Rights is expressly made subject to the
following conditions.

  a. Attribution.

       1. If You Share the Licensed Material, You must:

            a. retain the following if it is supplied by the Licensor
               with the Licensed Material:

                 i. identification of the creator(s) of the Licensed
                    Material and any others designated to receive
                    attribution, in any reasonable manner requested by
                    the Licensor (including by pseudonym if
                    designated);

                ii. a copyright notice;

               iii. a notice that refers to this Public License;

                iv. a notice that refers to the disclaimer of
                    warranties;

                 v. a URI or hyperlink to the Licensed Material to the
                    extent reasonably practicable;

            b. indicate if You modified the Licensed Material and
               retain an indication of any previous modifications; and

            c. indicate the Licensed Material is licensed under this
               Public License, and include the text of, or the URI or
               hyperlink to, this Public License.

          For the avoidance of doubt, You do not have permission under
          this Public License to Share Adapted Material.

       2. You may satisfy the conditions in Section 3(a)(1) in any
          reasonable manner based on the medium, means, and context in
          which You Share the Licensed Material. For example, it may be
          reasonable to satisfy the conditions by providing a URI or
          hyperlink to a resource that includes the required
          information.

       3. If requested by the Licensor, You must remove any of the
          information required by Section 3(a)(1)(A) to the extent
          reasonably practicable.


Section 4 -- Sui Generis Database Rights.

Where the Licensed Rights include Sui Generis Database Rights that
apply to Your use of the Licensed Material:

  a. for the avoidance of doubt, Section 2(a)(1) grants You the right
     to extract, reuse, reproduce, and Share all or a substantial
     portion of the contents of the database, provided You do not Share
     Adapted Material;
  b. if You include all or a substantial portion of the database
     contents in a database in which You have Sui Generis Database
     Rights, then the database in which You have Sui Generis Database
     Rights (but not its individual contents) is Adapted Material; and
  c. You must comply with the conditions in Section 3(a) if You Share
     all or a substantial portion of the contents of the database.

For the avoidance of doubt, this Section 4 supplements and does not
replace Your obligations under this Public License where the Licensed
Rights include other Copyright and Similar Rights.


Section 5 -- Disclaimer of Warranties and Limitation of Liability.

  a. UNLESS OTHERWISE SEPARATELY UNDERTAKEN BY THE LICENSOR, TO THE
     EXTENT POSSIBLE, THE LICENSOR OFFERS THE LICENSED MATERIAL AS-IS
     AND AS-AVAILABLE, AND MAKES NO REPRESENTATIONS OR WARRANTIES OF
     ANY KIND CONCERNING THE LICENSED MATERIAL, WHETHER EXPRESS,
     IMPLIED, STATUTORY, OR OTHER. THIS INCLUDES, WITHOUT LIMITATION,
     WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
     PURPOSE, NON-INFRINGEMENT, ABSENCE OF LATENT OR OTHER DEFECTS,
     ACCURACY, OR THE PRESENCE OR ABSENCE OF ERRORS, WHETHER OR NOT
     KNOWN OR DISCOVERABLE. WHERE DISCLAIMERS OF WARRANTIES ARE NOT
     ALLOWED IN FULL OR IN PART, THIS DISCLAIMER MAY NOT APPLY TO YOU.

  b. TO THE EXTENT POSSIBLE, IN NO EVENT WILL THE LICENSOR BE LIABLE
     TO YOU ON ANY LEGAL THEORY (INCLUDING, WITHOUT LIMITATION,
     NEGLIGENCE) OR OTHERWISE FOR ANY DIRECT, SPECIAL, INDIRECT,
     INCIDENTAL, CONSEQUENTIAL, PUNITIVE, EXEMPLARY, OR OTHER LOSSES,
     COSTS, EXPENSES, OR DAMAGES ARISING OUT OF THIS PUBLIC LICENSE OR
     USE OF THE LICENSED MATERIAL, EVEN IF THE LICENSOR HAS BEEN
     ADVISED OF THE POSSIBILITY OF SUCH LOSSES, COSTS, EXPENSES, OR
     DAMAGES. WHERE A LIMITATION OF LIABILITY IS NOT ALLOWED IN FULL OR
     IN PART, THIS LIMITATION MAY NOT APPLY TO YOU.

  c. The disclaimer of warranties and limitation of liability provided
     above shall be interpreted in a manner that, to the extent
     possible, most closely approximates an absolute disclaimer and
     waiver of all liability.


Section 6 -- Term and Termination.

  a. This Public License applies for the term of the Copyright and
     Similar Rights licensed here. However, if You fail to comply with
     this Public License, then Your rights under this Public License
     terminate automatically.

  b. Where Your right to use the Licensed Material has terminated under
     Section 6(a), it reinstates:

       1. automatically as of the date the violation is cured, provided
          it is cured within 30 days of Your discovery of the
          violation; or

       2. upon express reinstatement by the Licensor.

     For the avoidance of doubt, this Section 6(b) does not affect any
     right the Licensor may have to seek remedies for Your violations
     of this Public License.

  c. For the avoidance of doubt, the Licensor may also offer the
     Licensed Material under separate terms or conditions or stop
     distributing the Licensed Material at any time; however, doing so
     will not terminate this Public License.

  d. Sections 1, 5, 6, 7, and 8 survive termination of this Public
     License.


Section 7 -- Other Terms and Conditions.

  a. The Licensor shall not be bound by any additional or different
     terms or conditions communicated by You unless expressly agreed.

  b. Any arrangements, understandings, or agreements regarding the
     Licensed Material not stated herein are separate from and
     independent of the terms and conditions of this Public License.


Section 8 -- Interpretation.

  a. For the avoidance of doubt, this Public License does not, and
     shall not be interpreted to, reduce, limit, restrict, or impose
     conditions on any use of the Licensed Material that could lawfully
     be made without permission under this Public License.

  b. To the extent possible, if any provision of this Public License is
     deemed unenforceable, it shall be automatically reformed to the
     minimum extent necessary to make it enforceable. If the provision
     cannot be reformed, it shall be severed from this Public License
     without affecting the enforceability of the remaining terms and
     conditions.

  c. No term or condition of this Public License will be waived and no
     failure to comply consented to unless expressly agreed to by the
     Licensor.

  d. Nothing in this Public License constitutes or may be interpreted
     as a limitation upon, or waiver of, any privileges and immunities
     that apply to the Licensor or You, including from the legal
     processes of any jurisdiction or authority.

=======================================================================

Creative Commons is not a party to its public licenses.
Notwithstanding, Creative Commons may elect to apply one of its public
licenses to material it publishes and in those instances will be
considered the "Licensor." Except for the limited purpose of indicating
that material is shared under a Creative Commons public license or as
otherwise permitted by the Creative Commons policies published at
creativecommons.org/policies, Creative Commons does not authorize the
use of the trademark "Creative Commons" or any other trademark or logo
of Creative Commons without its prior written consent including,
without limitation, in connection with any unauthorized modifications
to any of its public licenses or any other arrangements,
understandings, or agreements concerning use of licensed material. For
the avoidance of doubt, this paragraph does not form part of the public
licenses.

Creative Commons may be contacted at creativecommons.org.


==> license-texts/doclicense-CC-by-sa-3.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-ShareAlike 3.0 Unported}





\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES
NOT PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE
DOES NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE
COMMONS PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS.
CREATIVE COMMONS MAKES NO WARRANTIES REGARDING THE
INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR DAMAGES
RESULTING FROM ITS USE.
\end{quotation}
\subsubsection{\emph{License}}
\par THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS
OF THIS CREATIVE COMMONS PUBLIC LICENSE (``CCPL'' OR
``LICENSE''). THE WORK IS PROTECTED BY COPYRIGHT AND/OR OTHER
APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS
PROHIBITED.
\par BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU
ACCEPT AND AGREE TO BE BOUND BY THE TERMS OF THIS LICENSE.
TO THE EXTENT THIS LICENSE MAY BE CONSIDERED TO BE A
CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS CONTAINED HERE
IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.
\par \textbf{1. Definitions}
\begin{enumerate}
\item \textbf{``Adaptation''} means a work based upon
the Work, or upon the Work and other pre-existing works,
such as a translation, adaptation, derivative work,
arrangement of music or other alterations of a literary
or artistic work, or phonogram or performance and
includes cinematographic adaptations or any other form in
which the Work may be recast, transformed, or adapted
including in any form recognizably derived from the
original, except that a work that constitutes a
Collection will not be considered an Adaptation for the
purpose of this License. For the avoidance of doubt,
where the Work is a musical work, performance or
phonogram, the synchronization of the Work in
timed-relation with a moving image (``synching'') will be
considered an Adaptation for the purpose of this
License.
\item \textbf{``Collection''} means a collection of
literary or artistic works, such as encyclopedias and
anthologies, or performances, phonograms or broadcasts,
or other works or subject matter other than works listed
in Section 1(f) below, which, by reason of the selection
and arrangement of their contents, constitute
intellectual creations, in which the Work is included in
its entirety in unmodified form along with one or more
other contributions, each constituting separate and
independent works in themselves, which together are
assembled into a collective whole. A work that
constitutes a Collection will not be considered an
Adaptation (as defined below) for the purposes of this
License.
\item \textbf{``Creative Commons Compatible
License''} means a license that is listed at
\url{https://creativecommons.org/compatiblelicenses} that has
been approved by Creative Commons as being essentially
equivalent to this License, including, at a minimum,
because that license: (i) contains terms that have the
same purpose, meaning and effect as the License Elements
of this License; and, (ii) explicitly permits the
relicensing of adaptations of works made available under
that license under this License or a Creative Commons
jurisdiction license with the same License Elements as
this License.
\item \textbf{``Distribute''} means to make available
to the public the original and copies of the Work or
Adaptation, as appropriate, through sale or other
transfer of ownership.
\item \textbf{``License Elements''} means the
following high-level license attributes as selected by
Licensor and indicated in the title of this License:
Attribution, ShareAlike.
\item \textbf{``Licensor''} means the individual,
individuals, entity or entities that offer(s) the Work
under the terms of this License.
\item \textbf{``Original Author''} means, in the case
of a literary or artistic work, the individual,
individuals, entity or entities who created the Work or
if no individual or entity can be identified, the
publisher; and in addition (i) in the case of a
performance the actors, singers, musicians, dancers, and
other persons who act, sing, deliver, declaim, play in,
interpret or otherwise perform literary or artistic works
or expressions of folklore; (ii) in the case of a
phonogram the producer being the person or legal entity
who first fixes the sounds of a performance or other
sounds; and, (iii) in the case of broadcasts, the
organization that transmits the broadcast.
\item \textbf{``Work''} means the literary and/or
artistic work offered under the terms of this License
including without limitation any production in the
literary, scientific and artistic domain, whatever may be
the mode or form of its expression including digital
form, such as a book, pamphlet and other writing; a
lecture, address, sermon or other work of the same
nature; a dramatic or dramatico-musical work; a
choreographic work or entertainment in dumb show; a
musical composition with or without words; a
cinematographic work to which are assimilated works
expressed by a process analogous to cinematography; a
work of drawing, painting, architecture, sculpture,
engraving or lithography; a photographic work to which
are assimilated works expressed by a process analogous to
photography; a work of applied art; an illustration, map,
plan, sketch or three-dimensional work relative to
geography, topography, architecture or science; a
performance; a broadcast; a phonogram; a compilation of
data to the extent it is protected as a copyrightable
work; or a work performed by a variety or circus
performer to the extent it is not otherwise considered a
literary or artistic work.
\item \textbf{``You''} means an individual or entity
exercising rights under this License who has not
previously violated the terms of this License with
respect to the Work, or who has received express
permission from the Licensor to exercise rights under
this License despite a previous violation.
\item \textbf{``Publicly Perform''} means to perform
public recitations of the Work and to communicate to the
public those public recitations, by any means or process,
including by wire or wireless means or public digital
performances; to make available to the public Works in
such a way that members of the public may access these
Works from a place and at a place individually chosen by
them; to perform the Work to the public by any means or
process and the communication to the public of the
performances of the Work, including by public digital
performance; to broadcast and rebroadcast the Work by any
means including signs, sounds or images.
\item \textbf{``Reproduce''} means to make copies of
the Work by any means including without limitation by
sound or visual recordings and the right of fixation and
reproducing fixations of the Work, including storage of a
protected performance or phonogram in digital form or
other electronic medium.
\end{enumerate}
\par \textbf{2. Fair Dealing Rights.} Nothing in this
License is intended to reduce, limit, or restrict any uses
free from copyright or rights arising from limitations or
exceptions that are provided for in connection with the
copyright protection under copyright law or other
applicable laws.
\par \textbf{3. License Grant.} Subject to the terms
and conditions of this License, Licensor hereby grants You
a worldwide, royalty-free, non-exclusive, perpetual (for
the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:
\begin{enumerate}
\item to Reproduce the Work, to incorporate the Work into
one or more Collections, and to Reproduce the Work as
incorporated in the Collections;
\item to create and Reproduce Adaptations provided that any
such Adaptation, including any translation in any medium,
takes reasonable steps to clearly label, demarcate or
otherwise identify that changes were made to the original
Work. For example, a translation could be marked ``The
original work was translated from English to Spanish,'' or
a modification could indicate ``The original work has been
modified.'';
\item to Distribute and Publicly Perform the Work including
as incorporated in Collections; and,
\item to Distribute and Publicly Perform Adaptations.
\item 
\par For the avoidance of doubt:
\begin{enumerate}
\item \textbf{Non-waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme cannot be waived, the
Licensor reserves the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License;
\item \textbf{Waivable Compulsory License
Schemes}. In those jurisdictions in which the
right to collect royalties through any statutory or
compulsory licensing scheme can be waived, the
Licensor waives the exclusive right to collect such
royalties for any exercise by You of the rights
granted under this License; and,
\item \textbf{Voluntary License Schemes}. The
Licensor waives the right to collect royalties,
whether individually or, in the event that the
Licensor is a member of a collecting society that
administers voluntary licensing schemes, via that
society, from any exercise by You of the rights
granted under this License.
\end{enumerate}

\end{enumerate}
\par The above rights may be exercised in all media and
formats whether now known or hereafter devised. The above
rights include the right to make such modifications as are
technically necessary to exercise the rights in other media
and formats. Subject to Section 8(f), all rights not
expressly granted by Licensor are hereby reserved.
\par \textbf{4. Restrictions.} The license granted in
Section 3 above is expressly made subject to and limited by
the following restrictions:
\begin{enumerate}
\item You may Distribute or Publicly Perform the Work only
under the terms of this License. You must include a copy
of, or the Uniform Resource Identifier (URI) for, this
License with every copy of the Work You Distribute or
Publicly Perform. You may not offer or impose any terms
on the Work that restrict the terms of this License or
the ability of the recipient of the Work to exercise the
rights granted to that recipient under the terms of the
License. You may not sublicense the Work. You must keep
intact all notices that refer to this License and to the
disclaimer of warranties with every copy of the Work You
Distribute or Publicly Perform. When You Distribute or
Publicly Perform the Work, You may not impose any
effective technological measures on the Work that
restrict the ability of a recipient of the Work from You
to exercise the rights granted to that recipient under
the terms of the License. This Section 4(a) applies to
the Work as incorporated in a Collection, but this does
not require the Collection apart from the Work itself to
be made subject to the terms of this License. If You
create a Collection, upon notice from any Licensor You
must, to the extent practicable, remove from the
Collection any credit as required by Section 4(c), as
requested. If You create an Adaptation, upon notice from
any Licensor You must, to the extent practicable, remove
from the Adaptation any credit as required by Section
4(c), as requested.
\item You may Distribute or Publicly Perform an Adaptation
only under the terms of: (i) this License; (ii) a later
version of this License with the same License Elements as
this License; (iii) a Creative Commons jurisdiction
license (either this or a later license version) that
contains the same License Elements as this License (e.g.,
Attribution-ShareAlike 3.0 US)); (iv) a Creative Commons
Compatible License. If you license the Adaptation under
one of the licenses mentioned in (iv), you must comply
with the terms of that license. If you license the
Adaptation under the terms of any of the licenses
mentioned in (i), (ii) or (iii) (the ``Applicable
License''), you must comply with the terms of the
Applicable License generally and the following
provisions: (I) You must include a copy of, or the URI
for, the Applicable License with every copy of each
Adaptation You Distribute or Publicly Perform; (II) You
may not offer or impose any terms on the Adaptation that
restrict the terms of the Applicable License or the
ability of the recipient of the Adaptation to exercise
the rights granted to that recipient under the terms of
the Applicable License; (III) You must keep intact all
notices that refer to the Applicable License and to the
disclaimer of warranties with every copy of the Work as
included in the Adaptation You Distribute or Publicly
Perform; (IV) when You Distribute or Publicly Perform the
Adaptation, You may not impose any effective
technological measures on the Adaptation that restrict
the ability of a recipient of the Adaptation from You to
exercise the rights granted to that recipient under the
terms of the Applicable License. This Section 4(b)
applies to the Adaptation as incorporated in a
Collection, but this does not require the Collection
apart from the Adaptation itself to be made subject to
the terms of the Applicable License.
\item If You Distribute, or Publicly Perform the Work or
any Adaptations or Collections, You must, unless a
request has been made pursuant to Section 4(a), keep
intact all copyright notices for the Work and provide,
reasonable to the medium or means You are utilizing: (i)
the name of the Original Author (or pseudonym, if
applicable) if supplied, and/or if the Original Author
and/or Licensor designate another party or parties (e.g.,
a sponsor institute, publishing entity, journal) for
attribution (``Attribution Parties'') in Licensor's
copyright notice, terms of service or by other reasonable
means, the name of such party or parties; (ii) the title
of the Work if supplied; (iii) to the extent reasonably
practicable, the URI, if any, that Licensor specifies to
be associated with the Work, unless such URI does not
refer to the copyright notice or licensing information
for the Work; and (iv) , consistent with Ssection 3(b),
in the case of an Adaptation, a credit identifying the
use of the Work in the Adaptation (e.g., ``French
translation of the Work by Original Author,'' or
``Screenplay based on original Work by Original Author'').
The credit required by this Section 4(c) may be
implemented in any reasonable manner; provided, however,
that in the case of a Adaptation or Collection, at a
minimum such credit will appear, if a credit for all
contributing authors of the Adaptation or Collection
appears, then as part of these credits and in a manner at
least as prominent as the credits for the other
contributing authors. For the avoidance of doubt, You may
only use the credit required by this Section for the
purpose of attribution in the manner set out above and,
by exercising Your rights under this License, You may not
implicitly or explicitly assert or imply any connection
with, sponsorship or endorsement by the Original Author,
Licensor and/or Attribution Parties, as appropriate, of
You or Your use of the Work, without the separate,
express prior written permission of the Original Author,
Licensor and/or Attribution Parties.
\item Except as otherwise agreed in writing by the Licensor
or as may be otherwise permitted by applicable law, if
You Reproduce, Distribute or Publicly Perform the Work
either by itself or as part of any Adaptations or
Collections, You must not distort, mutilate, modify or
take other derogatory action in relation to the Work
which would be prejudicial to the Original Author's honor
or reputation. Licensor agrees that in those
jurisdictions (e.g. Japan), in which any exercise of the
right granted in Section 3(b) of this License (the right
to make Adaptations) would be deemed to be a distortion,
mutilation, modification or other derogatory action
prejudicial to the Original Author's honor and
reputation, the Licensor will waive or not assert, as
appropriate, this Section, to the fullest extent
permitted by the applicable national law, to enable You
to reasonably exercise Your right under Section 3(b) of
this License (right to make Adaptations) but not
otherwise.
\end{enumerate}
\par \textbf{5. Representations, Warranties and
Disclaimer}
\par UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN
WRITING, LICENSOR OFFERS THE WORK AS-IS AND MAKES NO
REPRESENTATIONS OR WARRANTIES OF ANY KIND CONCERNING THE
WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE, INCLUDING,
WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE
ABSENCE OF LATENT OR OTHER DEFECTS, ACCURACY, OR THE
PRESENCE OF ABSENCE OF ERRORS, WHETHER OR NOT DISCOVERABLE.
SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION OF IMPLIED
WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.
\par \textbf{6. Limitation on Liability.} EXCEPT TO
THE EXTENT REQUIRED BY APPLICABLE LAW, IN NO EVENT WILL
LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR ANY
SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY
DAMAGES ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK,
EVEN IF LICENSOR HAS BEEN ADVISED OF THE POSSIBILITY OF
SUCH DAMAGES.
\par \textbf{7. Termination}
\begin{enumerate}
\item This License and the rights granted hereunder will
terminate automatically upon any breach by You of the
terms of this License. Individuals or entities who have
received Adaptations or Collections from You under this
License, however, will not have their licenses terminated
provided such individuals or entities remain in full
compliance with those licenses. Sections 1, 2, 5, 6, 7,
and 8 will survive any termination of this License.
\item Subject to the above terms and conditions, the
license granted here is perpetual (for the duration of
the applicable copyright in the Work). Notwithstanding
the above, Licensor reserves the right to release the
Work under different license terms or to stop
distributing the Work at any time; provided, however that
any such election will not serve to withdraw this License
(or any other license that has been, or is required to
be, granted under the terms of this License), and this
License will continue in full force and effect unless
terminated as stated above.
\end{enumerate}
\par \textbf{8. Miscellaneous}
\begin{enumerate}
\item Each time You Distribute or Publicly Perform the Work
or a Collection, the Licensor offers to the recipient a
license to the Work on the same terms and conditions as
the license granted to You under this License.
\item Each time You Distribute or Publicly Perform an
Adaptation, Licensor offers to the recipient a license to
the original Work on the same terms and conditions as the
license granted to You under this License.
\item If any provision of this License is invalid or
unenforceable under applicable law, it shall not affect
the validity or enforceability of the remainder of the
terms of this License, and without further action by the
parties to this agreement, such provision shall be
reformed to the minimum extent necessary to make such
provision valid and enforceable.
\item No term or provision of this License shall be deemed
waived and no breach consented to unless such waiver or
consent shall be in writing and signed by the party to be
charged with such waiver or consent.
\item This License constitutes the entire agreement between
the parties with respect to the Work licensed here. There
are no understandings, agreements or representations with
respect to the Work not specified here. Licensor shall
not be bound by any additional provisions that may appear
in any communication from You. This License may not be
modified without the mutual written agreement of the
Licensor and You.
\item The rights granted under, and the subject matter
referenced, in this License were drafted utilizing the
terminology of the Berne Convention for the Protection of
Literary and Artistic Works (as amended on September 28,
1979), the Rome Convention of 1961, the WIPO Copyright
Treaty of 1996, the WIPO Performances and Phonograms
Treaty of 1996 and the Universal Copyright Convention (as
revised on July 24, 1971). These rights and subject
matter take effect in the relevant jurisdiction in which
the License terms are sought to be enforced according to
the corresponding provisions of the implementation of
those treaty provisions in the applicable national law.
If the standard suite of rights granted under applicable
copyright law includes additional rights not granted
under this License, such additional rights are deemed to
be included in the License; this License is not intended
to restrict the license of any rights under applicable
law.
\end{enumerate}
 
\begin{quotation}
\subsubsection{Creative Commons Notice}
\par Creative Commons is not a party to this License, and
makes no warranty whatsoever in connection with the Work.
Creative Commons will not be liable to You or any party
on any legal theory for any damages whatsoever, including
without limitation any general, special, incidental or
consequential damages arising in connection to this
license. Notwithstanding the foregoing two (2) sentences,
if Creative Commons has expressly identified itself as
the Licensor hereunder, it shall have all rights and
obligations of Licensor.
\par Except for the limited purpose of indicating to the
public that the Work is licensed under the CCPL, Creative
Commons does not authorize the use by either party of the
trademark ``Creative Commons'' or any related trademark or
logo of Creative Commons without the prior written
consent of Creative Commons. Any permitted use will be in
compliance with Creative Commons' then-current trademark
usage guidelines, as may be published on its website or
otherwise made available upon request from time to time.
For the avoidance of doubt, this trademark restriction
does not form part of the License.
\par Creative Commons may be contacted at \url{https://creativecommons.org/}.
\end{quotation} 



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-sa-3.0-plaintext.tex <==
Creative Commons Legal Code

Attribution-ShareAlike 3.0 Unported

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS LICENSE DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE INFORMATION PROVIDED, AND DISCLAIMS LIABILITY FOR
    DAMAGES RESULTING FROM ITS USE.

License

THE WORK (AS DEFINED BELOW) IS PROVIDED UNDER THE TERMS OF THIS CREATIVE
COMMONS PUBLIC LICENSE ("CCPL" OR "LICENSE"). THE WORK IS PROTECTED BY
COPYRIGHT AND/OR OTHER APPLICABLE LAW. ANY USE OF THE WORK OTHER THAN AS
AUTHORIZED UNDER THIS LICENSE OR COPYRIGHT LAW IS PROHIBITED.

BY EXERCISING ANY RIGHTS TO THE WORK PROVIDED HERE, YOU ACCEPT AND AGREE
TO BE BOUND BY THE TERMS OF THIS LICENSE. TO THE EXTENT THIS LICENSE MAY
BE CONSIDERED TO BE A CONTRACT, THE LICENSOR GRANTS YOU THE RIGHTS
CONTAINED HERE IN CONSIDERATION OF YOUR ACCEPTANCE OF SUCH TERMS AND
CONDITIONS.

1. Definitions

 a. "Adaptation" means a work based upon the Work, or upon the Work and
    other pre-existing works, such as a translation, adaptation,
    derivative work, arrangement of music or other alterations of a
    literary or artistic work, or phonogram or performance and includes
    cinematographic adaptations or any other form in which the Work may be
    recast, transformed, or adapted including in any form recognizably
    derived from the original, except that a work that constitutes a
    Collection will not be considered an Adaptation for the purpose of
    this License. For the avoidance of doubt, where the Work is a musical
    work, performance or phonogram, the synchronization of the Work in
    timed-relation with a moving image ("synching") will be considered an
    Adaptation for the purpose of this License.
 b. "Collection" means a collection of literary or artistic works, such as
    encyclopedias and anthologies, or performances, phonograms or
    broadcasts, or other works or subject matter other than works listed
    in Section 1(f) below, which, by reason of the selection and
    arrangement of their contents, constitute intellectual creations, in
    which the Work is included in its entirety in unmodified form along
    with one or more other contributions, each constituting separate and
    independent works in themselves, which together are assembled into a
    collective whole. A work that constitutes a Collection will not be
    considered an Adaptation (as defined below) for the purposes of this
    License.
 c. "Creative Commons Compatible License" means a license that is listed
    at https://creativecommons.org/compatiblelicenses that has been
    approved by Creative Commons as being essentially equivalent to this
    License, including, at a minimum, because that license: (i) contains
    terms that have the same purpose, meaning and effect as the License
    Elements of this License; and, (ii) explicitly permits the relicensing
    of adaptations of works made available under that license under this
    License or a Creative Commons jurisdiction license with the same
    License Elements as this License.
 d. "Distribute" means to make available to the public the original and
    copies of the Work or Adaptation, as appropriate, through sale or
    other transfer of ownership.
 e. "License Elements" means the following high-level license attributes
    as selected by Licensor and indicated in the title of this License:
    Attribution, ShareAlike.
 f. "Licensor" means the individual, individuals, entity or entities that
    offer(s) the Work under the terms of this License.
 g. "Original Author" means, in the case of a literary or artistic work,
    the individual, individuals, entity or entities who created the Work
    or if no individual or entity can be identified, the publisher; and in
    addition (i) in the case of a performance the actors, singers,
    musicians, dancers, and other persons who act, sing, deliver, declaim,
    play in, interpret or otherwise perform literary or artistic works or
    expressions of folklore; (ii) in the case of a phonogram the producer
    being the person or legal entity who first fixes the sounds of a
    performance or other sounds; and, (iii) in the case of broadcasts, the
    organization that transmits the broadcast.
 h. "Work" means the literary and/or artistic work offered under the terms
    of this License including without limitation any production in the
    literary, scientific and artistic domain, whatever may be the mode or
    form of its expression including digital form, such as a book,
    pamphlet and other writing; a lecture, address, sermon or other work
    of the same nature; a dramatic or dramatico-musical work; a
    choreographic work or entertainment in dumb show; a musical
    composition with or without words; a cinematographic work to which are
    assimilated works expressed by a process analogous to cinematography;
    a work of drawing, painting, architecture, sculpture, engraving or
    lithography; a photographic work to which are assimilated works
    expressed by a process analogous to photography; a work of applied
    art; an illustration, map, plan, sketch or three-dimensional work
    relative to geography, topography, architecture or science; a
    performance; a broadcast; a phonogram; a compilation of data to the
    extent it is protected as a copyrightable work; or a work performed by
    a variety or circus performer to the extent it is not otherwise
    considered a literary or artistic work.
 i. "You" means an individual or entity exercising rights under this
    License who has not previously violated the terms of this License with
    respect to the Work, or who has received express permission from the
    Licensor to exercise rights under this License despite a previous
    violation.
 j. "Publicly Perform" means to perform public recitations of the Work and
    to communicate to the public those public recitations, by any means or
    process, including by wire or wireless means or public digital
    performances; to make available to the public Works in such a way that
    members of the public may access these Works from a place and at a
    place individually chosen by them; to perform the Work to the public
    by any means or process and the communication to the public of the
    performances of the Work, including by public digital performance; to
    broadcast and rebroadcast the Work by any means including signs,
    sounds or images.
 k. "Reproduce" means to make copies of the Work by any means including
    without limitation by sound or visual recordings and the right of
    fixation and reproducing fixations of the Work, including storage of a
    protected performance or phonogram in digital form or other electronic
    medium.

2. Fair Dealing Rights. Nothing in this License is intended to reduce,
limit, or restrict any uses free from copyright or rights arising from
limitations or exceptions that are provided for in connection with the
copyright protection under copyright law or other applicable laws.

3. License Grant. Subject to the terms and conditions of this License,
Licensor hereby grants You a worldwide, royalty-free, non-exclusive,
perpetual (for the duration of the applicable copyright) license to
exercise the rights in the Work as stated below:

 a. to Reproduce the Work, to incorporate the Work into one or more
    Collections, and to Reproduce the Work as incorporated in the
    Collections;
 b. to create and Reproduce Adaptations provided that any such Adaptation,
    including any translation in any medium, takes reasonable steps to
    clearly label, demarcate or otherwise identify that changes were made
    to the original Work. For example, a translation could be marked "The
    original work was translated from English to Spanish," or a
    modification could indicate "The original work has been modified.";
 c. to Distribute and Publicly Perform the Work including as incorporated
    in Collections; and,
 d. to Distribute and Publicly Perform Adaptations.
 e. For the avoidance of doubt:

     i. Non-waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme cannot be waived, the Licensor
        reserves the exclusive right to collect such royalties for any
        exercise by You of the rights granted under this License;
    ii. Waivable Compulsory License Schemes. In those jurisdictions in
        which the right to collect royalties through any statutory or
        compulsory licensing scheme can be waived, the Licensor waives the
        exclusive right to collect such royalties for any exercise by You
        of the rights granted under this License; and,
   iii. Voluntary License Schemes. The Licensor waives the right to
        collect royalties, whether individually or, in the event that the
        Licensor is a member of a collecting society that administers
        voluntary licensing schemes, via that society, from any exercise
        by You of the rights granted under this License.

The above rights may be exercised in all media and formats whether now
known or hereafter devised. The above rights include the right to make
such modifications as are technically necessary to exercise the rights in
other media and formats. Subject to Section 8(f), all rights not expressly
granted by Licensor are hereby reserved.

4. Restrictions. The license granted in Section 3 above is expressly made
subject to and limited by the following restrictions:

 a. You may Distribute or Publicly Perform the Work only under the terms
    of this License. You must include a copy of, or the Uniform Resource
    Identifier (URI) for, this License with every copy of the Work You
    Distribute or Publicly Perform. You may not offer or impose any terms
    on the Work that restrict the terms of this License or the ability of
    the recipient of the Work to exercise the rights granted to that
    recipient under the terms of the License. You may not sublicense the
    Work. You must keep intact all notices that refer to this License and
    to the disclaimer of warranties with every copy of the Work You
    Distribute or Publicly Perform. When You Distribute or Publicly
    Perform the Work, You may not impose any effective technological
    measures on the Work that restrict the ability of a recipient of the
    Work from You to exercise the rights granted to that recipient under
    the terms of the License. This Section 4(a) applies to the Work as
    incorporated in a Collection, but this does not require the Collection
    apart from the Work itself to be made subject to the terms of this
    License. If You create a Collection, upon notice from any Licensor You
    must, to the extent practicable, remove from the Collection any credit
    as required by Section 4(c), as requested. If You create an
    Adaptation, upon notice from any Licensor You must, to the extent
    practicable, remove from the Adaptation any credit as required by
    Section 4(c), as requested.
 b. You may Distribute or Publicly Perform an Adaptation only under the
    terms of: (i) this License; (ii) a later version of this License with
    the same License Elements as this License; (iii) a Creative Commons
    jurisdiction license (either this or a later license version) that
    contains the same License Elements as this License (e.g.,
    Attribution-ShareAlike 3.0 US)); (iv) a Creative Commons Compatible
    License. If you license the Adaptation under one of the licenses
    mentioned in (iv), you must comply with the terms of that license. If
    you license the Adaptation under the terms of any of the licenses
    mentioned in (i), (ii) or (iii) (the "Applicable License"), you must
    comply with the terms of the Applicable License generally and the
    following provisions: (I) You must include a copy of, or the URI for,
    the Applicable License with every copy of each Adaptation You
    Distribute or Publicly Perform; (II) You may not offer or impose any
    terms on the Adaptation that restrict the terms of the Applicable
    License or the ability of the recipient of the Adaptation to exercise
    the rights granted to that recipient under the terms of the Applicable
    License; (III) You must keep intact all notices that refer to the
    Applicable License and to the disclaimer of warranties with every copy
    of the Work as included in the Adaptation You Distribute or Publicly
    Perform; (IV) when You Distribute or Publicly Perform the Adaptation,
    You may not impose any effective technological measures on the
    Adaptation that restrict the ability of a recipient of the Adaptation
    from You to exercise the rights granted to that recipient under the
    terms of the Applicable License. This Section 4(b) applies to the
    Adaptation as incorporated in a Collection, but this does not require
    the Collection apart from the Adaptation itself to be made subject to
    the terms of the Applicable License.
 c. If You Distribute, or Publicly Perform the Work or any Adaptations or
    Collections, You must, unless a request has been made pursuant to
    Section 4(a), keep intact all copyright notices for the Work and
    provide, reasonable to the medium or means You are utilizing: (i) the
    name of the Original Author (or pseudonym, if applicable) if supplied,
    and/or if the Original Author and/or Licensor designate another party
    or parties (e.g., a sponsor institute, publishing entity, journal) for
    attribution ("Attribution Parties") in Licensor's copyright notice,
    terms of service or by other reasonable means, the name of such party
    or parties; (ii) the title of the Work if supplied; (iii) to the
    extent reasonably practicable, the URI, if any, that Licensor
    specifies to be associated with the Work, unless such URI does not
    refer to the copyright notice or licensing information for the Work;
    and (iv) , consistent with Ssection 3(b), in the case of an
    Adaptation, a credit identifying the use of the Work in the Adaptation
    (e.g., "French translation of the Work by Original Author," or
    "Screenplay based on original Work by Original Author"). The credit
    required by this Section 4(c) may be implemented in any reasonable
    manner; provided, however, that in the case of a Adaptation or
    Collection, at a minimum such credit will appear, if a credit for all
    contributing authors of the Adaptation or Collection appears, then as
    part of these credits and in a manner at least as prominent as the
    credits for the other contributing authors. For the avoidance of
    doubt, You may only use the credit required by this Section for the
    purpose of attribution in the manner set out above and, by exercising
    Your rights under this License, You may not implicitly or explicitly
    assert or imply any connection with, sponsorship or endorsement by the
    Original Author, Licensor and/or Attribution Parties, as appropriate,
    of You or Your use of the Work, without the separate, express prior
    written permission of the Original Author, Licensor and/or Attribution
    Parties.
 d. Except as otherwise agreed in writing by the Licensor or as may be
    otherwise permitted by applicable law, if You Reproduce, Distribute or
    Publicly Perform the Work either by itself or as part of any
    Adaptations or Collections, You must not distort, mutilate, modify or
    take other derogatory action in relation to the Work which would be
    prejudicial to the Original Author's honor or reputation. Licensor
    agrees that in those jurisdictions (e.g. Japan), in which any exercise
    of the right granted in Section 3(b) of this License (the right to
    make Adaptations) would be deemed to be a distortion, mutilation,
    modification or other derogatory action prejudicial to the Original
    Author's honor and reputation, the Licensor will waive or not assert,
    as appropriate, this Section, to the fullest extent permitted by the
    applicable national law, to enable You to reasonably exercise Your
    right under Section 3(b) of this License (right to make Adaptations)
    but not otherwise.

5. Representations, Warranties and Disclaimer

UNLESS OTHERWISE MUTUALLY AGREED TO BY THE PARTIES IN WRITING, LICENSOR
OFFERS THE WORK AS-IS AND MAKES NO REPRESENTATIONS OR WARRANTIES OF ANY
KIND CONCERNING THE WORK, EXPRESS, IMPLIED, STATUTORY OR OTHERWISE,
INCLUDING, WITHOUT LIMITATION, WARRANTIES OF TITLE, MERCHANTIBILITY,
FITNESS FOR A PARTICULAR PURPOSE, NONINFRINGEMENT, OR THE ABSENCE OF
LATENT OR OTHER DEFECTS, ACCURACY, OR THE PRESENCE OF ABSENCE OF ERRORS,
WHETHER OR NOT DISCOVERABLE. SOME JURISDICTIONS DO NOT ALLOW THE EXCLUSION
OF IMPLIED WARRANTIES, SO SUCH EXCLUSION MAY NOT APPLY TO YOU.

6. Limitation on Liability. EXCEPT TO THE EXTENT REQUIRED BY APPLICABLE
LAW, IN NO EVENT WILL LICENSOR BE LIABLE TO YOU ON ANY LEGAL THEORY FOR
ANY SPECIAL, INCIDENTAL, CONSEQUENTIAL, PUNITIVE OR EXEMPLARY DAMAGES
ARISING OUT OF THIS LICENSE OR THE USE OF THE WORK, EVEN IF LICENSOR HAS
BEEN ADVISED OF THE POSSIBILITY OF SUCH DAMAGES.

7. Termination

 a. This License and the rights granted hereunder will terminate
    automatically upon any breach by You of the terms of this License.
    Individuals or entities who have received Adaptations or Collections
    from You under this License, however, will not have their licenses
    terminated provided such individuals or entities remain in full
    compliance with those licenses. Sections 1, 2, 5, 6, 7, and 8 will
    survive any termination of this License.
 b. Subject to the above terms and conditions, the license granted here is
    perpetual (for the duration of the applicable copyright in the Work).
    Notwithstanding the above, Licensor reserves the right to release the
    Work under different license terms or to stop distributing the Work at
    any time; provided, however that any such election will not serve to
    withdraw this License (or any other license that has been, or is
    required to be, granted under the terms of this License), and this
    License will continue in full force and effect unless terminated as
    stated above.

8. Miscellaneous

 a. Each time You Distribute or Publicly Perform the Work or a Collection,
    the Licensor offers to the recipient a license to the Work on the same
    terms and conditions as the license granted to You under this License.
 b. Each time You Distribute or Publicly Perform an Adaptation, Licensor
    offers to the recipient a license to the original Work on the same
    terms and conditions as the license granted to You under this License.
 c. If any provision of this License is invalid or unenforceable under
    applicable law, it shall not affect the validity or enforceability of
    the remainder of the terms of this License, and without further action
    by the parties to this agreement, such provision shall be reformed to
    the minimum extent necessary to make such provision valid and
    enforceable.
 d. No term or provision of this License shall be deemed waived and no
    breach consented to unless such waiver or consent shall be in writing
    and signed by the party to be charged with such waiver or consent.
 e. This License constitutes the entire agreement between the parties with
    respect to the Work licensed here. There are no understandings,
    agreements or representations with respect to the Work not specified
    here. Licensor shall not be bound by any additional provisions that
    may appear in any communication from You. This License may not be
    modified without the mutual written agreement of the Licensor and You.
 f. The rights granted under, and the subject matter referenced, in this
    License were drafted utilizing the terminology of the Berne Convention
    for the Protection of Literary and Artistic Works (as amended on
    September 28, 1979), the Rome Convention of 1961, the WIPO Copyright
    Treaty of 1996, the WIPO Performances and Phonograms Treaty of 1996
    and the Universal Copyright Convention (as revised on July 24, 1971).
    These rights and subject matter take effect in the relevant
    jurisdiction in which the License terms are sought to be enforced
    according to the corresponding provisions of the implementation of
    those treaty provisions in the applicable national law. If the
    standard suite of rights granted under applicable copyright law
    includes additional rights not granted under this License, such
    additional rights are deemed to be included in the License; this
    License is not intended to restrict the license of any rights under
    applicable law.


Creative Commons Notice

    Creative Commons is not a party to this License, and makes no warranty
    whatsoever in connection with the Work. Creative Commons will not be
    liable to You or any party on any legal theory for any damages
    whatsoever, including without limitation any general, special,
    incidental or consequential damages arising in connection to this
    license. Notwithstanding the foregoing two (2) sentences, if Creative
    Commons has expressly identified itself as the Licensor hereunder, it
    shall have all rights and obligations of Licensor.

    Except for the limited purpose of indicating to the public that the
    Work is licensed under the CCPL, Creative Commons does not authorize
    the use by either party of the trademark "Creative Commons" or any
    related trademark or logo of Creative Commons without the prior
    written consent of Creative Commons. Any permitted use will be in
    compliance with Creative Commons' then-current trademark usage
    guidelines, as may be published on its website or otherwise made
    available upon request from time to time. For the avoidance of doubt,
    this trademark restriction does not form part of the License.

    Creative Commons may be contacted at https://creativecommons.org/.


==> license-texts/doclicense-CC-by-sa-4.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{Attribution-ShareAlike 4.0 International}







Official translations of this license are available in other languages.



\par Creative Commons Corporation (“Creative Commons”) is not a law firm and does not provide legal services or legal advice. Distribution of Creative Commons public licenses does not create a lawyer-client or other relationship. Creative Commons makes its licenses and related information available on an “as-is” basis. Creative Commons gives no warranties regarding its licenses, any material licensed under their terms and conditions, or any related information. Creative Commons disclaims all liability for damages resulting from their use to the fullest extent possible.


\par \textbf{Using Creative Commons Public Licenses}
\par Creative Commons public licenses provide a standard set of terms and conditions that creators and other rights holders may use to share original works of authorship and other material subject to copyright and certain other rights specified in the public license below. The following considerations are for informational purposes only, are not exhaustive, and do not form part of our licenses.
\begin{quotation}\textbf{Considerations for licensors:} Our public licenses are intended for use by those authorized to give the public permission to use material in ways otherwise restricted by copyright and certain other rights. Our licenses are irrevocable. Licensors should read and understand the terms and conditions of the license they choose before applying it. Licensors should also secure all rights necessary before applying our licenses so that the public can reuse the material as expected. Licensors should clearly mark any material not subject to the license. This includes other CC-licensed material, or material used under an exception or limitation to copyright. More considerations for licensors.\end{quotation}
\begin{quotation}\textbf{Considerations for the public:} By using one of our public licenses, a licensor grants the public permission to use the licensed material under specified terms and conditions. If the licensor’s permission is not necessary for any reason–for example, because of any applicable exception or limitation to copyright–then that use is not regulated by the license. Our licenses grant only permissions under copyright and certain other rights that a licensor has authority to grant. Use of the licensed material may still be restricted for other reasons, including because others have copyright or other rights in the material. A licensor may make special requests, such as asking that all changes be marked or described. Although not required by our licenses, you are encouraged to respect those requests where reasonable.
More considerations for the public.\end{quotation}

\subsubsection{Creative Commons Attribution-ShareAlike 4.0 International Public License}
\par By exercising the Licensed Rights (defined below), You accept and agree to be bound by the terms and conditions of this Creative Commons Attribution-ShareAlike 4.0 International Public License (``Public License''). To the extent this Public License may be interpreted as a contract, You are granted the Licensed Rights in consideration of Your acceptance of these terms and conditions, and the Licensor grants You such rights in consideration of benefits the Licensor receives from making the Licensed Material available under these terms and conditions.
\par \textbf{Section 1 – Definitions.}
\begin{enumerate}
\item \textbf{Adapted Material} means material subject to Copyright and Similar Rights that is derived from or based upon the Licensed Material and in which the Licensed Material is translated, altered, arranged, transformed, or otherwise modified in a manner requiring permission under the Copyright and Similar Rights held by the Licensor. For purposes of this Public License, where the Licensed Material is a musical work, performance, or sound recording, Adapted Material is always produced where the Licensed Material is synched in timed relation with a moving image.
\item \textbf{Adapter's License} means the license You apply to Your Copyright and Similar Rights in Your contributions to Adapted Material in accordance with the terms and conditions of this Public License.
\item \textbf{BY-SA Compatible License} means a license listed at  creativecommons.org/compatiblelicenses, approved by Creative Commons as essentially the equivalent of this Public License.
\item \textbf{Copyright and Similar Rights} means copyright and/or similar rights closely related to copyright including, without limitation, performance, broadcast, sound recording, and Sui Generis Database Rights, without regard to how the rights are labeled or categorized. For purposes of this Public License, the rights specified in Section 2(b)(1)-(2) are not Copyright and Similar Rights.
\item \textbf{Effective Technological Measures} means those measures that, in the absence of proper authority, may not
be circumvented under laws fulfilling obligations under Article 11 of the WIPO Copyright Treaty adopted on December 20, 1996, and/or similar
international agreements.
\item \textbf{Exceptions and Limitations} means fair use, fair dealing, and/or any other exception or limitation to Copyright and Similar Rights that applies to Your use of the Licensed Material.
\item \textbf{License Elements} means the license attributes listed in the name of a Creative Commons Public License. The License Elements of this Public License are Attribution and ShareAlike.
\item \textbf{Licensed Material} means the artistic or literary work, database, or other material to which the Licensor applied this Public License.
\item \textbf{Licensed Rights} means the rights granted to You subject to the terms and conditions of this Public License, which are limited to all Copyright and Similar Rights that apply to Your use of the Licensed Material and that the Licensor has authority to license.
\item \textbf{Licensor} means the individual(s) or entity(ies) granting rights under this Public License.
\item \textbf{Share} means to provide material to the public by any means or process that requires permission under the Licensed Rights, such as reproduction, public display, public performance, distribution, dissemination, communication, or importation, and to make material available to the public including in ways that members of the public may access the material from a place and at a time individually chosen by them.
\item \textbf{Sui Generis Database Rights} means rights other than copyright resulting from Directive 96/9/EC of the European Parliament and of the Council of 11 March 1996 on the legal protection of databases, as amended and/or succeeded, as well as other essentially equivalent rights anywhere in the world.
\item \textbf{You} means the individual or entity exercising the Licensed Rights under this Public License. \textbf{Your} has a corresponding meaning.
\end{enumerate}
\par \textbf{Section 2 – Scope.}
\begin{enumerate}
\item \textbf{License grant}.
\begin{enumerate}
\item Subject to the terms and conditions of this Public License, the Licensor hereby grants You a worldwide, royalty-free, non-sublicensable, non-exclusive, irrevocable license to exercise the Licensed Rights in the Licensed Material to:
\begin{enumerate}
\item reproduce and Share the Licensed Material, in whole or in part; and
\item produce, reproduce, and Share Adapted Material.
\end{enumerate}
\item Exceptions and Limitations. For the avoidance of doubt, where Exceptions and Limitations apply to Your use, this Public License does not apply, and You do not need to comply with its terms and conditions.
\item Term. The term of this Public License is specified in Section 6(a).
\item Media and formats; technical modifications allowed. The Licensor authorizes You to exercise the Licensed Rights in all media and formats whether now known or hereafter created, and to make technical modifications necessary to do so. The Licensor waives and/or agrees not to assert any right or authority to forbid You from making technical modifications necessary to exercise the Licensed Rights, including technical modifications necessary to circumvent Effective Technological Measures. For purposes of this Public License, simply making modifications authorized by this Section 2(a)(4) never produces Adapted Material.
\item Downstream recipients.

\begin{enumerate}
\item Offer from the Licensor – Licensed Material. Every recipient of the Licensed Material automatically receives an offer from the Licensor to exercise the Licensed Rights under the terms and conditions of this Public License.
\item Additional offer from the Licensor – Adapted Material. Every recipient of Adapted Material from You automatically receives an offer from the Licensor to exercise the Licensed Rights in the Adapted Material under the conditions of the Adapter’s License You apply.
\item No downstream restrictions. You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, the Licensed Material if doing so restricts exercise of the Licensed Rights by any recipient of the Licensed Material.
\end{enumerate}

\item No endorsement. Nothing in this Public License constitutes or may be construed as permission to assert or imply that You are, or that Your use of the Licensed Material is, connected with, or sponsored, endorsed, or granted official status by, the Licensor or others designated to receive attribution as provided in Section 3(a)(1)(A)(i).
\end{enumerate}
\item \par \textbf{Other rights}.
\begin{enumerate}
\item Moral rights, such as the right of integrity, are not licensed under this Public License, nor are publicity, privacy, and/or other similar personality rights; however, to the extent possible, the Licensor waives and/or agrees not to assert any such rights held by the Licensor to the limited extent necessary to allow You to exercise the Licensed Rights, but not otherwise.
\item Patent and trademark rights are not licensed under this Public License.
\item To the extent possible, the Licensor waives any right to collect royalties from You for the exercise of the Licensed Rights, whether directly or through a collecting society under any voluntary or waivable statutory or compulsory licensing scheme. In all other cases the Licensor expressly reserves any right to collect such royalties.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 3 – License Conditions.}
\par Your exercise of the Licensed Rights is expressly made subject to the following conditions.
\begin{enumerate}
\item \par \textbf{Attribution}.
\begin{enumerate}
\item \par If You Share the Licensed Material (including in modified form), You must:
\begin{enumerate}
\item retain the following if it is supplied by the Licensor with the Licensed Material:
\begin{enumerate}
\item identification of the creator(s) of the Licensed Material and any others designated to receive attribution, in any reasonable manner requested by the Licensor (including by pseudonym if designated);
\item a copyright notice;
\item a notice that refers to this Public License; 
\item a notice that refers to the disclaimer of warranties;
\item a URI or hyperlink to the Licensed Material to the extent reasonably practicable;
\end{enumerate}
\item indicate if You modified the Licensed Material and retain an indication of any previous modifications; and
\item indicate the Licensed Material is licensed under this Public License,
and include the text of, or the URI or hyperlink to, this Public
License.
\end{enumerate}

\item You may satisfy the conditions in Section 3(a)(1) in any reasonable manner based on the medium, means, and context in which You Share the Licensed Material. For example, it may be reasonable to satisfy the conditions by providing a URI or hyperlink to a resource that includes the required information.
\item If requested by the Licensor, You must remove any of the information required by Section 3(a)(1)(A) to the extent reasonably practicable.
\end{enumerate}

\item \textbf{ShareAlike}.
\par In addition to the conditions in Section 3(a), if You Share Adapted Material You produce, the following conditions also apply.
\begin{enumerate}
\item The Adapter’s License You apply must be a Creative Commons license with the same License Elements, this version or later, or a BY-SA Compatible License.
\item You must include the text of, or the URI or hyperlink to, the Adapter's License You apply. You may satisfy this condition in any reasonable manner based on the medium, means, and context in which You Share Adapted Material.
\item You may not offer or impose any additional or different terms or conditions on, or apply any Effective Technological Measures to, Adapted Material that restrict exercise of the rights granted under the Adapter's License You apply.
\end{enumerate}

\end{enumerate}
\par \textbf{Section 4 – Sui Generis Database Rights.}
\par Where the Licensed Rights include Sui Generis Database Rights that apply to Your use of the Licensed Material:
\begin{enumerate}
\item for the avoidance of doubt, Section 2(a)(1) grants You the right to extract, reuse, reproduce, and Share all or a substantial portion of the contents of the database;
\item if You include all or a substantial portion of the database contents in a database in which You have Sui Generis Database Rights, then the database in which You have Sui Generis Database Rights (but not its individual contents) is Adapted Material, including for purposes of Section 3(b); and
\item You must comply with the conditions in Section 3(a) if You Share all or a substantial portion of the contents of the database.
\end{enumerate}
For the avoidance of doubt, this Section 4 supplements and does not replace Your obligations under this Public License where the Licensed Rights include other Copyright and Similar Rights.
\par \textbf{Section 5 – Disclaimer of Warranties and Limitation of Liability.}
\begin{enumerate}
\item \textbf{Unless otherwise separately undertaken by the Licensor, to the extent possible, the Licensor offers the Licensed Material as-is and as-available, and makes no representations or warranties of any kind concerning the Licensed Material, whether express, implied, statutory, or other. This includes, without limitation, warranties of title, merchantability, fitness for a particular purpose, non-infringement, absence of latent or other defects, accuracy, or the presence or absence of errors, whether or not known or discoverable. Where disclaimers of warranties are not allowed in full or in part, this disclaimer may not apply to You.}
\item \textbf{To the extent possible, in no event will the Licensor be liable to You on any legal theory (including, without limitation, negligence) or otherwise for any direct, special, indirect, incidental, consequential, punitive, exemplary, or other losses, costs, expenses, or damages arising out of this Public License or use of the Licensed Material, even if the Licensor has been advised of the possibility of such losses, costs, expenses, or damages. Where a limitation of liability is not allowed in full or in part, this limitation may not apply to You.}
\end{enumerate}
\begin{enumerate}
\item The disclaimer of warranties and limitation of liability provided above shall be interpreted in a manner that, to the extent possible, most closely approximates an absolute disclaimer and waiver of all liability.
\end{enumerate}
\par \textbf{Section 6 – Term and Termination.}
\begin{enumerate}
\item This Public License applies for the term of the Copyright and Similar Rights licensed here. However, if You fail to comply with this Public License, then Your rights under this Public License terminate automatically.
\item 
\par Where Your right to use the Licensed Material has terminated under Section 6(a), it reinstates:
\begin{enumerate}
\item automatically as of the date the violation is cured, provided it is cured within 30 days of Your discovery of the violation; or
\item upon express reinstatement by the Licensor.
\end{enumerate}
For the avoidance of doubt, this Section 6(b) does not affect any right the Licensor may have to seek remedies for Your violations of this Public License.
\item For the avoidance of doubt, the Licensor may also offer the Licensed Material under separate terms or conditions or stop distributing the Licensed Material at any time; however, doing so will not terminate this Public License.
\item Sections 1, 5, 6, 7, and 8 survive termination of this Public License.
\end{enumerate}
\par \textbf{Section 7 – Other Terms and Conditions.}
\begin{enumerate}
\item The Licensor shall not be bound by any additional or different terms or conditions communicated by You unless expressly agreed.
\item Any arrangements, understandings, or agreements regarding the Licensed Material not stated herein are separate from and independent of the terms and conditions of this Public License.
\end{enumerate}
\par \textbf{Section 8 – Interpretation.}
\begin{enumerate}
\item For the avoidance of doubt, this Public License does not, and shall not be interpreted to, reduce, limit, restrict, or impose conditions on any use of the Licensed Material that could lawfully be made without permission under this Public License.
\item To the extent possible, if any provision of this Public License is deemed unenforceable, it shall be automatically reformed to the minimum extent necessary to make it enforceable. If the provision cannot be reformed, it shall be severed from this Public License without affecting the enforceability of the remaining terms and conditions.
\item No term or condition of this Public License will be waived and no failure to comply consented to unless expressly agreed to by the Licensor.
\item Nothing in this Public License constitutes or may be interpreted as a limitation upon, or waiver of, any privileges and immunities that apply to the Licensor or You, including from the legal processes of any jurisdiction or authority.
\end{enumerate}
\par Creative Commons is not a party to its public licenses. Notwithstanding, Creative Commons may elect to apply one of its public licenses to material it publishes and in those instances will be considered the “Licensor.” The text of the Creative Commons public licenses is dedicated to the public domain under the CC0 Public Domain Dedication. Except for the limited purpose of indicating that material is shared under a Creative Commons public license or as otherwise permitted by the Creative Commons policies published at creativecommons.org/policies, Creative Commons does not authorize the use of the trademark “Creative Commons” or any other trademark or logo of Creative Commons without its prior written consent including, without limitation, in connection with any unauthorized modifications to any of its public licenses or any other arrangements, understandings, or agreements concerning use of licensed material. For the avoidance of doubt, this paragraph does not form part of the public licenses.\\\\
Creative Commons may be contacted at creativecommons.org.
\par Additional languages available: Bahasa Indonesia, Nederlands, norsk, suomeksi, te reo Māori, українська, 日本語. Please read the FAQ for more information about official translations. 


\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-by-sa-4.0-plaintext.tex <==
Attribution-ShareAlike 4.0 International

=======================================================================

Creative Commons Corporation ("Creative Commons") is not a law firm and
does not provide legal services or legal advice. Distribution of
Creative Commons public licenses does not create a lawyer-client or
other relationship. Creative Commons makes its licenses and related
information available on an "as-is" basis. Creative Commons gives no
warranties regarding its licenses, any material licensed under their
terms and conditions, or any related information. Creative Commons
disclaims all liability for damages resulting from their use to the
fullest extent possible.

Using Creative Commons Public Licenses

Creative Commons public licenses provide a standard set of terms and
conditions that creators and other rights holders may use to share
original works of authorship and other material subject to copyright
and certain other rights specified in the public license below. The
following considerations are for informational purposes only, are not
exhaustive, and do not form part of our licenses.

     Considerations for licensors: Our public licenses are
     intended for use by those authorized to give the public
     permission to use material in ways otherwise restricted by
     copyright and certain other rights. Our licenses are
     irrevocable. Licensors should read and understand the terms
     and conditions of the license they choose before applying it.
     Licensors should also secure all rights necessary before
     applying our licenses so that the public can reuse the
     material as expected. Licensors should clearly mark any
     material not subject to the license. This includes other CC-
     licensed material, or material used under an exception or
     limitation to copyright. More considerations for licensors:
	wiki.creativecommons.org/Considerations_for_licensors

     Considerations for the public: By using one of our public
     licenses, a licensor grants the public permission to use the
     licensed material under specified terms and conditions. If
     the licensor's permission is not necessary for any reason--for
     example, because of any applicable exception or limitation to
     copyright--then that use is not regulated by the license. Our
     licenses grant only permissions under copyright and certain
     other rights that a licensor has authority to grant. Use of
     the licensed material may still be restricted for other
     reasons, including because others have copyright or other
     rights in the material. A licensor may make special requests,
     such as asking that all changes be marked or described.
     Although not required by our licenses, you are encouraged to
     respect those requests where reasonable. More_considerations
     for the public: 
	wiki.creativecommons.org/Considerations_for_licensees

=======================================================================

Creative Commons Attribution-ShareAlike 4.0 International Public
License

By exercising the Licensed Rights (defined below), You accept and agree
to be bound by the terms and conditions of this Creative Commons
Attribution-ShareAlike 4.0 International Public License ("Public
License"). To the extent this Public License may be interpreted as a
contract, You are granted the Licensed Rights in consideration of Your
acceptance of these terms and conditions, and the Licensor grants You
such rights in consideration of benefits the Licensor receives from
making the Licensed Material available under these terms and
conditions.


Section 1 -- Definitions.

  a. Adapted Material means material subject to Copyright and Similar
     Rights that is derived from or based upon the Licensed Material
     and in which the Licensed Material is translated, altered,
     arranged, transformed, or otherwise modified in a manner requiring
     permission under the Copyright and Similar Rights held by the
     Licensor. For purposes of this Public License, where the Licensed
     Material is a musical work, performance, or sound recording,
     Adapted Material is always produced where the Licensed Material is
     synched in timed relation with a moving image.

  b. Adapter's License means the license You apply to Your Copyright
     and Similar Rights in Your contributions to Adapted Material in
     accordance with the terms and conditions of this Public License.

  c. BY-SA Compatible License means a license listed at
     creativecommons.org/compatiblelicenses, approved by Creative
     Commons as essentially the equivalent of this Public License.

  d. Copyright and Similar Rights means copyright and/or similar rights
     closely related to copyright including, without limitation,
     performance, broadcast, sound recording, and Sui Generis Database
     Rights, without regard to how the rights are labeled or
     categorized. For purposes of this Public License, the rights
     specified in Section 2(b)(1)-(2) are not Copyright and Similar
     Rights.

  e. Effective Technological Measures means those measures that, in the
     absence of proper authority, may not be circumvented under laws
     fulfilling obligations under Article 11 of the WIPO Copyright
     Treaty adopted on December 20, 1996, and/or similar international
     agreements.

  f. Exceptions and Limitations means fair use, fair dealing, and/or
     any other exception or limitation to Copyright and Similar Rights
     that applies to Your use of the Licensed Material.

  g. License Elements means the license attributes listed in the name
     of a Creative Commons Public License. The License Elements of this
     Public License are Attribution and ShareAlike.

  h. Licensed Material means the artistic or literary work, database,
     or other material to which the Licensor applied this Public
     License.

  i. Licensed Rights means the rights granted to You subject to the
     terms and conditions of this Public License, which are limited to
     all Copyright and Similar Rights that apply to Your use of the
     Licensed Material and that the Licensor has authority to license.

  j. Licensor means the individual(s) or entity(ies) granting rights
     under this Public License.

  k. Share means to provide material to the public by any means or
     process that requires permission under the Licensed Rights, such
     as reproduction, public display, public performance, distribution,
     dissemination, communication, or importation, and to make material
     available to the public including in ways that members of the
     public may access the material from a place and at a time
     individually chosen by them.

  l. Sui Generis Database Rights means rights other than copyright
     resulting from Directive 96/9/EC of the European Parliament and of
     the Council of 11 March 1996 on the legal protection of databases,
     as amended and/or succeeded, as well as other essentially
     equivalent rights anywhere in the world.

  m. You means the individual or entity exercising the Licensed Rights
     under this Public License. Your has a corresponding meaning.


Section 2 -- Scope.

  a. License grant.

       1. Subject to the terms and conditions of this Public License,
          the Licensor hereby grants You a worldwide, royalty-free,
          non-sublicensable, non-exclusive, irrevocable license to
          exercise the Licensed Rights in the Licensed Material to:

            a. reproduce and Share the Licensed Material, in whole or
               in part; and

            b. produce, reproduce, and Share Adapted Material.

       2. Exceptions and Limitations. For the avoidance of doubt, where
          Exceptions and Limitations apply to Your use, this Public
          License does not apply, and You do not need to comply with
          its terms and conditions.

       3. Term. The term of this Public License is specified in Section
          6(a).

       4. Media and formats; technical modifications allowed. The
          Licensor authorizes You to exercise the Licensed Rights in
          all media and formats whether now known or hereafter created,
          and to make technical modifications necessary to do so. The
          Licensor waives and/or agrees not to assert any right or
          authority to forbid You from making technical modifications
          necessary to exercise the Licensed Rights, including
          technical modifications necessary to circumvent Effective
          Technological Measures. For purposes of this Public License,
          simply making modifications authorized by this Section 2(a)
          (4) never produces Adapted Material.

       5. Downstream recipients.

            a. Offer from the Licensor -- Licensed Material. Every
               recipient of the Licensed Material automatically
               receives an offer from the Licensor to exercise the
               Licensed Rights under the terms and conditions of this
               Public License.

            b. Additional offer from the Licensor -- Adapted Material.
               Every recipient of Adapted Material from You
               automatically receives an offer from the Licensor to
               exercise the Licensed Rights in the Adapted Material
               under the conditions of the Adapter's License You apply.

            c. No downstream restrictions. You may not offer or impose
               any additional or different terms or conditions on, or
               apply any Effective Technological Measures to, the
               Licensed Material if doing so restricts exercise of the
               Licensed Rights by any recipient of the Licensed
               Material.

       6. No endorsement. Nothing in this Public License constitutes or
          may be construed as permission to assert or imply that You
          are, or that Your use of the Licensed Material is, connected
          with, or sponsored, endorsed, or granted official status by,
          the Licensor or others designated to receive attribution as
          provided in Section 3(a)(1)(A)(i).

  b. Other rights.

       1. Moral rights, such as the right of integrity, are not
          licensed under this Public License, nor are publicity,
          privacy, and/or other similar personality rights; however, to
          the extent possible, the Licensor waives and/or agrees not to
          assert any such rights held by the Licensor to the limited
          extent necessary to allow You to exercise the Licensed
          Rights, but not otherwise.

       2. Patent and trademark rights are not licensed under this
          Public License.

       3. To the extent possible, the Licensor waives any right to
          collect royalties from You for the exercise of the Licensed
          Rights, whether directly or through a collecting society
          under any voluntary or waivable statutory or compulsory
          licensing scheme. In all other cases the Licensor expressly
          reserves any right to collect such royalties.


Section 3 -- License Conditions.

Your exercise of the Licensed Rights is expressly made subject to the
following conditions.

  a. Attribution.

       1. If You Share the Licensed Material (including in modified
          form), You must:

            a. retain the following if it is supplied by the Licensor
               with the Licensed Material:

                 i. identification of the creator(s) of the Licensed
                    Material and any others designated to receive
                    attribution, in any reasonable manner requested by
                    the Licensor (including by pseudonym if
                    designated);

                ii. a copyright notice;

               iii. a notice that refers to this Public License;

                iv. a notice that refers to the disclaimer of
                    warranties;

                 v. a URI or hyperlink to the Licensed Material to the
                    extent reasonably practicable;

            b. indicate if You modified the Licensed Material and
               retain an indication of any previous modifications; and

            c. indicate the Licensed Material is licensed under this
               Public License, and include the text of, or the URI or
               hyperlink to, this Public License.

       2. You may satisfy the conditions in Section 3(a)(1) in any
          reasonable manner based on the medium, means, and context in
          which You Share the Licensed Material. For example, it may be
          reasonable to satisfy the conditions by providing a URI or
          hyperlink to a resource that includes the required
          information.

       3. If requested by the Licensor, You must remove any of the
          information required by Section 3(a)(1)(A) to the extent
          reasonably practicable.

  b. ShareAlike.

     In addition to the conditions in Section 3(a), if You Share
     Adapted Material You produce, the following conditions also apply.

       1. The Adapter's License You apply must be a Creative Commons
          license with the same License Elements, this version or
          later, or a BY-SA Compatible License.

       2. You must include the text of, or the URI or hyperlink to, the
          Adapter's License You apply. You may satisfy this condition
          in any reasonable manner based on the medium, means, and
          context in which You Share Adapted Material.

       3. You may not offer or impose any additional or different terms
          or conditions on, or apply any Effective Technological
          Measures to, Adapted Material that restrict exercise of the
          rights granted under the Adapter's License You apply.


Section 4 -- Sui Generis Database Rights.

Where the Licensed Rights include Sui Generis Database Rights that
apply to Your use of the Licensed Material:

  a. for the avoidance of doubt, Section 2(a)(1) grants You the right
     to extract, reuse, reproduce, and Share all or a substantial
     portion of the contents of the database;

  b. if You include all or a substantial portion of the database
     contents in a database in which You have Sui Generis Database
     Rights, then the database in which You have Sui Generis Database
     Rights (but not its individual contents) is Adapted Material,

     including for purposes of Section 3(b); and
  c. You must comply with the conditions in Section 3(a) if You Share
     all or a substantial portion of the contents of the database.

For the avoidance of doubt, this Section 4 supplements and does not
replace Your obligations under this Public License where the Licensed
Rights include other Copyright and Similar Rights.


Section 5 -- Disclaimer of Warranties and Limitation of Liability.

  a. UNLESS OTHERWISE SEPARATELY UNDERTAKEN BY THE LICENSOR, TO THE
     EXTENT POSSIBLE, THE LICENSOR OFFERS THE LICENSED MATERIAL AS-IS
     AND AS-AVAILABLE, AND MAKES NO REPRESENTATIONS OR WARRANTIES OF
     ANY KIND CONCERNING THE LICENSED MATERIAL, WHETHER EXPRESS,
     IMPLIED, STATUTORY, OR OTHER. THIS INCLUDES, WITHOUT LIMITATION,
     WARRANTIES OF TITLE, MERCHANTABILITY, FITNESS FOR A PARTICULAR
     PURPOSE, NON-INFRINGEMENT, ABSENCE OF LATENT OR OTHER DEFECTS,
     ACCURACY, OR THE PRESENCE OR ABSENCE OF ERRORS, WHETHER OR NOT
     KNOWN OR DISCOVERABLE. WHERE DISCLAIMERS OF WARRANTIES ARE NOT
     ALLOWED IN FULL OR IN PART, THIS DISCLAIMER MAY NOT APPLY TO YOU.

  b. TO THE EXTENT POSSIBLE, IN NO EVENT WILL THE LICENSOR BE LIABLE
     TO YOU ON ANY LEGAL THEORY (INCLUDING, WITHOUT LIMITATION,
     NEGLIGENCE) OR OTHERWISE FOR ANY DIRECT, SPECIAL, INDIRECT,
     INCIDENTAL, CONSEQUENTIAL, PUNITIVE, EXEMPLARY, OR OTHER LOSSES,
     COSTS, EXPENSES, OR DAMAGES ARISING OUT OF THIS PUBLIC LICENSE OR
     USE OF THE LICENSED MATERIAL, EVEN IF THE LICENSOR HAS BEEN
     ADVISED OF THE POSSIBILITY OF SUCH LOSSES, COSTS, EXPENSES, OR
     DAMAGES. WHERE A LIMITATION OF LIABILITY IS NOT ALLOWED IN FULL OR
     IN PART, THIS LIMITATION MAY NOT APPLY TO YOU.

  c. The disclaimer of warranties and limitation of liability provided
     above shall be interpreted in a manner that, to the extent
     possible, most closely approximates an absolute disclaimer and
     waiver of all liability.


Section 6 -- Term and Termination.

  a. This Public License applies for the term of the Copyright and
     Similar Rights licensed here. However, if You fail to comply with
     this Public License, then Your rights under this Public License
     terminate automatically.

  b. Where Your right to use the Licensed Material has terminated under
     Section 6(a), it reinstates:

       1. automatically as of the date the violation is cured, provided
          it is cured within 30 days of Your discovery of the
          violation; or

       2. upon express reinstatement by the Licensor.

     For the avoidance of doubt, this Section 6(b) does not affect any
     right the Licensor may have to seek remedies for Your violations
     of this Public License.

  c. For the avoidance of doubt, the Licensor may also offer the
     Licensed Material under separate terms or conditions or stop
     distributing the Licensed Material at any time; however, doing so
     will not terminate this Public License.

  d. Sections 1, 5, 6, 7, and 8 survive termination of this Public
     License.


Section 7 -- Other Terms and Conditions.

  a. The Licensor shall not be bound by any additional or different
     terms or conditions communicated by You unless expressly agreed.

  b. Any arrangements, understandings, or agreements regarding the
     Licensed Material not stated herein are separate from and
     independent of the terms and conditions of this Public License.


Section 8 -- Interpretation.

  a. For the avoidance of doubt, this Public License does not, and
     shall not be interpreted to, reduce, limit, restrict, or impose
     conditions on any use of the Licensed Material that could lawfully
     be made without permission under this Public License.

  b. To the extent possible, if any provision of this Public License is
     deemed unenforceable, it shall be automatically reformed to the
     minimum extent necessary to make it enforceable. If the provision
     cannot be reformed, it shall be severed from this Public License
     without affecting the enforceability of the remaining terms and
     conditions.

  c. No term or condition of this Public License will be waived and no
     failure to comply consented to unless expressly agreed to by the
     Licensor.

  d. Nothing in this Public License constitutes or may be interpreted
     as a limitation upon, or waiver of, any privileges and immunities
     that apply to the Licensor or You, including from the legal
     processes of any jurisdiction or authority.


=======================================================================

Creative Commons is not a party to its public licenses.
Notwithstanding, Creative Commons may elect to apply one of its public
licenses to material it publishes and in those instances will be
considered the "Licensor." Except for the limited purpose of indicating
that material is shared under a Creative Commons public license or as
otherwise permitted by the Creative Commons policies published at
creativecommons.org/policies, Creative Commons does not authorize the
use of the trademark "Creative Commons" or any other trademark or logo
of Creative Commons without its prior written consent including,
without limitation, in connection with any unauthorized modifications
to any of its public licenses or any other arrangements,
understandings, or agreements concerning use of licensed material. For
the avoidance of doubt, this paragraph does not form part of the public
licenses.

Creative Commons may be contacted at creativecommons.org.


==> license-texts/doclicense-CC-zero-1.0-latex.tex <==
\advance\csname @enumdepth\endcsname\csname @ne\endcsname
\section{Creative Commons Legal Code}

\subsection{CC0 1.0 Universal}







Official translations of this legal tool are available in other languages.


\begin{quotation}
CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT
PROVIDE LEGAL SERVICES. DISTRIBUTION OF THIS DOCUMENT DOES
NOT CREATE AN ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS
PROVIDES THIS INFORMATION ON AN ``AS-IS'' BASIS. CREATIVE
COMMONS MAKES NO WARRANTIES REGARDING THE USE OF THIS
DOCUMENT OR THE INFORMATION OR WORKS PROVIDED HEREUNDER, AND
DISCLAIMS LIABILITY FOR DAMAGES RESULTING FROM THE USE OF
THIS DOCUMENT OR THE INFORMATION OR WORKS PROVIDED
HEREUNDER.
\end{quotation}
\subsubsection{\emph{Statement of Purpose}}
\par The laws of most jurisdictions throughout the world
automatically confer exclusive Copyright and Related Rights
(defined below) upon the creator and subsequent owner(s) (each
and all, an ``owner'') of an original work of authorship and/or
a database (each, a ``Work'').
\par Certain owners wish to permanently relinquish those rights
to a Work for the purpose of contributing to a commons of
creative, cultural and scientific works (``Commons'') that the
public can reliably and without fear of later claims of
infringement build upon, modify, incorporate in other works,
reuse and redistribute as freely as possible in any form
whatsoever and for any purposes, including without limitation
commercial purposes. These owners may contribute to the
Commons to promote the ideal of a free culture and the further
production of creative, cultural and scientific works, or to
gain reputation or greater distribution for their Work in part
through the use and efforts of others.
\par For these and/or other purposes and motivations, and
without any expectation of additional consideration or
compensation, the person associating CC0 with a Work (the
``Affirmer''), to the extent that he or she is an owner of
Copyright and Related Rights in the Work, voluntarily elects
to apply CC0 to the Work and publicly distribute the Work
under its terms, with knowledge of his or her Copyright and
Related Rights in the Work and the meaning and intended legal
effect of CC0 on those rights.
\par \textbf{1. Copyright and Related Rights.}
A Work made available under CC0 may be protected by
copyright and related or neighboring rights (``Copyright and
Related Rights''). Copyright and Related Rights include, but
are not limited to, the following:

\begin{enumerate}
\item the right to reproduce, adapt, distribute, perform,
display, communicate, and translate a Work;
\item  moral rights retained by the original author(s) and/or
performer(s);
\item publicity and privacy rights pertaining to a person's
image or likeness depicted in a Work;
\item rights protecting against unfair competition in regards
to a Work, subject to the limitations in paragraph 4(a),
below;
\item rights protecting the extraction, dissemination, use and
reuse of data in a Work;
\item database rights (such as those arising under Directive
96/9/EC of the European Parliament and of the Council of 11
March 1996 on the legal protection of databases, and under
any national implementation thereof, including any amended
or successor version of such directive); and
\item other similar, equivalent or corresponding rights
throughout the world based on applicable law or treaty, and
any national implementations thereof.
\end{enumerate}
\par \textbf{2. Waiver.} To the greatest extent
permitted by, but not in contravention of, applicable law,
Affirmer hereby overtly, fully, permanently, irrevocably and
unconditionally waives, abandons, and surrenders all of
Affirmer's Copyright and Related Rights and associated claims
and causes of action, whether now known or unknown (including
existing as well as future claims and causes of action), in
the Work (i) in all territories worldwide, (ii) for the
maximum duration provided by applicable law or treaty
(including future time extensions), (iii) in any current or
future medium and for any number of copies, and (iv) for any
purpose whatsoever, including without limitation commercial,
advertising or promotional purposes (the ``Waiver''). Affirmer
makes the Waiver for the benefit of each member of the public
at large and to the detriment of Affirmer's heirs and
successors, fully intending that such Waiver shall not be
subject to revocation, rescission, cancellation, termination,
or any other legal or equitable action to disrupt the quiet
enjoyment of the Work by the public as contemplated by
Affirmer's express Statement of Purpose.

\par \textbf{3. Public License Fallback.} Should any
part of the Waiver for any reason be judged legally invalid or
ineffective under applicable law, then the Waiver shall be
preserved to the maximum extent permitted taking into account
Affirmer's express Statement of Purpose. In addition, to the
extent the Waiver is so judged Affirmer hereby grants to each
affected person a royalty-free, non transferable, non
sublicensable, non exclusive, irrevocable and unconditional
license to exercise Affirmer's Copyright and Related Rights
in the Work (i) in all territories worldwide, (ii) for the
maximum duration provided by applicable law or treaty
(including future time extensions), (iii) in any current or
future medium and for any number of copies, and (iv) for any
purpose whatsoever, including without limitation commercial,
advertising or promotional purposes (the ``License''). The
License shall be deemed effective as of the date CC0 was
applied by Affirmer to the Work. Should any part of the
License for any reason be judged legally invalid or
ineffective under applicable law, such partial invalidity or
ineffectiveness shall not invalidate the remainder of the
License, and in such case Affirmer hereby affirms that he or
she will not (i) exercise any of his or her remaining
Copyright and Related Rights in the Work or (ii) assert any
associated claims and causes of action with respect to the
Work, in either case contrary to Affirmer's express Statement
of Purpose.
\par \textbf{4. Limitations and Disclaimers.}
\begin{enumerate}
\item No trademark or patent rights held by Affirmer are
waived, abandoned, surrendered, licensed or otherwise
affected by this document.
\item Affirmer offers the Work as-is and makes no
representations or warranties of any kind concerning the
Work, express, implied, statutory or otherwise, including
without limitation warranties of title, merchantability,
fitness for a particular purpose, non infringement, or the
absence of latent or other defects, accuracy, or the present
or absence of errors, whether or not discoverable, all to
the greatest extent permissible under applicable law.
\item Affirmer disclaims responsibility for clearing rights of
other persons that may apply to the Work or any use thereof,
including without limitation any person's Copyright and
Related Rights in the Work. Further, Affirmer disclaims
responsibility for obtaining any necessary consents,
permissions or other rights required for any use of the
Work.
\item Affirmer understands and acknowledges that Creative
Commons is not a party to this document and has no duty or
obligation with respect to this CC0 or use of the Work.
\end{enumerate}
\begin{quotation}Additional languages available: français, Nederlands, polski, suomeksi, 日本語. Please read the FAQ for more information about official translations.\end{quotation}



\advance\csname @enumdepth\endcsname-\csname @ne\endcsname


==> license-texts/doclicense-CC-zero-1.0-plaintext.tex <==
Creative Commons Legal Code

CC0 1.0 Universal

    CREATIVE COMMONS CORPORATION IS NOT A LAW FIRM AND DOES NOT PROVIDE
    LEGAL SERVICES. DISTRIBUTION OF THIS DOCUMENT DOES NOT CREATE AN
    ATTORNEY-CLIENT RELATIONSHIP. CREATIVE COMMONS PROVIDES THIS
    INFORMATION ON AN "AS-IS" BASIS. CREATIVE COMMONS MAKES NO WARRANTIES
    REGARDING THE USE OF THIS DOCUMENT OR THE INFORMATION OR WORKS
    PROVIDED HEREUNDER, AND DISCLAIMS LIABILITY FOR DAMAGES RESULTING FROM
    THE USE OF THIS DOCUMENT OR THE INFORMATION OR WORKS PROVIDED
    HEREUNDER.

Statement of Purpose

The laws of most jurisdictions throughout the world automatically confer
exclusive Copyright and Related Rights (defined below) upon the creator
and subsequent owner(s) (each and all, an "owner") of an original work of
authorship and/or a database (each, a "Work").

Certain owners wish to permanently relinquish those rights to a Work for
the purpose of contributing to a commons of creative, cultural and
scientific works ("Commons") that the public can reliably and without fear
of later claims of infringement build upon, modify, incorporate in other
works, reuse and redistribute as freely as possible in any form whatsoever
and for any purposes, including without limitation commercial purposes.
These owners may contribute to the Commons to promote the ideal of a free
culture and the further production of creative, cultural and scientific
works, or to gain reputation or greater distribution for their Work in
part through the use and efforts of others.

For these and/or other purposes and motivations, and without any
expectation of additional consideration or compensation, the person
associating CC0 with a Work (the "Affirmer"), to the extent that he or she
is an owner of Copyright and Related Rights in the Work, voluntarily
elects to apply CC0 to the Work and publicly distribute the Work under its
terms, with knowledge of his or her Copyright and Related Rights in the
Work and the meaning and intended legal effect of CC0 on those rights.

1. Copyright and Related Rights. A Work made available under CC0 may be
protected by copyright and related or neighboring rights ("Copyright and
Related Rights"). Copyright and Related Rights include, but are not
limited to, the following:

  i. the right to reproduce, adapt, distribute, perform, display,
     communicate, and translate a Work;
 ii. moral rights retained by the original author(s) and/or performer(s);
iii. publicity and privacy rights pertaining to a person's image or
     likeness depicted in a Work;
 iv. rights protecting against unfair competition in regards to a Work,
     subject to the limitations in paragraph 4(a), below;
  v. rights protecting the extraction, dissemination, use and reuse of data
     in a Work;
 vi. database rights (such as those arising under Directive 96/9/EC of the
     European Parliament and of the Council of 11 March 1996 on the legal
     protection of databases, and under any national implementation
     thereof, including any amended or successor version of such
     directive); and
vii. other similar, equivalent or corresponding rights throughout the
     world based on applicable law or treaty, and any national
     implementations thereof.

2. Waiver. To the greatest extent permitted by, but not in contravention
of, applicable law, Affirmer hereby overtly, fully, permanently,
irrevocably and unconditionally waives, abandons, and surrenders all of
Affirmer's Copyright and Related Rights and associated claims and causes
of action, whether now known or unknown (including existing as well as
future claims and causes of action), in the Work (i) in all territories
worldwide, (ii) for the maximum duration provided by applicable law or
treaty (including future time extensions), (iii) in any current or future
medium and for any number of copies, and (iv) for any purpose whatsoever,
including without limitation commercial, advertising or promotional
purposes (the "Waiver"). Affirmer makes the Waiver for the benefit of each
member of the public at large and to the detriment of Affirmer's heirs and
successors, fully intending that such Waiver shall not be subject to
revocation, rescission, cancellation, termination, or any other legal or
equitable action to disrupt the quiet enjoyment of the Work by the public
as contemplated by Affirmer's express Statement of Purpose.

3. Public License Fallback. Should any part of the Waiver for any reason
be judged legally invalid or ineffective under applicable law, then the
Waiver shall be preserved to the maximum extent permitted taking into
account Affirmer's express Statement of Purpose. In addition, to the
extent the Waiver is so judged Affirmer hereby grants to each affected
person a royalty-free, non transferable, non sublicensable, non exclusive,
irrevocable and unconditional license to exercise Affirmer's Copyright and
Related Rights in the Work (i) in all territories worldwide, (ii) for the
maximum duration provided by applicable law or treaty (including future
time extensions), (iii) in any current or future medium and for any number
of copies, and (iv) for any purpose whatsoever, including without
limitation commercial, advertising or promotional purposes (the
"License"). The License shall be deemed effective as of the date CC0 was
applied by Affirmer to the Work. Should any part of the License for any
reason be judged legally invalid or ineffective under applicable law, such
partial invalidity or ineffectiveness shall not invalidate the remainder
of the License, and in such case Affirmer hereby affirms that he or she
will not (i) exercise any of his or her remaining Copyright and Related
Rights in the Work or (ii) assert any associated claims and causes of
action with respect to the Work, in either case contrary to Affirmer's
express Statement of Purpose.

4. Limitations and Disclaimers.

 a. No trademark or patent rights held by Affirmer are waived, abandoned,
    surrendered, licensed or otherwise affected by this document.
 b. Affirmer offers the Work as-is and makes no representations or
    warranties of any kind concerning the Work, express, implied,
    statutory or otherwise, including without limitation warranties of
    title, merchantability, fitness for a particular purpose, non
    infringement, or the absence of latent or other defects, accuracy, or
    the present or absence of errors, whether or not discoverable, all to
    the greatest extent permissible under applicable law.
 c. Affirmer disclaims responsibility for clearing rights of other persons
    that may apply to the Work or any use thereof, including without
    limitation any person's Copyright and Related Rights in the Work.
    Further, Affirmer disclaims responsibility for obtaining any necessary
    consents, permissions or other rights required for any use of the
    Work.
 d. Affirmer understands and acknowledges that Creative Commons is not a
    party to this document and has no duty or obligation with respect to
    this CC0 or use of the Work.


==> license-texts/get-pretty <==
#!/bin/bash
## @author Copyright (C) 2015 Robin Schneider <ypid@riseup.net>
## @license AGPLv3 <https://www.gnu.org/licenses/agpl-3.0.html>

get() {
    ## https://creativecommons.org/weblog/entry/27094
    modifier="$1"
    version="$2"
    wget --continue "https://creativecommons.org/licenses/${modifier}/${version}/legalcode" --output-document "doclicense-CC-${modifier}-${version}-latex.html"
    gnuhtml2latex -n "doclicense-CC-${modifier}-${version}-latex.html"
    ./strip-head-and-tail "doclicense-CC-${modifier}-${version}-latex.tex" | sed --regexp-extended '
        s@\<(https://creativecommons.org/compatiblelicenses|https://creativecommons.org/)@\\url{\1}@ig;
    ' | perl -0pe "s/\"(([^\"])*)\"/\`\`\1''/g" > "doclicense-CC-${modifier}-${version}-latex2.tex"
    mv "doclicense-CC-${modifier}-${version}-latex2.tex" "doclicense-CC-${modifier}-${version}-latex.tex"
}

## Needs different URL schema (again)?
# get 'pd' '1.0'

get 'zero' '1.0'
get 'by' '3.0'
get 'by-sa' '3.0'
get 'by-nd' '3.0'
get 'by-nc' '3.0'
get 'by-nc-sa' '3.0'
get 'by-nc-nd' '3.0'
get 'by' '4.0'
get 'by-sa' '4.0'
get 'by-nd' '4.0'
get 'by-nc' '4.0'
get 'by-nc-sa' '4.0'
get 'by-nc-nd' '4.0'

./adjust_enumerate_depth.sh

